Design-Based Inference for Spatial Experiments under Unknown Interference

We consider design-based causal inference for spatial experiments in which treatments may have effects that bleed out and feed back in complex ways. Such spatial spillover effects violate the standard ``no interference'' assumption for standard causal inference methods. The complexity of spatial spillover effects also raises the risk of misspecification and bias in model-based analyses. We offer an approach for robust inference in such settings without having to specify a parametric outcome model. We define a spatial ``average marginalized effect'' (AME) that characterizes how, in expectation, units of observation that are a specified distance from an intervention location are affected by treatment at that location, averaging over effects emanating from other intervention nodes. We show that randomization is sufficient for non-parametric identification of the AME even if the nature of interference is unknown. Under mild restrictions on the extent of interference, we establish asymptotic distributions of estimators and provide methods for both sample-theoretic and randomization-based inference. We show conditions under which the AME recovers a structural effect. We illustrate our approach with a simulation study. Then we re-analyze a randomized field experiment and a quasi-experiment on forest conservation, showing how our approach offers robust inference on policy-relevant spillover effects.

==> proofs/HAHTcomparison_details.tex <==
\textcolor{blue}{Conisder the following class of estimators, which adjust the treated and control outcomes with a treatment-arm-specfic intercepts.
	\begin{equation}
		\widehat{\tau}(\mu_1,\mu_0)= \mu_1-\mu_0 -\left( \frac{1}{Np}\sum_{i=1}^n \Z_i(\mu_i(\Y;d)-\mu_1) \frac{1}{N(1-p)}\sum_{i=1}^n (1-\Z_i)(\mu_i(\Y;d)-\mu_0)\right)
	\end{equation}
	Both the HT estimator and the linearized version of the Hajek estimator have this form: $\widehat{\mu}(d)=	\widehat{\tau}(0,0)$ and $\widehat{\mu}_{HA}(d)=	\widehat{\tau}(\mutd,\mucd)$. It is in this class of the estimators we discuss the efficiency property of the Hajek estimator. We define two interactive effects:
\begin{equation*}
	\Delta(1)=  \frac{1}{N}\sumij\left(\E[\muitt]-\E[\muict]-\left(\E[\muit]-\E[\muic]\right)\right),
\end{equation*}
and
\begin{equation*}
	\Delta(0)=  \frac{1}{N}\sumij\left(\E[\muicc]-\E[\muitc]-\left(\E[\muic]-\E[\muit]\right)\right).
\end{equation*}
Note we have the idenity $p	\Delta(1)=(1-p)\Delta(0)$.\footnote{This follows by a calculation
\begin{align*}
	& N\times\left(p\Delta(1)-(1-p)\Delta(0)\right)=  \sumij \left(p\E[\muitt]+(1-p)\E[\muitc]\right) \\
	& - \sumij  \left(p\E[\muict]+(1-p)\E[\muicc]\right)- \left(\sum_{i=1}^N c_i(d)\E[\muit] - \sum_{i=1}^N c_i(d)\E[\muic]\right)\\
	& =0 .
\end{align*}
}
		\begin{prop}
	Under C\ref{assn:bern-des}-C\ref{assn:spacing}, we have, for any scalars $\mu_1$ and $\mu_0$,
	\begin{align}
		&\V\left(	\widehat{\tau}(\mu_1,\mu_0) \right)=
		\frac{1}{N^2p}\sum_{i=1}^N \E\left[ \left(\muit- \mu_1\right)^2\right] + \frac{1}{N^2(1-p)}\sum_{i=1}^N \E\left[\left(\muic- \mu_0\right)^2\right]  \\
		-&  \frac{1}{N^2}\sum_{i=1}^N\left(\E\left[\muit - \muic - (\mu_1 - \mu_0 )\right]\right)^2\\
		+ & \frac{1}{N^2} \sumij \sum_{a=0}^1 \sum_{b=0}^1 \E[\left(\muiab - \mu_a\right) \left(\mujab - \mu_b\right)] \\
		- & \frac{1}{N^2}\sumij \sum_{a=0}^1 \sum_{b=0}^1  (-1)^{a+b} \E[\muia -\mu_a] E[\mujb - \mu_b].
	\end{align}
	In particular, we have the following algebraic identity:
	\begin{equation*}
		\V\left(	\widehat{\tau}(\mu_1,\mu_0) \right)=  \frac{(1-p)p}{N} \left( \frac{\mu_1}{p}+\frac{\mu_0}{1-p}-\left(  \frac{\bar{\mu}_1(d)}{p} + \frac{\bar{\mu}_0(d)}{1-p} +\frac{p\Delta(1)}{p(1-p)} \right)\right)^2+C,
	\end{equation*}
	where $C$ is a constant independent of $\mu_1$ and $\mu_0$.
\end{prop}
\begin{proof}
	Expanding the variance expression we have the following identity:
	\begin{align*}
		&\V\left(	\widehat{\tau}(\mu_1,\mu_0) \right)=\left(	\frac{1}{Np}-\frac{1}{N}\right)\mu^2_1 + 
		\left(\frac{1}{N(1-p)}-\frac{1}{N}\right)\mu_0^2+\frac{2}{N}\mu_1\mu_0\\
		& +\left( \left(-\frac{2}{Np} +\frac{2}{N}\right)\bar{\mu}_1(d)-\frac{2}{N}\bar{\mu}_0(d) - \frac{2}{N}\Delta(1)\right)\mu_1\\
		& +\left( \left(-\frac{2}{N(1-p)} +\frac{2}{N}\right)\bar{\mu}_0(d)-\frac{2}{N}\bar{\mu}_1(d)  - \frac{2}{N}\Delta(0)\right)\mu_0\\
		& + \V(\widehat{\tau}(0,0))\\
		& = \frac{1}{N}\left( \frac{1-p}{p}\mu_1^2 + \frac{p}{1-p}\mu_0^2 + 2\mu_1\mu_0 \right)- \frac{2}{N}\left(   \frac{1-p}{p}\bar{\mu}_1(d) +\bar{\mu}_0(d) +\Delta(1) \right)\mu_1\\
		& - \frac{2}{N}\left(   \frac{p}{1-p}\bar{\mu}_0(d) + \bar{\mu}_1(d) +\Delta(0) \right)\mu_0+ \V(\widehat{\tau}(0,0))\\		 
		& = \frac{(1-p)p}{N}\left( \frac{\mu_1^2}{p^2} +\frac{\mu_0^2}{(1-p)^2} + 2\frac{\mu_1\mu_0}{p(1-p)} \right)-  \frac{2(1-p)p}{N}\left(  \frac{\bar{\mu}_1(d)}{p} + \frac{\bar{\mu}_0(d)}{1-p} +\frac{p\Delta(1)}{p(1-p)} \right)\frac{\mu_1}{p}\\
& - \frac{2(1-p)p}{N}\left(   \frac{\bar{\mu}_0(d)}{1-p} + \frac{\bar{\mu}_1(d)}{p} +\frac{(1-p)\Delta(0)}{p(1-p)} \right)\mu_0+ \V(\widehat{\tau}(0,0))\\		 		
& = \frac{(1-p)p}{N} \left(\left(  \frac{\mu_1}{p}+\frac{\mu_0}{1-p}\right)^2- 2\left(  \frac{\bar{\mu}_1(d)}{p} + \frac{\bar{\mu}_0(d)}{1-p} +\frac{p\Delta(1)}{p(1-p)} \right)\left(  \frac{\mu_1}{p}+\frac{\mu_0}{1-p}\right)\right) + \V(\widehat{\tau}(0,0))\\
& = \frac{(1-p)p}{N} \left( \frac{\mu_1}{p}+\frac{\mu_0}{1-p}-\left(  \frac{\bar{\mu}_1(d)}{p} + \frac{\bar{\mu}_0(d)}{1-p} +\frac{p\Delta(1)}{p(1-p)} \right)\right)^2+C
	\end{align*}
where $C$ is independent of $\mu_1$ and $\mu_0$. Note we use the fact that, for each $i$ and $j$, $j\in B(i;d) $ implies that $i\in B(j;d) $ and vice versa.
\end{proof}
}



==> proofs/HTEstimator.tex <==
\subsubsection{Proof for Proposition \ref{prop:identification}}
\begin{proof}The Horvitz-Thompson estimator is defined in (\ref{eq:ht}) and the AME is defined in (\ref{def:AME}). We have:
\begin{align*}
&	\textnormal{AME}(d;\eta)   = \frac{1}{N}\sum_{i=1}^N \mu_i(1; d, \eta) - \frac{1}{N}\sum_{i=1}^N \mu_i(0; d, \eta) \\
& = \frac{1}{Np}\sum_{i=1}^N p \E[\mu_i(\Y; d) | Z_i=1 ]- \frac{1}{N(1-p)}\sum_{i=1}^N(1-p)  \E[\mu_i(\Y; d) | Z_i=0 ]\\
& = \frac{1}{Np}\sum_{i=1}^N \E[Z_i \mu_i(\Y; d) ] - \frac{1}{N(1-p)}\sum_{i=1}^N\E[(1-Z_i)\mu_i(\Y; d) ]\\
& = \E\left[ \frac{1}{Np}\sum_{i=1}^N Z_i \mu_i(\Y; d) - \frac{1}{N(1-p)}\sum_{i=1}^N (1-Z_i) \mu_i(\Y; d)\right]= \E[\widehat{\tau}_{\HT}(d) ],
\end{align*}
where the second equality uses the definition of $\mu_i(z; d, \eta)$, and the third equality follows from Lemma \ref{lemma:1}.
\end{proof}

\subsubsection{Variance Characterization}
We now characterize the variance of the Horvitz-Thompson estimator. 
\begin{lemma}\label{lemma:ht-var}
	Under conditions C\ref{assn:bern-des}-C\ref{assn:local-inf} as defined in the main text, the variance of estimator $\widehat{\tau}_{\HT}(d)$ is bounded as follows:
	\begin{align*}
		& \Var\left(\widehat{\tau}_{\HT}(d) \right) 
		\leq  \frac{1}{N^2p} \sum_{i=1}^N \E\left[\muit^2\right] + \frac{1}{N^2(1-p)} \sum_{i=1}^N \E\left[ \muic^2 \right] \\
		& + \frac{1}{N^2}\sumij\sum_{a=0}^1\sum_{b=0}^1 (-1)^{a+b}\Big\{ \E\left[\muiab\mujab  \right] - \E\left[\muia\right] \E\left[\mujb\right]\Big\},
	\end{align*}
	and, in addition under C\ref{assn:spacing}, we have that
	\begin{align*}
		\Var\left(\widehat{\tau}_{\HT}(d) \right) = O\left(\frac{1}{N}\right).
	\end{align*}
\end{lemma}


\begin{proof}
	Using the expression of the Horvitz-Thompson estimator, we have:
	\begin{align*}
		& \Var\left(\widehat{\tau}_{\HT}(d)  \right) =\frac{1}{N^2} \Var\left[\sum_{i=1}^N \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y; d) \right] \\
		& =  \frac{1}{N^2} \sum_{i=1}^N \Var\left[ \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y; d) \right] \\
		& + \frac{1}{N^2} \sum_{i=1}^N \sum_{j \neq i} \Cov\left[ \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y; d), \left(\frac{Z_j}{p} - \frac{1-Z_j}{1-p}\right)\mu_j(\Y; d) \right] \\
		= & \frac{1}{N^2} \sum_{i=1}^N \E\left[\left( \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y; d) \right)^2\right] - \frac{1}{N^2} \sum_{i=1}^N \left(\E\left[ \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y; d) \right] \right)^2\\
		& + \frac{1}{N^2} \sum_{i=1}^N \sum_{j \neq i} \Cov\left[ \frac{Z_i}{p}\mu_i(\Y; d), \frac{Z_j}{p} \mu_j(\Y; d) \right] \\
		& - \frac{1}{N^2} \sum_{i=1}^N \sum_{j \neq i} \Cov\left[ \frac{Z_i}{p}\mu_i(\Y; d), \frac{1-Z_j}{1-p} \mu_j(\Y; d) \right] \\
		& - \frac{1}{N^2} \sum_{i=1}^N \sum_{j \neq i} \Cov\left[ \frac{1-Z_i}{1-p}\mu_i(\Y; d), \frac{Z_j}{p} \mu_j(\Y; d) \right] \\
		& + \frac{1}{N^2} \sum_{i=1}^N \sum_{j \neq i} \Cov\left[ \frac{1-Z_i}{1-p}\mu_i(\Y; d), \frac{1-Z_j}{1-p} \mu_j(\Y; d) \right].
	\end{align*}
	
	We further expand the first two terms in the above expression:
	\begin{align*}
		& \frac{1}{N^2} \sum_{i=1}^N \E\left[\left( \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y; d) \right)^2\right] - \frac{1}{N^2} \sum_{i=1}^N \E\left[ \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y; d) \right]^2\\
		= & \frac{1}{N^2} \sum_{i=1}^N \E\left[ \frac{Z_i^2}{p^2} \mu_i^2(\Y; d) \right] + \frac{1}{N^2} \sum_{i=1}^N \E\left[ \frac{(1-Z_i)^2}{(1-p)^2} \mu_i^2(\Y); d) \right] \\
		& - \frac{1}{N^2} \sum_{i=1}^N \E^2\left[ \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y; d) \right] \\
		= & \frac{1}{N^2p} \sum_{i=1}^N \E\left[\muit^2\right] + \frac{1}{N^2(1-p)} \sum_{i=1}^N \E\left[ \muic^2\right] - \frac{1}{N^2} \sum_{i=1}^N \left(\E\left[\muit - \muic \right]\right)^2 \\
		\leq &  \frac{1}{N^2p} \sum_{i=1}^N \E\left[\muit^2 \right] + \frac{1}{N^2(1-p)} \sum_{i=1}^N \E\left[ \muic^2\right].
	\end{align*}
	We also have:
	\begin{align*}
		\frac{1}{Np} \sum_{i=1}^N \E\left[\muit^2\right] + \frac{1}{N^2(1-p)} \sum_{i=1}^N \E\left[ \muic^2\right] - \frac{1}{N^2} \sum_{i=1}^N \left(\E\left[\muit - \muic \right]\right)^2= O\left(1\right),
	\end{align*}
	since C\ref{assn:bounded-y} implies that all the moments are bounded. Next, we examine the first covariance term, which equals
	\begin{align*}
		& \frac{1}{N^2} \sum_{i=1}^N \sum_{j \neq i} \Cov\left[ \frac{Z_i}{p}\mu_i(\Y(\Z); d), \frac{Z_j}{p} \mu_j(\Y(\Z); d) \right] = \frac{1}{N^2}\sumij\Cov\left[ \frac{Z_i}{p}\mu_i(\Y(\Z); d), \frac{Z_j}{p} \mu_j(\Y(\Z); d) \right] \\
		= & \frac{1}{N^2} \sumij\E\left[\muitt\mujtt\right]- \frac{1}{N^2}\sumij\E\left[\muit \right]\E\left[\mujt \right].
	\end{align*}
	The first equality holds because of assumption C3 on local interference: for $j \notin \mathcal{B}(i;d)$, $\muitt =\muit$ and $\E\left[\muitt\mujtt \right] =\E[\muit]\E[\mujt]$, following the definition of interference in Section 4. Moreover,
	\begin{align*}
		\frac{1}{N^2} \sumij\E\left[\muitt\mujtt\right]- \frac{1}{N^2}\sumij\E\left[\muit \right]\E\left[\mujt \right]= O\left(1\right),
	\end{align*}
	since $|\mathcal{B}(i;d)|$ is bounded by (C4a). Other covariance terms have similar forms. We obtain the bound of the variance and its convergence rate by combining these terms together. 
\end{proof}
\subsubsection{Unbiasedness of the HT estimator in observaitional studies}\label{Section:HTobsproof}

\begin{proof}
	Note that in our setup the only randomness comes from the random assignment. Hence functions of the covariates are considered fixed.  In the scenario of observational studies and known propensity scores, we have
	\begin{align*}
		&	\textnormal{AME}(d;\eta)  = \frac{1}{N}\sum_{i=1}^N \mu_i(1; d, \eta) - \frac{1}{N}\sum_{i=1}^N \mu_i(0; d, \eta) \\
		& = \frac{1}{N}\sum_{i=1}^N \E\left[ \frac{p(\C) }{p(\C) }\mu_i(\Y(\mathbf{Z}); d)|Z_i=1\right] - \frac{1}{N}\sum_{i=1}^N \E\left[\frac{1-p(\mathbf{C}_i) }{1-p(\mathbf{C}_i) }\mu_i(\Y( \mathbf{Z}); d)|Z_i=0\right]\\
		& = \frac{1}{N}\sum_{i=1}^N\frac{p(\C) }{p(\C) } \E[Z_i\mu_i(\Y(\mathbf{Z}); d) | Z_i=1] -  \frac{1}{N}\sum_{i=1}^N\frac{1-p(\C) }{1-p(\C) } \E[(1-Z_i)\mu_i(\Y(\mathbf{Z}); d) | Z_i=0]   \\
		& = \E\left[ \frac{1}{N}\sum_{i=1}^N \frac{Z_i}{p(\C) } \mu_i(\Y; d) - \frac{1}{N}\sum_{i=1}^N \frac{1-Z_i}{p(\C)} \mu_i(\Y; d)\right]
	\end{align*}
	The third equality uses C\ref{assn:assignment_obsstudy} and the fourth equality uses C\ref{assn:assignment_obsstudy}-(ii) and the law of total expectations.
\end{proof}


%\begin{proof}
%Using the expression of the Horvitz-Thompson estimator, we have:
%\begin{align*}
%& \Var\left(\widehat{\tau}(d)  \right) \\
%= &\frac{1}{N^2} \Var\left[\sum_{i=1}^N \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y(\Z); d) \right] \\
%= & \frac{1}{N^2} \sum_{i=1}^N \Var\left[ \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y(\Z); d) \right] \\
%& + \frac{1}{N^2} \sum_{i=1}^N \sum_{j \neq i} \Cov\left[ \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y(\Z); d), \left(\frac{Z_j}{p} - \frac{1-Z_j}{1-p}\right)\mu_j(\Y(\Z); d) \right] \\
%= & \frac{1}{N^2} \sum_{i=1}^N \Var\left[ \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y(\Z); d) \right] \\
%& + \frac{1}{N^2} \sum_{i=1}^N \sum_{j \in \mathcal{B}(i;d)} \Cov\left[ \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y(\Z); d), \left(\frac{Z_j}{p} - \frac{1-Z_j}{1-p}\right)\mu_j(\Y(\Z); d) \right] \\
%= & \frac{1}{N}\times \frac{1}{N}\Var\left[ \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y(\Z); d) \right] \\
%+ & \frac{1}{N}\times \frac{1}{N}\sum_{i=1}^N \sum_{j\in\mathcal{B}(i;d)}\Cov\left[ \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y(\Z); d), \left(\frac{Z_j}{p} - \frac{1-Z_j}{1-p}\right)\mu_j(\Y(\Z); d) \right]\\
%= & \frac{1}{N}\times O(1) + \frac{1}{N}\times O(1),
%\end{align*}
%where for the last line we used C\ref{assn:bounded-y}-C\ref{assn:local-inf}. In particular the cardinally of $\mathcal{B}(i;d)$ is bounded for all $i=1,...,N$.
%\end{proof}

==> proofs/identification.tex <==
\subsubsection{Proof for Proposition \ref{prop:identification}}
\begin{proof}The Horvitz-Thompson estimator is defined in (\ref{eq:ht}) and the AME is defined in (\ref{def:AME}). We have:
\begin{align*}
&	\textnormal{AME}(d;\eta)   = \frac{1}{N}\sum_{i=1}^N \mu_i(1; d, \eta) - \frac{1}{N}\sum_{i=1}^N \mu_i(0; d, \eta) \\
& = \frac{1}{Np}\sum_{i=1}^N p \E[\mu_i(\Y; d) | Z_i=1 ]- \frac{1}{N(1-p)}\sum_{i=1}^N(1-p)  \E[\mu_i(\Y; d) | Z_i=0 ]\\
& = \frac{1}{Np}\sum_{i=1}^N \E[Z_i \mu_i(\Y; d) ] - \frac{1}{N(1-p)}\sum_{i=1}^N\E[(1-Z_i)\mu_i(\Y; d) ]\\
& = \E\left[ \frac{1}{Np}\sum_{i=1}^N Z_i \mu_i(\Y; d) - \frac{1}{N(1-p)}\sum_{i=1}^N (1-Z_i) \mu_i(\Y; d)\right]= \E[\widehat{\tau}_{\HT}(d) ],
\end{align*}
where the second equality uses the definition of $\mu_i(z; d, \eta)$, and the third equality follows from Lemma \ref{lemma:1}.
\end{proof}

\subsubsection{Variance Characterization}
We now characterize the variance of the Horvitz-Thompson estimator. 
\begin{lemma}\label{lemma:ht-var}
	Under conditions C\ref{assn:bern-des}-C\ref{assn:local-inf} as defined in the main text, the variance of estimator $\widehat{\tau}_{\HT}(d)$ is bounded as follows:
	\begin{align*}
		& \Var\left(\widehat{\tau}_{\HT}(d) \right) 
		\leq  \frac{1}{N^2p} \sum_{i=1}^N \E\left[\muit^2\right] + \frac{1}{N^2(1-p)} \sum_{i=1}^N \E\left[ \muic^2 \right] \\
		& + \frac{1}{N^2}\sumij\sum_{a=0}^1\sum_{b=0}^1 (-1)^{a+b}\Big\{ \E\left[\muiab\mujab  \right] - \E\left[\muia\right] \E\left[\mujb\right]\Big\},
	\end{align*}
	and, in addition under C\ref{assn:spacing}, we have that
	\begin{align*}
		\Var\left(\widehat{\tau}_{\HT}(d) \right) = O\left(\frac{1}{N}\right).
	\end{align*}
\end{lemma}


\begin{proof}
	Using the expression of the Horvitz-Thompson estimator, we have:
	\begin{align*}
		& \Var\left(\widehat{\tau}_{\HT}(d)  \right) =\frac{1}{N^2} \Var\left[\sum_{i=1}^N \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y; d) \right] \\
		& =  \frac{1}{N^2} \sum_{i=1}^N \Var\left[ \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y; d) \right] \\
		& + \frac{1}{N^2} \sum_{i=1}^N \sum_{j \neq i} \Cov\left[ \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y; d), \left(\frac{Z_j}{p} - \frac{1-Z_j}{1-p}\right)\mu_j(\Y; d) \right] \\
		= & \frac{1}{N^2} \sum_{i=1}^N \E\left[\left( \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y; d) \right)^2\right] - \frac{1}{N^2} \sum_{i=1}^N \left(\E\left[ \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y; d) \right] \right)^2\\
		& + \frac{1}{N^2} \sum_{i=1}^N \sum_{j \neq i} \Cov\left[ \frac{Z_i}{p}\mu_i(\Y; d), \frac{Z_j}{p} \mu_j(\Y; d) \right] \\
		& - \frac{1}{N^2} \sum_{i=1}^N \sum_{j \neq i} \Cov\left[ \frac{Z_i}{p}\mu_i(\Y; d), \frac{1-Z_j}{1-p} \mu_j(\Y; d) \right] \\
		& - \frac{1}{N^2} \sum_{i=1}^N \sum_{j \neq i} \Cov\left[ \frac{1-Z_i}{1-p}\mu_i(\Y; d), \frac{Z_j}{p} \mu_j(\Y; d) \right] \\
		& + \frac{1}{N^2} \sum_{i=1}^N \sum_{j \neq i} \Cov\left[ \frac{1-Z_i}{1-p}\mu_i(\Y; d), \frac{1-Z_j}{1-p} \mu_j(\Y; d) \right].
	\end{align*}
	
	We further expand the first two terms in the above expression:
	\begin{align*}
		& \frac{1}{N^2} \sum_{i=1}^N \E\left[\left( \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y; d) \right)^2\right] - \frac{1}{N^2} \sum_{i=1}^N \E\left[ \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y; d) \right]^2\\
		= & \frac{1}{N^2} \sum_{i=1}^N \E\left[ \frac{Z_i^2}{p^2} \mu_i^2(\Y; d) \right] + \frac{1}{N^2} \sum_{i=1}^N \E\left[ \frac{(1-Z_i)^2}{(1-p)^2} \mu_i^2(\Y); d) \right] \\
		& - \frac{1}{N^2} \sum_{i=1}^N \E^2\left[ \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y; d) \right] \\
		= & \frac{1}{N^2p} \sum_{i=1}^N \E\left[\muit^2\right] + \frac{1}{N^2(1-p)} \sum_{i=1}^N \E\left[ \muic^2\right] - \frac{1}{N^2} \sum_{i=1}^N \left(\E\left[\muit - \muic \right]\right)^2 \\
		\leq &  \frac{1}{N^2p} \sum_{i=1}^N \E\left[\muit^2 \right] + \frac{1}{N^2(1-p)} \sum_{i=1}^N \E\left[ \muic^2\right].
	\end{align*}
	We also have:
	\begin{align*}
		\frac{1}{Np} \sum_{i=1}^N \E\left[\muit^2\right] + \frac{1}{N^2(1-p)} \sum_{i=1}^N \E\left[ \muic^2\right] - \frac{1}{N^2} \sum_{i=1}^N \left(\E\left[\muit - \muic \right]\right)^2= O\left(1\right),
	\end{align*}
	since C\ref{assn:bounded-y} implies that all the moments are bounded. Next, we examine the first covariance term, which equals
	\begin{align*}
		& \frac{1}{N^2} \sum_{i=1}^N \sum_{j \neq i} \Cov\left[ \frac{Z_i}{p}\mu_i(\Y(\Z); d), \frac{Z_j}{p} \mu_j(\Y(\Z); d) \right] = \frac{1}{N^2}\sumij\Cov\left[ \frac{Z_i}{p}\mu_i(\Y(\Z); d), \frac{Z_j}{p} \mu_j(\Y(\Z); d) \right] \\
		= & \frac{1}{N^2} \sumij\E\left[\muitt\mujtt\right]- \frac{1}{N^2}\sumij\E\left[\muit \right]\E\left[\mujt \right].
	\end{align*}
	The first equality holds because of assumption C3 on local interference: for $j \notin \mathcal{B}(i;d)$, $\muitt =\muit$ and $\E\left[\muitt\mujtt \right] =\E[\muit]\E[\mujt]$, following the definition of interference in Section 4. Moreover,
	\begin{align*}
		\frac{1}{N^2} \sumij\E\left[\muitt\mujtt\right]- \frac{1}{N^2}\sumij\E\left[\muit \right]\E\left[\mujt \right]= O\left(1\right),
	\end{align*}
	since $|\mathcal{B}(i;d)|$ is bounded by (C4a). Other covariance terms have similar forms. We obtain the bound of the variance and its convergence rate by combining these terms together. 
\end{proof}
\subsubsection{Unbiasedness of the HT estimator in observaitional studies}\label{Section:HTobsproof}

\begin{proof}
	Note that in our setup the only randomness comes from the random assignment. Hence functions of the covariates are considered fixed.  In the scenario of observational studies and known propensity scores, we have
	\begin{align*}
		&	\textnormal{AME}(d;\eta)  = \frac{1}{N}\sum_{i=1}^N \mu_i(1; d, \eta) - \frac{1}{N}\sum_{i=1}^N \mu_i(0; d, \eta) \\
		& = \frac{1}{N}\sum_{i=1}^N \E\left[ \frac{p(\C) }{p(\C) }\mu_i(\Y(\mathbf{Z}); d)|Z_i=1\right] - \frac{1}{N}\sum_{i=1}^N \E\left[\frac{1-p(\mathbf{C}_i) }{1-p(\mathbf{C}_i) }\mu_i(\Y( \mathbf{Z}); d)|Z_i=0\right]\\
		& = \frac{1}{N}\sum_{i=1}^N\frac{p(\C) }{p(\C) } \E[Z_i\mu_i(\Y(\mathbf{Z}); d) | Z_i=1] -  \frac{1}{N}\sum_{i=1}^N\frac{1-p(\C) }{1-p(\C) } \E[(1-Z_i)\mu_i(\Y(\mathbf{Z}); d) | Z_i=0]   \\
		& = \E\left[ \frac{1}{N}\sum_{i=1}^N \frac{Z_i}{p(\C) } \mu_i(\Y; d) - \frac{1}{N}\sum_{i=1}^N \frac{1-Z_i}{p(\C)} \mu_i(\Y; d)\right]
	\end{align*}
	The third equality uses C\ref{assn:assignment_obsstudy} and the fourth equality uses C\ref{assn:assignment_obsstudy}-(ii) and the law of total expectations.
\end{proof}


%\begin{proof}
%Using the expression of the Horvitz-Thompson estimator, we have:
%\begin{align*}
%& \Var\left(\widehat{\tau}(d)  \right) \\
%= &\frac{1}{N^2} \Var\left[\sum_{i=1}^N \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y(\Z); d) \right] \\
%= & \frac{1}{N^2} \sum_{i=1}^N \Var\left[ \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y(\Z); d) \right] \\
%& + \frac{1}{N^2} \sum_{i=1}^N \sum_{j \neq i} \Cov\left[ \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y(\Z); d), \left(\frac{Z_j}{p} - \frac{1-Z_j}{1-p}\right)\mu_j(\Y(\Z); d) \right] \\
%= & \frac{1}{N^2} \sum_{i=1}^N \Var\left[ \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y(\Z); d) \right] \\
%& + \frac{1}{N^2} \sum_{i=1}^N \sum_{j \in \mathcal{B}(i;d)} \Cov\left[ \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y(\Z); d), \left(\frac{Z_j}{p} - \frac{1-Z_j}{1-p}\right)\mu_j(\Y(\Z); d) \right] \\
%= & \frac{1}{N}\times \frac{1}{N}\Var\left[ \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y(\Z); d) \right] \\
%+ & \frac{1}{N}\times \frac{1}{N}\sum_{i=1}^N \sum_{j\in\mathcal{B}(i;d)}\Cov\left[ \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y(\Z); d), \left(\frac{Z_j}{p} - \frac{1-Z_j}{1-p}\right)\mu_j(\Y(\Z); d) \right]\\
%= & \frac{1}{N}\times O(1) + \frac{1}{N}\times O(1),
%\end{align*}
%where for the last line we used C\ref{assn:bounded-y}-C\ref{assn:local-inf}. In particular the cardinally of $\mathcal{B}(i;d)$ is bounded for all $i=1,...,N$.
%\end{proof}

==> proofs/jp_mixing.tex <==

Jenish and Prucha (2009) provide a CLT for $\alpha$-mixing nonstationary random fields on potentially unevenly spaced lattices. For their central limit theorem to apply to our case, we need conditions that satisfy their Assumption 1, Corollary 1, Assumption 3(b), Assumption 3(c), and Assumption 5.  We need to do this on the $d$-radius circle averages.

We define the inferential setting in terms of a sequence of random fields indexed by $N$. We have a set of intervention points, $\mathcal{N}_N = \{1,...,N\}$.  Outcomes used to construct $d$-distance estimates are located at $\mathcal{X}_N(d) = \cup_{i=1}^N \mathcal{X}_{(i)}(d)$, where $\mathcal{X}_{(i)}(d)$ is the finite set of points at distance $d$ from intervention points $i$ used to construct each circle average $\mu_i(Y;d)$.  We have that $\mathcal{X}_N(d)$ and the locations of each $i \in \mathcal{N}_N$ are strict subsets of an infinite countable lattice $\mathcal{X} \subset \mathbb{R}^2$. For all $i,j \in \mathcal{N}$, we have a distance metric $\rho(i,j) = \max_{l \in \{1,2\}} |j_l - i_l|$.  The distance between subsets $U, V \in \mathcal{X}$ is given by $\rho(U,V) = \inf \{ \rho(i,j) : i \in U \text{ and } j \in V\}$.
%\min \{\max_{l \in \{1,2\}}|x'_l - x_l|; x \in \mathcal{X}_{(i)}(d), x' \in \mathcal{X}_{(j)}(d) \}$.

We define an increasing domain asymptotic growth process by assuming the following: 
\begin{assn}\label{assn:distance}
All unique elements in the array $\{\mathcal{N}_N, N \in \mathbb{N}\}$ have distance at least $\rho_0 > 0$ from each other.
\end{assn}

Following our definition of potential outcomes from the paper, we assume that treatment is assigned by the equivalent of independent coin flips:
\begin{assn}\label{assn:bern}
$(Z_1,...,Z_N)$ is a vector of i.i.d. $\text{Bernouilli}(p)$ draws.
\end{assn}

The next assumption ensures that moments of random variables constructed on the basis of potential outcomes are bounded:
\begin{assn}\label{assn:bounded}
$|Y_x(\mathbf{z})| < b$ for some real constant $b$ and all $x \in \mathcal{X}$ and $\mathbf{z} \in \mathcal{Z}$.
\end{assn}
This ensures that the first part of Jenish and Prucha's Corollary 1 holds.  To see this, define 
$$
\zeta_{i,N}(d) = \mu_i(Y(\mathbf{Z});d)\frac{Z_i - p}{p(1-p)} - \sum_{\mathbf{z} \in \mathcal{Z}} \mu_i(Y(\mathbf{z});d)\frac{z_i - p}{p(1-p)},
$$
where $(z_i - p)/p(1-p)$ is the Horvitz-Thompson transformation such that $N^{-1} \sum_{i=1}^N \zeta_{i,N}(d) = \widehat{\tau}(d) - \tau(d; \alpha)$.  The $\zeta_{i,N}(d)$ each have mean zero with respect to $\mathbf{Z}$ given that all $\mathbf{z} \in \mathcal{Z}$ are equally likely under Assumption \ref{assn:bern}. Then by Assumption \ref{assn:bounded}, it must be that $|\zeta_{i,N}(d)| < b$ and so the first part of Corollary 1 from Jenish and Prucha holds trivially for the $\zeta_{i,N}(d)$. Define $S_N(d) = \sum_{i=1}^N \zeta_{i,N}(d)$, which is the centered sum of treated circle averages, and $\sigma^2_N(d) = \text{Var}(S_N(d))$.

Next, we need to define $\alpha$-mixing for our case.  An $\alpha$-mixing coefficient is generically defined on a probability space $(\Omega, \mathcal{F}, P)$ for $\mathcal{U}, \mathcal{B} \in \mathcal{F}$ as,
$$
\alpha(\mathcal{U}, \mathcal{B}) = \sup(|P(A \cap B) - P(A)P(B)|, A \in \mathcal{U}, B \in \mathcal{B}).
$$
To apply this to our 2-dimensional random field, we need to define a few terms. First, define the random field,
$$
\{\zeta_{i,N}(d) : i \in \mathcal{N}_N, N \in \mathbb{N}\} = \{ \{X_{i,1} : i \in \mathcal{N}_1\}, \{X_{i,2} : i \in \mathcal{N}_2\},...\}
$$ 
as a triangular array of real random variables $\zeta_{i,N}(d)$ defined on the probability space $(\Omega, \mathcal{F}, P)$ at each point $i \in \mathcal{N}_N$, and where points in $\mathcal{N}_N$ are a finite subset of $\mathcal{X}$ satisfying Assumption \ref{assn:distance}.


For $U \subseteq \mathcal{N}_N$ and $V \subseteq \mathcal{N}_N$, define a sub-sigma-algebra operator $\sigma_N(U) = \sigma(\zeta_{i,N}(d); i \in U)$ and corresponding $\alpha_N(U,V) = \alpha(\sigma_N(U), \sigma_N(V))$.  	Then, the $\alpha$-mixing coefficient for the random field $\{\zeta_{i,N}(d) : i \in \mathcal{N}_N, N \in \mathbb{N}\}$ is,
	$$
	\alpha_{k,l,N}(r) = \sup(\alpha_N(U,V), |U| \le k, |V| \le l,  \rho(U,V) \ge r),
	$$
	with $k,l,r,N \in \mathbb{N}$.  To account for the dependence of the random field on $N$, Jenish and Prucha define,
	$$
	\overline{\alpha}_{k,l}(r) = \sup_N \alpha_{k,l,N}(r).
	$$
This is the maximal dependence of sets of size $k$ and $l$ where the distance between members of the sets can be as small as $r$.

We now collect assumptions corresponding to the second condition in Corollary 1 and Assumptions 3(b) and 3(c) from Jenish and Prucha:
\begin{assn}\label{assn:mixing}
Suppose for the random field $\{\zeta_{i,N}(d); i \in \mathcal{N}_N, N \in \mathbb{N}\}$ and some $\delta > 0$, we have:
\begin{enumerate}
\item $\sum_{m=1}^{\infty} \overline{\alpha}_{1,1}(m)m^{[d(2+\delta)/\delta]-1} <\infty$,
\item $\sum_{m=1}^{\infty} m^{d-1} \overline{\alpha}_{k,l}(m) < \infty$ for $k+l \le 4$, and
\item $\overline{\alpha}_{1,\infty}(m) = O(m^{- d-\epsilon})$ for some $\epsilon > 0$.
\end{enumerate}
\end{assn}
Of course, these mixing conditions follow trivially if the $\zeta_{i,N}(d)$s were independent at some strict cutoff in distance, as we propose in the main text. The proposition below is based on weaker assumptions.

Our final assumption is the asymptotic negligibility condition, corresponding to Assumption 5 from Jenish and Prucha's Theorem 1 and Corollary 1:
\begin{assn}\label{assn:variance}
$$
\lim \inf_{N \rightarrow \infty} \sigma^2_N(d) /N > 0.
$$
\end{assn}

We can now apply the CLT result to our case:
\begin{prop}\label{prop:CLT}
Suppose $\mathcal{N}_N$ is a sequence of arbitrary $N$ points located at subsets of $\mathcal{X}$, satisfying Assumption \ref{assn:distance}. Suppose as well that $\{\zeta_{i,N}(d); i \in \mathcal{N}_N, N \in \mathbb{N}\}$, as defined above, is an array of random variables satisfying Assumptions \ref{assn:bern} and \ref{assn:bounded}, that Assumption \ref{assn:variance} also holds, and that the random field is $\alpha$-mixing, satisfying Assumption \ref{assn:mixing}. Then, as $N \rightarrow \infty$, $S_N(d)/\sigma_N(d) \rightsquigarrow N(0,1)$.
\end{prop}

\begin{proof}
The result is based on Jenish and Prucha (2009, Theorem 1 and Corollary 1). Assumptions \ref{assn:distance}, \ref{assn:mixing}, and \ref{assn:variance} above are stated in directly analogous terms as Assumption 1, the second assumption of Corollary 1, Assumptions 3(b) and 3(c), and Assumption 5 from Jenish and Prucha (2009). As discussed above, Assumption 2 and the first assumption of Corollary 1 from Jenish and Prucha follow trivially when potential outcomes are bounded.
\end{proof}

==> proofs/reference/consistency-old.tex <==
\begin{proof}
We consider the convergence properties of
$$
\sqrt{N}(\widehat{\tau}(d) - \tau(d; \alpha)) = \sqrt{N}\left(\frac{1}{Np}\sum_{i=1}^N Z_i \mu_i(\Y; d) - \frac{1}{N(1-p)}\sum_{i=1}^N (1-Z_i) \mu_i(\Y; d) - \tau(d; \alpha) \right).
$$ 
By proposition \ref{prop:identification} this has mean zero.  The variance is equal to,
\begin{align}
N \Var\bigg[ \frac{1}{Np}\sum_{i=1}^N Z_i \mu_i(\Y; d) & - \frac{1}{N(1-p)}\sum_{i=1}^N (1-Z_i) \mu_i(\Y; d)\bigg] \nonumber \\
& = N \Var\left[ \frac{1}{Np}\sum_{i=1}^N Z_i \mu_i(\Y; d)\right] \nonumber \\
& \hspace{1em} + N \Var \left[ \frac{1}{N(1-p)}\sum_{i=1}^N (1-Z_i) \mu_i(\Y; d)\right]\nonumber  \\ 
& \hspace{1em} - 2N \Cov \left[ \frac{1}{Np}\sum_{i=1}^N Z_i \mu_i(\Y; d),\frac{1}{N(1-p)}\sum_{i=1}^N (1-Z_i) \mu_i(\Y; d)\right] .\label{eq:var}
\end{align}

Considering expression \ref{eq:var}, for the first term we have,
\begin{align*}
N \Var\left[ \frac{1}{Np}\sum_{i=1}^N Z_i \mu_i(\Y; d)\right] & = \frac{1}{Np^2} \Var\left[\sum_{i=1}^N Z_i \mu_i(\Y; d)\right]\\
& = \frac{1}{Np^2}\sum_{i=1}^N\sum_{j=1}^N\Cov\left[Z_i \mu_i(\Y; d), Z_j \mu_j(\Y; d)\right] \\
& = \frac{1}{Np^2}\sum_{i=1}^N\sum_{j=1}^N\Cov\left[Z_i \mu_i(\Y(1, \Z_{-i}); d), Z_j \mu_j(\Y(1, \Z_{-j}); d)\right] \\
& \le \frac{1}{Np^2} Nc(d)k =  \frac{c(d)k}{p^2},
\end{align*}
for $k >0$. By C2, $k$ is finite and bounded, and by C3, $c(d)$ is finite and bounded. By the same logic,
$$
N \Var\left[ \frac{1}{N(1-p)}\sum_{i=1}^N (1-Z_i) \mu_i(\Y; d)\right] \le \frac{c(d)k}{(1-p)^2}.
$$
Finally,
\begin{align*}
- 2N \Cov \bigg[ \frac{1}{Np}&\sum_{i=1}^N Z_i \mu_i(\Y; d), \frac{1}{N(1-p)}\sum_{i=1}^N (1-Z_i) \mu_i(Y; d)\bigg] \\
& = - \frac{2}{Np(1-p)}\sum_{i=1}^N \Cov[Z_i \mu_i(\Y(1, \Z_{-i}); d), (1-Z_i) \mu_i(\Y(0, \Z_{-i}); d)] \\
& \hspace{1em} - \frac{2}{Np(1-p)}  \sum_{i=1}^N\sum_{j\ne i} \Cov[Z_i \mu_i(\Y(1, \Z_{-i}); d), (1-Z_j) \mu_j(\Y(0, \Z_{-j}); d)] \\
& \le \frac{2k(1+ c(d))}{p(1-p)}
\end{align*}
by C2 and C3. Then, the condition $\frac{c(d)}{N} \rightarrow 0$ implies that that as $N \rightarrow \infty$, $\Var\left[\widehat{\tau}(d) - \tau(d; \alpha)\right] \rightarrow 0$.  Combining these results with the unbiasedness result from Proposition \ref{prop:identification} and Chebychev's inequality we have that $\widehat{\tau}(d) \overset{p}{\rightarrow} \tau(d; \alpha)$.
\end{proof}

==> proofs/reference/consistency.tex <==
\begin{proof}
Following \citet{chin2019-clt-interference}, we define 
\begin{align}
\mathcal{F} = \{ \mu_i(\Y(1, \Z_{-i});d), \mu_i(\Y(0, \Z_{-i});d), i \in \{1,2,...,N\}\}
\end{align}
and use the law of total variance to decompose $\Var[ \widehat{\tau}(d)]$ as
\begin{align}
\Var[\widehat{\tau}(d)] = \E[\Var[\widehat{\tau}(d) \mid \mathcal{F}]] + \Var[\E[\widehat{\tau}(d) \mid \mathcal{F}]] .\label{eq:var_dec}
\end{align}
The first part of \eqref{eq:var_dec} is the analogue to the Neyman variance, but for a Bernouilli design (by C1).  Under C1, the $\{Z_i\}$ are independent, and we have
\begin{align*}
\E\left[\Var[\widehat{\tau}(d) \mid \mathcal{F}]\right] 
	& = \E \left[ 
		\Var \left[ 
			\frac{1}{Np}\sum_{i=1}^NZ_i \mu_i(\Y(1, \Z_{-i});d) 
			- \frac{1}{N(1-p)}\sum_{i=1}^N (1-Z_i)\mu_i(\Y(0, \Z_{-i});d) 
			\mid \mathcal{F}  
		\right] 
	\right]\\
	& = \E \bigg[ 
		\frac{1}{N^2p^2} 
			\sum_{i=1}^N \Var \left[ Z_i \mu_i(\Y(1, \Z_{-i});d) \mid \mathcal{F} \right] \\
			& \hspace{2em} + \frac{1}{N^2(1-p)^2}\sum_{i=1}^N \Var \left[(1-Z_i)\mu_i(\Y(0, \Z_{-i});d) \mid \mathcal{F}\right] \\
			& \hspace{2em} - \frac{2}{N^2p(1-p)}\sum_{i=1}^N\sum_{j=1}^N \Cov\left[ Z_i \mu_i(\Y(1, \Z_{-i});d), (1-Z_i)\mu_i(\Y(0, \Z_{-i});d) \mid \mathcal{F} \right]
	\bigg] \\
	& = \frac{1-p}{N^2p} \sum_{i=1}^N \E\left[ \mu_i^2(\Y(1, \Z_{-i});d) \right] + \frac{p}{N^2(1-p)}\sum_{i=1}^N\E\left[\mu_i^2(\Y(0,\Z_{-i};d)\right]\\
	& \hspace{2em} + \frac{2}{N^2} \sum_{i=1}^N\E\left[ \mu_i(\Y(1,\Z_{-i});d)\mu_i(\Y(0,\Z_{-i});d)\right] \\
	& \le \frac{1}{N^2p} \sum_{i=1}^N \E\left[ \mu_i^2(\Y(1, \Z_{-i});d) \right] + \frac{1}{N^2(1-p)}\sum_{i=1}^N\E\left[\mu_i^2(\Y(0,\Z_{-i};d)\right] \\
	& \le \frac{b^2}{Np(1-p)},
\end{align*}
where the last line follows from C2.

The second part of \eqref{eq:var_dec} is the additional variance due to the interference.  We have 


\clearpage

We consider the convergence properties of
$$
\sqrt{N}(\widehat{\tau}(d) - \tau(d; \alpha)) = \sqrt{N}\left(\frac{1}{Np}\sum_{i=1}^N Z_i \mu_i(\Y; d) - \frac{1}{N(1-p)}\sum_{i=1}^N (1-Z_i) \mu_i(\Y; d) - \tau(d; \alpha) \right).
$$ 
By proposition \ref{prop:identification} this has mean zero.  The variance is equal to,
\begin{align}
N \Var\bigg[ \frac{1}{Np}\sum_{i=1}^N Z_i \mu_i(\Y; d) & - \frac{1}{N(1-p)}\sum_{i=1}^N (1-Z_i) \mu_i(\Y; d)\bigg] \nonumber \\
& = N \Var\left[ \frac{1}{Np}\sum_{i=1}^N Z_i \mu_i(\Y; d)\right] \nonumber \\
& \hspace{1em} + N \Var \left[ \frac{1}{N(1-p)}\sum_{i=1}^N (1-Z_i) \mu_i(\Y; d)\right]\nonumber  \\ 
& \hspace{1em} - 2N \Cov \left[ \frac{1}{Np}\sum_{i=1}^N Z_i \mu_i(\Y; d),\frac{1}{N(1-p)}\sum_{i=1}^N (1-Z_i) \mu_i(\Y; d)\right] .\label{eq:var}
\end{align}

Considering expression \ref{eq:var}, for the first term we have,
\begin{align*}
N \Var\left[ \frac{1}{Np}\sum_{i=1}^N Z_i \mu_i(\Y; d)\right] & = \frac{1}{Np^2} \Var\left[\sum_{i=1}^N Z_i \mu_i(\Y; d)\right]\\
& = \frac{1}{Np^2}\sum_{i=1}^N\sum_{j=1}^N\Cov\left[Z_i \mu_i(\Y; d), Z_j \mu_j(\Y; d)\right] \\
& = \frac{1}{Np^2}\sum_{i=1}^N\sum_{j=1}^N\Cov\left[Z_i \mu_i(\Y(1, \Z_{-i}); d), Z_j \mu_j(\Y(1, \Z_{-j}); d)\right] \\
& \le \frac{1}{Np^2} Nc(d)k =  \frac{c(d)k}{p^2},
\end{align*}
for $k >0$. By C2, $k$ is finite and bounded, and by C3, $c(d)$ is finite and bounded. By the same logic,
$$
N \Var\left[ \frac{1}{N(1-p)}\sum_{i=1}^N (1-Z_i) \mu_i(\Y; d)\right] \le \frac{c(d)k}{(1-p)^2}.
$$
Finally,
\begin{align*}
- 2N \Cov \bigg[ \frac{1}{Np}&\sum_{i=1}^N Z_i \mu_i(\Y; d), \frac{1}{N(1-p)}\sum_{i=1}^N (1-Z_i) \mu_i(Y; d)\bigg] \\
& = - \frac{2}{Np(1-p)}\sum_{i=1}^N \Cov[Z_i \mu_i(\Y(1, \Z_{-i}); d), (1-Z_i) \mu_i(\Y(0, \Z_{-i}); d)] \\
& \hspace{1em} - \frac{2}{Np(1-p)}  \sum_{i=1}^N\sum_{j\ne i} \Cov[Z_i \mu_i(\Y(1, \Z_{-i}); d), (1-Z_j) \mu_j(\Y(0, \Z_{-j}); d)] \\
& \le \frac{2k(1+ c(d))}{p(1-p)}
\end{align*}
by C2 and C3. Then, the condition $\frac{c(d)}{N} \rightarrow 0$ implies that that as $N \rightarrow \infty$, $\Var\left[\widehat{\tau}(d) - \tau(d; \alpha)\right] \rightarrow 0$.  Combining these results with the unbiasedness result from Proposition \ref{prop:identification} and Chebychev's inequality we have that $\widehat{\tau}(d) \overset{p}{\rightarrow} \tau(d; \alpha)$.
\end{proof}

==> proofs/reference/normality_old.tex <==
\input{tex-header}
\begin{document}
The consistency of the proposed estimator follows from the fact that both $\Var(\widehat{\tau}(d))$ and $\Var(\widehat{\tau}_{HA}(d))$ converge to zero as $N \rightarrow \infty$ under conditions C1-C4. The asymptotic normality of the Horvitz-Thompson estimator can be derived using classic central limit theorems for dependent random variables \citet{ross2011fundamentals}. Proving the asymptotic normality of the Hajek estimator is more challenging since the denominators $N_1$ and $N_0$ are decided by the entire assignment vector. Hence, any two terms in the summand of $\widehat{\tau}_{HA}(d)$ are always dependent. We rely on a result in  \citet{chatterjee2014-stein} for the proof. This result is an extension of Stein's method and has been used by \citet{chin2019-clt-interference} in a similar setting. Below we introduce some necessary concepts and restate the result in \citet{chatterjee2014-stein}.

Suppose $\Z = (Z_1,...,Z_N) \in \mathcal{Z}^N$ is a vector of independent random variables on a sample space $\mathcal{Z}$ and $f : \mathcal{Z}^N \rightarrow \mathbb{R}$ be a scalar-valued measurable function. Denote any independent copy of $\Z$ as $\Z^{'} = (Z_{1}^{'},...,Z_{N}^{'}) $. For any finite set $A \subset \{1,2,\dots,N\}$, define $\Z^{A}$ as the vector obtained by swapping out $Z_i$ for $Z_{i}^{'}$  in $\Z$ when $i \in A$. In other words,
\begin{align*}
Z_{i}^{A} = \begin{cases} 
Z_i^{'} \text{  if } i \in A \\
Z_{i}  \text{  if } i \notin A
\end{cases}.
\end{align*}
Further define $\Delta_i f = f(\Z) - f(\Z^i)$ for any $i \in \{1,2,\dots,N\}$ and  $\Delta_i f^A = f(\Z) - f(\Z^A \cup i)$ for any $A \subset \{1,\dots,i-1,i+1,\dots,N\}$. These quantities measure the response of $f$ to the perturbations of $\Z$ in some elements ($\{i\}$ or $A$). Now we state the lemma adapted from \citet{chatterjee2014-stein}:

\begin{lemma}(Chatterjee (2014), Corollary 3.2)\label{lemma:cha-2014}
Let $\Z = (Z_1 , . . . , Z_N )$ be a vector of independent real-valued random variables, and let $S = f(\Z)$. Suppose $E[S] = 0$ and $\sigma^2 := E[S^2] < \infty$. For every $i,j$, let $c_{i,j}$ be a constant such that for all $A \in \{1,2,\dots,N\} \setminus \{i\}$ and $B \in \{1,2,\dots,N\} \setminus \{j\}$,
$$
Cov(\Delta_i f \Delta_i f^A, \Delta_j f \Delta_j f^B) \leq c_{ij}.
$$
Then
$$
d_{\mathcal{W}}(S/\sigma) \leq \frac{1}{2\sigma^2}\left(\sum_{i=1}^N \sum_{j=1}^N c_{ij}\right)^{1/2} + \frac{1}{2\sigma^3}\sum_{i=1}^N \E\left[|\Delta_i f|^3 \right].
$$
where $d_{\mathcal{W}}(S/\sigma)$ Wasserstein metric between $S/\sigma$ and the standard normal distribution.
\end{lemma}

Define $S = f(\Z)\sqrt{N} = (\widehat{\tau}_{HA}(d) - \tau(d;\alpha)) $. From previous discussions, we know that $S$ satisfies conditions required by Lemma \ref{lemma:cha-2014}. Hence, the Wasserstein distance between $S$ and the standard normal distribution is bounded by the two terms $\left(\sum_{i=1}^N \sum_{j=1}^N c_{ij}\right)^{1/2}$ and $\sum_{i=1}^N \E\left[|\Delta_i f|^3 \right]$. All we need to show is that both terms converge to zero as $N \rightarrow \infty$.

In what remains of this section, we treat the circle averages, which we will denote using the shorthand $\{\mu_i\}_{1:N}$, as observed outcomes. (Note that we are economizing on notation by removing the explicit reference to $d$.) We then complete the proof by showing that under conditions C1-C4, $d_{\mathcal{W}}(S/\sigma) \rightarrow 0$.  A crucial requirement is C4, which we used in the consistency results above, but only with regard to its implications for covariances across intervention nodes.  For this CLT result, the full independence-type implications of C4 are crucial. 

\begin{proof}
First we need to define several auxillary concepts. Define $H_N$ as a undirected graph on the $N$ intervention nodes which represents a dependency graph for ``strong interference." The neighborhood of unit $i$ on $H_N$ is denoted by $\mathcal{N}_{i}^{H_N} = \{j \in \mathcal{N}: (H_N)_{ij} = 1\}$.

 \citet{chin2019-clt-interference} proves that both the Horvitz-Thompson and the Hajek estimators converge to the normal distribution (after rescaled by $\sqrt{N}$) under the following assumptions:

\begin{description}
\item[A1.] (Bernoulli design.) $Z_i \sim \text{Bernoulli}(p)$ for $i=1,...,N$.
\item[A2.] (Bounded fourth moments.) $\E|\mu_i^k(\z)| < b$ for some finite real constant $b$ and all $i \in \{1,2,\dots,N\}$ and $k \leq 4$.
\item[A3.] (Covariance regularity conditions.) The following covariance constraints hold: \\
(a) $\sum_{i=1}^{N} \sum_{j=1}^{N} |\Cov(\mu_i, \mu_j)| = o(N^2)$. \\
(b) $\sum_{i=1}^{N} \sum_{r\neq i} \sum_{j \neq i}  |\Cov(\Delta_i \mu_r, \mu_j)| = o(N^2)$. \\
(c) $\sum_{i=1}^{N} \sum_{j=1}^{N} \sum_{r\neq i} \sum_{s \neq i, s \neq r}  |\Cov(\Delta_i \mu_r, \Delta_j \mu_s)| = o(N^2)$. \\
\item[A4.] (Approximate local interference.) There exists a sequence of graphs $\{H_N\}_{N=1}^{\infty}$ having maximal
degree sequence $h_N = o(N^{1/3})$ such that:
\begin{align*}
\max \Bigg\{\sum_{r \notin \mathcal{N}_{i}^{H_N}} |\Delta_i \mu_r|, \sum_{r \notin \mathcal{N}_{i}^{H_N}}|\Delta_r \mu_i|\Bigg\} \rightarrow 0
\end{align*}
almost surely for every $i$.
\end{description}

Now let's prove that the circle averages defined in the paper satisfy the four assumptions. Notice that A1 is the same as C1 in the paper, and A2 holds due to the boundedness of the outcome values, C2. 

To see that A3 holds, notice that the boundedness of $Y_x$ implies the boundedness of $\mu_i$, as well as all the relevant moments:
\begin{align*}
& |\mu_i| = \lvert \frac{\sum_x 1(d_i(x) = d) Y_{x}}{\sum_x 1(d_i(x) = d)}\lvert \leq b \\
& \lvert \E\mu_i \lvert = \lvert \sum_{\mathbf{z} \in \mathbf{Z}}p(\mathbf{Z} = \mathbf{z}) \mu_i(\mathbf{z}) \lvert \leq b \\
&\Var \mu_i \leq \lvert \E\mu_i^2 \lvert = \lvert \sum_{\mathbf{z} \in \mathbf{Z}}p(\mathbf{Z} = \mathbf{z}) \mu_i^2(\mathbf{z}) \lvert \leq b^2.
\end{align*}
Before stating Lemma \ref{lemma:ht-var}, we defined $\mathbf{B}(i;d) = \{j : ||x(i) - x(j)|| - d \le h(d)\}$, the set of intervention points in the interference region of $i$ for the circle average of radius $d$, as assumed under condition C3. Also, by C4, for any $i$, $c_i(d) = |\mathbf{B}(i;d)|\leq \tilde c$.    

Now, for the three conditions in A3, we have:
\begin{align*}
& \frac{1}{N^2}\sum_{i=1}^{N} \sum_{j=1}^{N} |\Cov(\mu_i, \mu_j)|= \frac{1}{N^2}\sum_{i=1}^{N} \sum_{j \in \mathbf{B}(i)} |\Cov(\mu_i, \mu_j)| \\
\leq & \frac{1}{N^2}\sum_{i=1}^{N} \sum_{j \in \mathbf{B}(i)} b^2 = \frac{b^2\sum_{i=1}^{N} c_i }{N^2} = o_P(1),
\end{align*}
\begin{align*}
& \frac{1}{N^2}\sum_{i=1}^{N} \sum_{r\neq i} \sum_{j \neq i}  |\Cov(\Delta_i \mu_r, \mu_j)| = \frac{1}{N^2}\sum_{i=1}^{N} \sum_{r \in  \mathbf{B}(i)} \sum_{j \neq i, j \in  \mathbf{B}(r)}  |\Cov(\Delta_i \mu_r, \mu_j)| \\
\leq & \frac{\sum_{i=1}^{N} \tilde c c_i 2b^2}{N^2} = o_P(1),
\end{align*}
\begin{align*}
& \frac{1}{N^2}\sum_{i=1}^{N} \sum_{j=1}^{N} \sum_{r\neq i} \sum_{s \neq i, s \neq r}  |\Cov(\Delta_i \mu_r, \Delta_j \mu_s)| = \frac{1}{N^2}\sum_{i=1}^{N} \sum_{r \in  \mathbf{B}(i)} \sum_{s \in  \mathbf{B}(r)}\sum_{j \in  \mathbf{B}(s)}  |\Cov(\Delta_i \mu_r, \Delta_j \mu_s)| \\
\leq & \frac{\sum_{i=1}^{N} \tilde c^2 c_i 2b^2}{N^2} = o_P(1).
\end{align*}
using conditions C2 to C4. 

A4 holds as $\max h_N = \tilde c$ in our case, which goes to zero at the speed $N^{\varepsilon}$, for any $\varepsilon > 0$, and
\begin{align*}
\max \Bigg\{\sum_{r \notin \mathcal{N}_{i}^{H_N}} |\Delta_i \mu_r|, \sum_{r \notin \mathcal{N}_{i}^{H_N}}|\Delta_r \mu_i|\Bigg\} = 0.
\end{align*}

%Define 
%\begin{align*}
%f_n (\mathbf{Z}) = & \sqrt{N}(\hat \tau_{HT, d} - \tau_d) \\ 
%= & \sqrt{N} \left[\frac{1}{Np}\sum_{i=1}^N Z_i\mu_i(1, \mathbf{Z}_{-i}; d) - \frac{1}{N(1-p)}\sum_{i=1}^N (1-Z_i)\mu_i(0, \mathbf{Z}_{-i}; d)\right] - \sqrt{N}\tau_d.
%\end{align*}
%Denote $Z_{i}^{'}$ as an independent copy of $Z_i$ and $\Z^{i}$ as the treatment vector obtained by swapping out $Z_i$ for $Z_{i}^{'}$  in $\Z$.

%In other words,
%\begin{align*}
%Z_{j}^{i} = \begin{cases} 
%Z_j \text{  if } j=i \\
%Z_{j}^{'}  \text{  if } j \neq i
%\end{cases}.
%\end{align*}

\end{proof}

\end{document}




==> proofs/reference/regression-hac_old.tex <==
We analyze the approach of estimating of $\tau(d;\alpha)$ using a two-step process. In the first step, we transform all the outcomes into the circle mean for each intervention node: $\mu_i(d) = \frac{\sum_x \mathbf{1}\{d_{i}(x) = d\}Y_x}{\sum_x \mathbf{1}\{d_{i}(x) = d\}}$. In the second step, we apply the Horvitz-Thompson estimator or the Hajek estimator to all the $(Z_i, \mu_i(d))$.

It is well-known that regression could be used to generate unbiased estimate of the average treatment effect in experiments. Treating $\mu_i(d)$ as the outcome, we can estimate the following regression equation:

\begin{align*}
\mu_i(d) = \zeta(d) + \tau(d) Z_i + \varepsilon_i(d).
\end{align*}

It is easy to show that under OLS, $\hat{\zeta}(d) = \frac{1}{N_0}\sum_{i=1}^{N} (1-Z_i) \mu_i(d) = \bar{\mu}_0(d)$ and $\hat{\tau}_{OLS}(d) = \frac{1}{N_1}\sum_{i=1}^{N} Z_i \mu_i(d) - \frac{1}{N_0}\sum_{i=1}^{N} (1-Z_i) \mu_i(d) = \bar{\mu}_1(d) - \bar{\mu}_0(d)$, where $N_0 = \sum_{i=1}^{N} (1-Z_i)$ and $N_1 = \sum_{i=1}^{N}Z_i$. Clearly, $\hat{\tau}_{OLS}(d) = \widehat{\tau}_{HA}(d)$. Then the residual for each observation $\hat{e}_i(d) = \mu_i(d) - \hat{\zeta}(d) - \hat{\tau}_{OLS}(d) Z_i = \mu_i(d) - \bar{\mu}_0(d) - [\bar{\mu}_1(d) - \bar{\mu}_0(d)] Z_i $. 
%The strong law of large numbers renders that as $N \rightarrow \infty$, $\bar{\mu}_1(d) \overset{a.s.}{\rightarrow} \frac{\sum_{i=1}^N \E\left[\mu_i (1,\mathbf{Z}_{-i};d) \right]}{N}$ and $\bar{\mu}_0(d) \overset{a.s.}{\rightarrow} \frac{\sum_{i=1}^N \E\left[\mu_i (0,\mathbf{Z}_{-i};d) \right]}{N}$.

Denote $\begin{pmatrix}
1, Z_1 \\
1, Z_2 \\
\dots \\
1, Z_N
\end{pmatrix}$ as $\mathbf{X}$, the spatial HAC standard errors of $(\hat{\zeta}(d), \hat{\tau}_{OLS}(d))$ can be expressed as:

\begin{align*}
\sigma \begin{pmatrix}
\hat{\zeta}(d) \\
\hat{\tau}_{OLS}(d)
\end{pmatrix} = & \sqrt{\Var \begin{pmatrix}
\hat{\zeta}(d) \\
\hat{\tau}_{OLS}(d)
\end{pmatrix}} \\
 \widehat{\Var} \begin{pmatrix}
\hat{\zeta}(d) \\
\hat{\tau}_{OLS}(d)
\end{pmatrix} = & (\mathbf{X}' \mathbf{X})^{-1}(\mathbf{X}' \Sigma \mathbf{X})(\mathbf{X}' \mathbf{X})^{-1} \\
= & \begin{pmatrix}
N, N_1 \\
N_1, N_1
\end{pmatrix}^{-1}\left(\sum_{i=1}^N \sum_{j=1}^N \mathbf{X}_{i} \mathbf{X}_{j}^{'}\hat{e}_i(d) \hat{e}_j(d) \mathbf{1}\{j \in \mathbf{B}(i; d) \}\right)\begin{pmatrix}
N, N_1 \\
N_1, N_1
\end{pmatrix}^{-1} \\
= & \frac{1}{N_1^2 N_0^2}\begin{pmatrix}
N_1, -N_1 \\
-N_1, N
\end{pmatrix}\left(\sum_{i=1}^N \sum_{j=1}^N \begin{pmatrix}
1, Z_j \\
Z_i, Z_i Z_j
\end{pmatrix}\hat{e}_i(d) \hat{e}_j(d) \mathbf{1}\{j \in \mathbf{B}(i; d) \}\right)\begin{pmatrix}
N_1, -N_1 \\
-N_1, N
\end{pmatrix}
\end{align*}
Note that the $(2,2)$ entry of $\begin{pmatrix}
N_1, -N_1 \\
-N_1, N
\end{pmatrix} \begin{pmatrix}
1, Z_j \\
Z_i, Z_i Z_j
\end{pmatrix} \begin{pmatrix}
N_1, -N_1 \\
-N_1, N
\end{pmatrix}$ equals to $N_1^2 - N_1 N Z_i - - N_1 N Z_j + N^2 Z_i Z_j$. Rearrange the sample such that treated observations lie before observations under control and plug in the expression of $\hat{e}_i(d)$ , we can see that:
\begin{align*}
& \widehat{\Var}(\hat{\tau}_{OLS}(d)) \\
= & \frac{1}{N_1^2} \sum_{i=1}^{N_1} \hat{e}_i(d)^2 + \frac{1}{N_0^2} \sum_{i=N_1+1}^{N} \hat{e}_i(d)^2 + \frac{1}{N_1^2} \sum_{i=1}^{N_1} \sum_{j \neq i, Z_j = 1}\hat{e}_i(d)\hat{e}_j(d) \\
- & \frac{1}{N_1 N_0} \sum_{i=1}^{N_1} \sum_{j \neq i, Z_j = 0}\hat{e}_i(d)\hat{e}_j(d) - \frac{1}{N_1 N_0} \sum_{i=N_1+1}^{N} \sum_{j \neq i, Z_j = 1}\hat{e}_i(d)\hat{e}_j(d)  + \frac{1}{N_0^2} \sum_{i=N_1+1}^{N} \sum_{j \neq i, Z_j = 0}\hat{e}_i(d)\hat{e}_j(d) \\
= & \frac{1}{N_1^2} \sum_{i=1}^{N_1} \left(\mu_i (d) - \bar{\mu}_1 (d)\right)^2 + \frac{1}{N_0^2} \sum_{i=N_1+1}^{N} \left(\mu_i (d) - \bar{\mu}_0 (d)\right)^2  \\
+ & \frac{1}{N_1^2} \sum_{i=1}^{N_1} \sum_{j \in \mathbf{B}(i; d), Z_j = 1} \left(\mu_i (d) - \bar{\mu}_1 (d)\right) \left(\mu_j (d) - \bar{\mu}_1 (d)\right) \\
- & \frac{1}{N_1 N_0} \sum_{i=1}^{N_1} \sum_{j \in \mathbf{B}(i; d), Z_j = 0} \left(\mu_i (d) - \bar{\mu}_1 (d)\right) \left(\mu_j (d) - \bar{\mu}_0 (d)\right) \\
- & \frac{1}{N_1 N_0} \sum_{i=N_1+1}^{N} \sum_{j \in \mathbf{B}(i; d), Z_j = 1} \left(\mu_i (d) - \bar{\mu}_0 (d)\right) \left(\mu_j (d) - \bar{\mu}_1 (d)\right) \\
+ & \frac{1}{N_0^2} \sum_{i=N_1+1}^{N} \sum_{j \in \mathbf{B}(i; d), Z_j = 0} \left(\mu_i (d) - \bar{\mu}_0 (d)\right) \left(\mu_j (d) - \bar{\mu}_0 (d)\right)
\end{align*}

Finally, we show that the variance estimate $\widehat{\Var}(\hat{\tau}_{OLS}(d))$ is asymptotically unbiased for the true variance of the Hajek estimator, $\Var(\widehat{\tau}_{HA}(d))$ under C5, the assumption on homogeneous local interference.  Note that the first part in the true variance for the Hajek estimator can be written as:
\begin{align*}
& \frac{1}{N^2p}\sum_{i=1}^N \E\left[\left(\mu_i(\Y(1, \Z_{-i}); d)- \bar {\mu}_1\right)^2\right] \\
= & \frac{1}{N^2p}\sum_{i=1}^N \E\left[\mu_i^2(\Y(1, \Z_{-i}); d)\right] - \frac{2}{N^2p}\sum_{i=1}^N \E\left[\mu_i(\Y(1, \Z_{-i}); d)\frac{1}{N}\sum_{i=1}^N \mu_i(\Y(1, \Z_{-i}); d)\right] \\
& + \frac{1}{N^2p}\sum_{i=1}^N \E\left[\left(\frac{1}{N}\sum_{i=1}^N \mu_i(\Y(1, \Z_{-i}); d)\right)^2\right] \\
= & \frac{1}{N^2p}\sum_{i=1}^N \E\left[\mu_i^2(\Y(1, \Z_{-i}); d)\right]  - \frac{1}{N^3p} \E\left[\left(\sum_{i=1}^N \mu_i(\Y(1, \Z_{-i}); d)\right)^2\right] \\
= & \frac{1}{N^2p}(1-\frac{1}{N})\sum_{i=1}^N \E\left[\mu_i^2(\Y(1, \Z_{-i}); d)\right] - \frac{1}{N^3p}\sum_{i=1}^N \sum_{j\neq i}^N \E\left[\mu_i(\Y(1, \Z_{-i}); d)\mu_j(\Y(1, \Z_{-j}); d)\right] \\
= & \frac{1}{N^2p}(1-\frac{1}{N})\sum_{i=1}^N \E\left[\mu_i^2(\Y(1, \Z_{-i}); d)\right] - \frac{1}{N^3p}\sum_{i=1}^N \sum_{j\neq i}^N \E\left[\mu_i(\Y(1,1, \Z_{-i}); d)\mu_j(\Y(1,1, \Z_{-j}); d)\right]
\end{align*}

Taking expectation on the first term of the variance estimate, we have:
% Note that $\E\left[\frac{N_1^2}{N^2} \right] = p$, 
%\begin{align*}
%& \E\left[ \sum_{i=1}^{N_1} \left(\mu_i (d) - \bar{\mu}_1 (d)\right)^2\right] \\
%= & \E\left[ \sum_{i=1}^{N} Z_i\left(\mu_i (\Y(1, \mathbf{Z}_{-i});d) - \bar{\mu}_1 (d)\right)^2\right] \\
%= & \sum_{i=1}^{N}\E\left[Z_i \left(\mu_i (\Y(1, \mathbf{Z}_{-i});d) - \bar{\mu}_1 (d)\right)^2\right] \\
%= & p\sum_{i=1}^{N}\E\left[\left(\mu_i (\Y(1, \mathbf{Z}_{-i});d) - \bar{\mu}_1 (d)\right)^2\right]
%\end{align*}
%and $\E\left[ N_1^2\right] = N^2 p^2$. Therefore,
%\begin{align*}
%& \E\left[\frac{1}{N_1^2} \sum_{i=1}^{N_1} \left(\mu_i (d) - \bar{\mu}_1 (d)\right)^2\right] \\
%\rightarrow & \frac{p\sum_{i=1}^{N}\E\left[\left(\mu_i (\Y(1, \mathbf{Z}_{-i});d) - \bar{\mu}_1 (d)\right)^2\right]}{N^2 p^2}  \\
%= & \frac{1}{N^2 p}\sum_{i=1}^{N}\E\left[\left(\mu_i (\Y(1, \mathbf{Z}_{-i});d) - \bar{\mu}_1 (d)\right)^2 \right]
%\end{align*}
%Similarly,
%\begin{align*}
%& \E\left[\frac{1}{N_0^2} \sum_{i=N_1+1}^{N} \left(\mu_i (d) - \bar{\mu}_1 (d)\right)^2\right] \\
%\rightarrow & \frac{(1-p)\sum_{i=1}^{N}\E\left[\left(\mu_i (0, \mathbf{Z}_{-i};d) - \bar{\mu}_0 (d)\right)^2\right]}{N^2 (1-p)^2}  \\
%= & \frac{1}{N^2 (1-p)}\sum_{i=1}^{N}\E\left[\left(\mu_i (0, \mathbf{Z}_{-i};d) - \bar{\mu}_0 (d)\right)^2 \right]
%\end{align*}
%and
%\begin{align*}
%& \E\left[\frac{1}{N_1^2} \sum_{i=1}^{N_1} \sum_{j \in \mathbf{B}(i; d), Z_j = 1} \left(\mu_i (d) - \bar{\mu}_1 (d)\right) \left(\mu_j (d) - \bar{\mu}_1 (d)\right)\right] \\
%\rightarrow & \frac{p^2 \sum_{i=1}^{N}\E\left[\left(\mu_i (d) - \bar{\mu}_1 (d)\right) \left(\mu_j (d) - \bar{\mu}_1 (d)\right)\right]}{N^2 p^2}  \\
%= & \frac{1}{N^2}\sum_{i=1}^{N}\E\left[\left(\mu_i (d) - \bar{\mu}_1 (d)\right) \left(\mu_j (d) - \bar{\mu}_1 (d)\right)\right]
%\end{align*}
\begin{align*}
& \E\left[\frac{1}{N_1^2} \sum_{i=1}^{N_1} \left(\mu_i (d) - \bar{\mu}_1 (d)\right)^2\right] = \E\left[\frac{1}{N_1^2} \sum_{i=1}^{N_1} \left(\mu_i (\Y(1, \mathbf{Z}_{-i});d) - \bar{\mu}_1 (d)\right)^2\right] \\
= & \E\left[\frac{1}{N_1^2} \left(\sum_{i=1}^{N_1} \mu_i^2 (\Y(1, \mathbf{Z}_{-i});d) - 2\bar{\mu}_1 (d)\sum_{i=1}^{N_1}\mu_i (\Y(1, \mathbf{Z}_{-i});d) + \sum_{i=1}^{N_1}(\bar{\mu}_1 (d))^2 \right)\right] \\
= & \E\left[\frac{1}{N_1^2} \left(\sum_{i=1}^{N_1} \mu_i^2 (\Y(1, \mathbf{Z}_{-i});d) - N_1\bar{\mu}_1^2 (d)\right)\right] \\
= & \E\left[\frac{1}{N_1^2} \sum_{i=1}^{N_1} \mu_i^2 (\Y(1, \mathbf{Z}_{-i});d) \right] - \E\left[\frac{1}{N_1}\bar{\mu}_1^2 (d)\right] \\
= & \E\left[\frac{1}{N_1^2}(1-\frac{1}{N_1}) \sum_{i=1}^{N_1} \mu_i^2 (\Y(1, \mathbf{Z}_{-i});d) \right] - \E\left[\frac{1}{N_1^3}\sum_{i=1}^{N_1}\sum_{j\neq i}^{N_1} \mu_i (\Y(1, \mathbf{Z}_{-i});d) \mu_j (\Y(1, \mathbf{Z}_{-j});d)\right] \\
= & \frac{1}{N^2p^2}(1-\frac{1}{N}) \sum_{i=1}^{N} \E\left[  Z_i\mu_i^2 (\Y(1, \mathbf{Z}_{-i});d)\right] \\
& - \frac{1}{N^3p^3}\sum_{i=1}^{N}\sum_{j\neq i}^{N} \E\left[  Z_iZ_j\mu_i (\Y(Z_i, \mathbf{Z}_{-i});d) \mu_j (\Y(Z_j, \mathbf{Z}_{-j});d)\right] +o_P(1)  \\
= & \frac{1}{N^2p}(1-\frac{1}{N}) \sum_{i=1}^{N} \E\left[ \mu_i^2 (\Y(1, \mathbf{Z}_{-i});d)\right] \\
& - \frac{1}{N^3p}\sum_{i=1}^{N}\sum_{j\neq i}^{N} \E\left[  \mu_i (\Y(1,1, \mathbf{Z}_{-(i,j)});d) \mu_j (\Y(1, 1,\mathbf{Z}_{-(i,j)});d)\right]  +o_P(1)
\end{align*}
which is exactly the first part of the Hajek estimator's variance in the limit.

The second part can be shown to be asymptotically unbiased only when C5 holds. Now consider the first covariance part in the true variance, we have:
\begin{align*}
& \frac{1}{N^2} \sum_{i=1} \sum_{j \in \mathbf{B}(i; d)} \Cov[\mu_i(\Y(1, \Z_{-i}); d), \mu_j(\Y(1, \Z_{-j}); d)] \\
= & \frac{1}{N^2} \sum_{i=1} \sum_{j \in \mathbf{B}(i; d)} \E[\mu_i(\Y(1, \Z_{-i}); d)\mu_j(\Y(1, \Z_{-j}); d)] \\
& - \frac{1}{N^2} \sum_{i=1}\E[\mu_i(\Y(1, \Z_{-i}); d)] \sum_{j \in \mathbf{B}(i; d)} \E[\mu_j(\Y(1, \Z_{-j}); d)] \\
= &  \frac{1}{N^2} \sum_{i=1} \sum_{j \in \mathbf{B}(i; d)} \E[\mu_i(\Y(1, \Z_{-i}); d)\mu_j(\Y(1, \Z_{-j}); d)] \\
& - \left(\frac{1}{N} \sum_{i=1}\E[\mu_i(\Y(1, \Z_{-i}); d)]c_i(d)\right)\left(\frac{1}{N^2} \sum_{i=1} \frac{1}{c_i(d)} \sum_{j \in \mathbf{B}(i)} \E[\mu_j(\Y(1, \Z_{-j}); d)]\right) + o_P(N^{-1}) \\
= &  \frac{1}{N^2} \sum_{i=1} \sum_{j \in \mathbf{B}(i; d)} \E[\mu_i(\Y(1, \Z_{-i}); d)\mu_j(\Y(1, \Z_{-j}); d)] \\
& - \left(\frac{1}{N} \sum_{i=1}\E[\mu_i(\Y(1, \Z_{-i}); d)]\right)\left(\frac{c(d)}{N^2} \sum_{i=1} \E[\mu_j(\Y(1, \Z_{-j}); d)]\right) + o_P(N^{-1}).
\end{align*}.
The second and the third equality uses the two assumptions in C5, respectively.

Noticing that $\sum_{i=1}^{N_1}\sum_{j \in \mathcal{B}(i), Z_j = 1} \mu_i (d) = \sum_{i=1}^{N_1}\sum_{j \in \mathcal{B}(i), Z_j = 1} \mu_j (d) = \sum_{i=1}^{N_1} c_i^1 \mu_i (d)$, where $c_i^1 = \sum_{j \in \mathcal{B}(i)} Z_j$ is the number of treated nodes that depend on node $i$. It is also easy to see that $\frac{c_i^1}{c_i} = \frac{\sum_{j \in \mathcal{B}(i) } Z_j}{c_i} = p + o_P(1)$.  Then, the expectation of the corresponding estimate equals to:
\begin{align*}
&\E\left[ \frac{1}{N_1^2} \sum_{i=1}^{N_1} \sum_{j \in \mathcal{B}(i), Z_j = 1} \left(\mu_i (d) - \bar{\mu}_1 (d)\right) \left(\mu_j (d) - \bar{\mu}_1 (d)\right)\right]\\
= & \E\left[ \frac{1}{N^2p^2} \sum_{i=1}^{N_1} \sum_{j \in \mathcal{B}(i), Z_j = 1} \left(\mu_i (d) - \bar{\mu}_1 (d)\right) \left(\mu_j (d) - \bar{\mu}_1 (d)\right)\right]  + o_P(1) \\
= & \frac{1}{N^2 p^2} \sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)} \E \left[Z_iZ_j\mu_i (1, \mathbf{Z}_{-i};d)\mu_j (1, \mathbf{Z}_{-j};d)\right] \\
& - \frac{1}{N^2 p^2} \E \left[\sum_{i=1}^{N_1}\sum_{j \in \mathcal{B}(i), Z_j = 1} \bar{\mu}_1 (d) \left(\mu_i (d) - \bar{\mu}_1 (d) +\mu_j (d)\right) \right]  + o_P(1) \\
= & \frac{1}{N^2} \sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)} \E \left[\mu_i (1, 1, \mathbf{Z}_{-(i,j)};d)\mu_j (1, 1, \mathbf{Z}_{-(i,j)};d)\right] \\
& - \frac{1}{N^2 p^2} \E \left[\bar{\mu}_1 (d) \sum_{i=1}^{N_1}\left(2c_i^1  -  \frac{\sum_{i=1}^{N_1}c_i^1}{N_1} \right)\mu_i (d)\right]  + o_P(1) \\
= & \frac{1}{N^2} \sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)} \E \left[\mu_i (1, 1, \mathbf{Z}_{-(i,j)};d)\mu_j (1, 1, \mathbf{Z}_{-(i,j)};d)\right] \\
& -\frac{1}{N^2 p^2} \E \left[\bar{\mu}_1 (d) \sum_{i=1}^{N_1}c_i(d)p\mu_i (d)\right]  + o_P(1) \\
= & \frac{1}{N^2} \sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)} \E \left[\mu_i (1, 1, \mathbf{Z}_{-(i,j)};d)\mu_j (1, 1, \mathbf{Z}_{-(i,j)};d)\right] \\
& -\left(\frac{1}{N} \sum_{i=1}\E[\mu_i(\Y(1, \Z_{-i}); d)]\right)  \frac{1}{N^2 p^2} \E \left[\sum_{i=1}^{N_1}c(d)p \mu_i (d)\right]  + o_P(1) \\
= & \frac{1}{N^2} \sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)} \E \left[\mu_i (1, 1, \mathbf{Z}_{-(i,j)};d)\mu_j (1, 1, \mathbf{Z}_{-(i,j)};d)\right] \\
& -\left(\frac{1}{N} \sum_{i=1}\E[\mu_i(\Y(1, \Z_{-i}); d)]\right)  \left(\frac{c(d)}{N^2} \sum_{i=1} \E[\mu_j(\Y(1, \Z_{-j}); d)]\right) + o_P(1).
\end{align*}
%= & \frac{1}{N^2} \sum_{i=1}^{N} \sum_{j \in \mathbf{B}(i; d)} \E \left[\mu_i (\Y(1, \mathbf{Z}_{-i});d)\mu_j (\Y(1, \mathbf{Z}_{-j});d)\right] - \frac{1}{N^3 p^3} \sum_{i=1}^{N} \sum_{j \in \mathbf{B}(i; d)} \sum_{k=1}^{N} \E \left[Z_iZ_jZ_k\mu_i (\Y(1, \mathbf{Z}_{-i});d)\mu_k (1, \mathbf{Z}_{-k};d)\right] \\
%& - \frac{1}{N^3 p^3} \sum_{i=1}^{N} \sum_{j \in \mathbf{B}(i; d)}\sum_{k=1}^{N} \E \left[Z_iZ_jZ_k\mu_j (\Y(1, \mathbf{Z}_{-j});d)\mu_k (1, \mathbf{Z}_{-k};d)\right] + \frac{1}{N^2 p^2} \sum_{i=1}^{N} \sum_{j \in \mathbf{B}(i; d)} \E \left[Z_iZ_j\bar{\mu}_1^2 (d)\right] \\
%= & \frac{1}{N^2} \sum_{i=1}^{N} \sum_{j \in \mathbf{B}(i; d)} \E \left[\mu_i (\Y(1, \mathbf{Z}_{-i});d)\mu_j (\Y(1, \mathbf{Z}_{-j});d)\right] - \frac{1}{N^3 p} \sum_{i=1}^{N} \sum_{j \in \mathbf{B}(i; d)} \E \left[\mu_i (1, 1, 1, \mathbf{Z}_{-i};d)\mu_k (1, \mathbf{Z}_{-k};d)\right] \\
%When $N \rightarrow \infty$, we can apply the dominated convergence theorem to the second term above, then:
%\begin{align*}
%& \lim_{N \rightarrow \infty} \frac{1}{N^2 p^2} \sum_{i=1}^{N}\E \left[\bar{\mu}_1 (d) \sum_{j \in \mathbf{B}(i; d)} Z_iZ_j\left(\mu_i (\Y(1, \mathbf{Z}_{-i});d) - \bar{\mu}_1 (d) +\mu_j (\Y(1, \mathbf{Z}_{-j});d)\right) \right] \\
%= & \frac{1}{N^2 p^2} \sum_{i=1}^{N}\E \left[\lim_{N \rightarrow \infty} \bar{\mu}_1 (d) \sum_{j \in \mathbf{B}(i; d)} Z_iZ_j\left(\mu_i (\Y(1, \mathbf{Z}_{-i});d) - \bar{\mu}_1 (d) +\mu_j (\Y(1, \mathbf{Z}_{-j});d)\right) \right] \\
%= & \frac{1}{N^2 p^2} \sum_{i=1}^{N} \E\left[\mu_i(\Y(1, \mathbf{Z}_{-i});d) \right]\E \left[ \sum_{j \in \mathbf{B}(i; d)} Z_iZ_j\left(\mu_i (\Y(1, \mathbf{Z}_{-i});d) - \bar{\mu}_1 (d) +\mu_j (\Y(1, \mathbf{Z}_{-j});d)\right) \right] \\
%= & \frac{1}{N^2} \sum_{i=1}^{N} \E\left[\mu_i(\Y(1, \mathbf{Z}_{-i});d) \right] \sum_{j \in \mathbf{B}(i; d)} \E \left[ \mu_j (\Y(1,1, \mathbf{Z}_{-(i,j)});d) \right] \\
%\end{align*}

%(What remains to be shown here is that $\sum_{i=1}^N \sum_{j\neq i}^N \E\left[\mu_i(\Y(1, \Z_{-i}); d)\mu_j(\Y(1, \Z_{-j}); d)\right] = \sum_{i=1}^N \sum_{j\neq i}^N \E\left[\mu_i(\Y(1, 1, \Z_{-(i,j)}); d)\mu_j(\Y(1, 1, \Z_{-(i,j)}); d)\right]$).

The other terms can be similarly shown. Hence, the spatial HAC variance is an asymptotically unbiased estimate of the Hajek estimator's variance.


==> proofs/reference/regression.tex <==
\begin{align*}
\hat \tau(d) & = \frac{1}{Np}\sum_{i=1}^N Z_i\mu_i(\Y; d) - \frac{1}{N(1-p)}\sum_{i=1}^N(1-Z_i)\mu_i(\Y; d) \\
& = \frac{1}{N}\sum_{i=1}^N \frac{Z_i - p}{p(1-p)} \mu_i(\Y; d) \\
& = \frac{1}{N}\sum_{i=1}^N \frac{Z_i - p}{p(1-p)} \frac{\sum_{x\in \tilde{\mathcal{X}}} Y_x 1(d_i(x)=d)}{\sum_{x\in \mathcal{\tilde{X}}} 1(d_i(x)=d)} \\
& = \sum_{x\in \tilde{\mathcal{X}}} Y_x \frac{1}{N}\sum_{i=1}^N \frac{Z_i - p}{p(1-p)} \frac{ 1(d_i(x)=d)}{\sum_{x\in \mathcal{\tilde{X}}} 1(d_i(x)=d)}
\end{align*}


==> proofs/reference/variance_expression-for-paper_old.tex <==
%\input{tex-header}
%\begin{document}

We now present a lemma that derives the expectation and Neyman variance for the Hajek estimator under a Bernoulli design and the stable unit treatment value assumption (SUTVA, that is, no interference). This will be applied when we use the law of total variance to analyze the variance of the Hajek estimator given interference, where we can decompose the variance into terms that isolate the contributions due to interference.
\begin{lemma}\label{lemma:hajek-delta}
Suppose a binary treatment, $Z_i \in \{0,1\}$, a set of units $i=1,...,N$ for which the stable unit treatment value assumption (SUTVA) holds \citep{rubin80_randomization_analysis} , in which case we have potential outcomes $Y_i(1)$ and $Y_i(0)$ and realized outcomes $Y_i = Z_iY_i(1) + (1-Z_i)Y_i(0)$, and $Z_i \sim \text{Bernoulli}(p)$.  Suppose further that potential outcomes are bounded.  In this case, define a Hajek estimator of the average treatment effect as,
\begin{align*}
\hat \tau_{HA} = \frac{1}{N_1}\sum_{i=1}^{N}Z_i Y_i - \frac{1}{N_0}\sum_{i=1}^{N}(1-Z_i) Y_i
\end{align*}
where $N_1 = \sum_{i=1}^{N}Z_i$ and $N_0 = \sum_{i=1}^{N}(1-Z_i)$. Then, 
\begin{align*}
\Var(\hat \tau_{HA}) \leq \frac{1}{Np} \frac{\sum_{i=1}^{N}\left[Y_i(1) - \bar{Y}(1)\right]^2}{N} + \frac{1}{N(1-p)} \frac{\sum_{i=1}^{N}\left[Y_i(0) - \bar{Y}(0)\right]^2}{N} + o_P(N^{-1}).
\end{align*}
\end{lemma}

\begin{proof}
We can see that $\E(\frac{1}{N} \sum_{i=1}^{N}Z_i Y_i) = \frac{p}{N} \sum_{i=1}^{N}Y_i(1) = p\bar{Y}(1)$ and $\E(\frac{1}{N}\sum_{i=1}^{N}Z_i ) = p$. 

Using the law of large numbers, we know that $\frac{1}{N} \sum_{i=1}^{N}Z_i Y_i - p\bar{Y}(1) = o_p(1)$ and $\frac{1}{N}\sum_{i=1}^{N}Z_i  - p = o_p(1)$ when $Y_i$ has bounded variance. 

Let $f(a, b) = \frac{a}{b}$, then $\frac{1}{N_1}\sum_{i=1}^{N}Z_i Y_i = f(\frac{1}{N}\sum_{i=1}^{N}Z_i Y_i, \frac{1}{N}\sum_{i=1}^{N}Z_i )$. Taylor expansion around $(p\bar{Y}(1), p)$ results in $\frac{1}{N_1}\sum_{i=1}^{N}Z_i Y_i = \bar{Y}(1) + \frac{1}{p}(\frac{1}{N}\sum_{i=1}^{N}Z_i Y_i - p\bar{Y}(1) ) - \frac{\bar{Y}(1)}{p}(\frac{1}{N}\sum_{i=1}^{N}Z_i - p) + r_1$, where $r_1 = o_P(\frac{1}{N}\sum_{i=1}^{N}Z_i Y_i - p\bar{Y}(1))+ o_P(\frac{1}{N}\sum_{i=1}^{N}Z_i - p) = o_P(\frac{1}{\sqrt{N}})$ is the high-order remainder. Similarly,  $\frac{1}{N_0}\sum_{i=1}^{N}(1-Z_i) Y_i = \bar{Y}(0) + \frac{1}{1-p}(\frac{1}{N}\sum_{i=1}^{N}(1-Z_i) Y_i - (1-p)\bar{Y}(0) ) - \frac{\bar{Y}(0)}{1-p}(\frac{1}{N}\sum_{i=1}^{N}(1-Z_i) - (1-p)) + r_0$, where $r_0 = o_P(\frac{1}{N}\sum_{i=1}^{N}(1-Z_i) Y_i - (1-p)\bar{Y}(0) )+ o_P(\frac{1}{N}\sum_{i=1}^{N}(1-Z_i) - (1-p)) = o_P(\frac{1}{\sqrt{N}})$. Then $\E\left(\hat \tau_{HA}\right) = \E\left( \frac{1}{N_1}\sum_{i=1}^{N}Z_i Y_i - \frac{1}{N_0}\sum_{i=1}^{N}(1-Z_i) Y_i\right) =  \bar{Y}(1) - \bar{Y}(0) + o_P(1)$.

We know that:
\begin{align*}
\Var \begin{pmatrix}
\frac{1}{N} \sum_{i=1}^{N}Z_i Y_i \\
\frac{1}{N}\sum_{i=1}^{N}Z_i 
\end{pmatrix} = \begin{pmatrix}
\frac{p(1-p)}{N}\bar{Y}^2(1) & \frac{p(1-p)}{N}\bar{Y}(1) \\
\frac{p(1-p)}{N}\bar{Y}(1) & \frac{p(1-p)}{N}
\end{pmatrix}
\end{align*}
where $\bar{Y}^2(1) = \frac{1}{N}\sum_{i=1}^N Y_i^2(1)$.

As $\frac{1}{N_1}\sum_{i=1}^{N}Z_i Y_i = f(\frac{1}{N} \sum_{i=1}^{N}Z_i Y_i,  \frac{1}{N}\sum_{i=1}^{N}Z_i)$, we can apply the delta method to obtain: 

\begin{align*}
\Var\left(\frac{1}{N_1}\sum_{i=1}^{N}Z_i Y_i\right)  = & \begin{pmatrix}
\frac{1}{p} \\
-\frac{\bar{Y}(1)}{p}
\end{pmatrix}^{'} \Var \begin{pmatrix}
\frac{1}{N} \sum_{i=1}^{N}Z_i Y_i \\
\frac{1}{N}\sum_{i=1}^{N}Z_i 
\end{pmatrix} \begin{pmatrix}
\frac{1}{p} \\
-\frac{\bar{Y}(1)}{p}
\end{pmatrix}  + o_P(N^{-1}) \\
= & \begin{pmatrix}
\frac{1}{p} \\
-\frac{\bar{Y}(1)}{p}
\end{pmatrix}^{'} \begin{pmatrix}
\frac{p(1-p)}{N}\bar{Y}^2(1) & \frac{p(1-p)}{N}\bar{Y}(1) \\
\frac{p(1-p)}{N}\bar{Y}(1) & \frac{p(1-p)}{N}
\end{pmatrix} \begin{pmatrix}
\frac{1}{p} \\
-\frac{\bar{Y}(1)}{p}
\end{pmatrix}  + o_P(N^{-1}) \\
= & \frac{1-p}{Np}\begin{pmatrix}
1 \\
-\bar{Y}(1)
\end{pmatrix}^{'} \begin{pmatrix}
\bar{Y}^2(1) & \bar{Y}(1) \\
\bar{Y}(1) & 1
\end{pmatrix} \begin{pmatrix}
1 \\
-\bar{Y}(1)
\end{pmatrix}  + o_P(N^{-1}) \\
= & \frac{1-p}{Np} \frac{\sum_{i=1}^{N}\left[Y_i(1) - \bar{Y}(1)\right]^2}{N} + o_P(N^{-1}).
\end{align*}

Similarly, 
\begin{align*}
\Var\left(\frac{1}{N_0}\sum_{i=1}^{N}(1-Z_i) Y_i\right)
= \frac{p}{N(1-p)} \frac{\sum_{i=1}^{N}\left[Y_i(0) - \bar{Y}(0)\right]^2}{N} + o_P(N^{-1}).
\end{align*}

\begin{align*}
\Cov\left(\frac{1}{N_1}\sum_{i=1}^{N}Z_i Y_i,  \frac{1}{N_0}\sum_{i=1}^{N}(1-Z_i) Y_i\right)
= -\frac{1}{N^2} \sum_{i=1}^{N}\left[Y_i(1) - \bar{Y}(1)\right]\left[Y_i(0) - \bar{Y}(0)\right] + o_P(N^{-1}).
\end{align*}
Therefore,  
\begin{align*}
\Var(\hat \tau_{HA}) = & \Var\left(\frac{1}{N_1}\sum_{i=1}^{N}Z_i Y_i\right) + \Var\left(\frac{1}{N_0}\sum_{i=1}^{N}(1-Z_i) Y_i\right) \\ - & 2\Cov\left(\frac{1}{N_1}\sum_{i=1}^{N}Z_i Y_i,  \frac{1}{N_0}\sum_{i=1}^{N}(1-Z_i) Y_i\right) \\
\leq & \frac{1}{Np} \frac{\sum_{i=1}^{N}\left[Y_i(1) - \bar{Y}(1)\right]^2}{N} + \frac{1}{N(1-p)} \frac{\sum_{i=1}^{N}\left[Y_i(0) - \bar{Y}(0)\right]^2}{N}+ o_P(N^{-1}).
\end{align*}
\end{proof}

We now characterize the variance of the Horvitz-Thompson estimator. Our approach applies the decomposition proposed by \citet{chin2019-clt-interference}.  Remember that $\mathbf{B}(i;d) = \{j : ||x(i) - x(j)|| - d \le h(d)\}$, the set of intervention points in the interference region of $i$ for circle average with radius $d$, as characterized by condition C3.  Recall the implication of C3, that for $i,j$ with $||x(i) - x(j)|| - d > h(d)$,  $\Cov[\mu_i(Y(z, \Z_{-i});d), \mu_j(Y(z', \Z_{-j});d)] = 0$ for all $z, z^{'}$.

\begin{lemma}\label{lemma:ht-var}
Under conditions C1-C3 as defined in the main text, and for the estimator $\widehat{\tau}(d)$ defined in the main text, 
\begin{align*}
\Var(\widehat{\tau}(d)) \\
\leq & \frac{1}{N^2p}\sum_{i=1}^N \E[\mu_i^2(\Y(1, \Z_{-i}); d)] + \frac{1}{N^2(1-p)}\sum_{i=1}^N \E[\mu_i^2(\Y(0, \Z_{-i}); d)] \\
& + \frac{1}{N^2} \sum_{i=1} \sum_{j \in \mathbf{B}(i;d)}\{ \Cov[\mu_i(\Y(1, \Z_{-i}); d), \mu_j(\Y(1, \Z_{-j}); d)] \\
& - \Cov[\mu_i(\Y(1, \Z_{-i}); d), \mu_j(\Y(0, \Z_{-j}); d)] \\
& - \Cov[\mu_i(\Y(0, \Z_{-i}); d), \mu_j(\Y(1, \Z_{-j}); d)] \\
& + \Cov[\mu_i(\Y(0, \Z_{-i}); d), \mu_j(\Y(0, \Z_{-j}); d)] \}.
\end{align*}
\end{lemma}

\begin{proof}
Following the derivation in \citet{chin2019-clt-interference}, we define 
$$
\mathcal{F} = \{\mu_i(\Y(1, \Z_{-i}); d), \mu_i(\Y(0, \Z_{-i}); d)\}_{i \in \mathcal{N}}.
$$
Then:
\begin{align*}
\Var(\widehat{\tau}(d)) = &  \E[\Var(\widehat{\tau}(d) | \mathcal{F})] + \Var[\E(\widehat{\tau}(d) | \mathcal{F})] \\
\end{align*}

Notice that $\mu_i(\Y(1, \Z_{-i}); d)$ and $\mu_i(\Y(0, \Z_{-i}); d)$ are constants conditional on $\mathcal{F}$ and  $\{Z_i\}$ are independent to each other, hence we have:
\begin{align*}
\E[\Var (\widehat{\tau}(d) | \mathcal{F})] = & \E\left[\Var\left(\frac{1}{Np}\sum_{i=1}^N Z_i\mu_i(\Y(1, \mathbf{Z}_{-i}); d) - \frac{1}{N(1-p)}\sum_{i=1}^N (1-Z_i)\mu_i(\Y(0, \mathbf{Z}_{-i}); d) | \mathcal{F}\right)\right]  \\
= & \E\bigg[\frac{1}{N^2 p^2}\sum_{i=1}^N \Var(Z_i\mu_i(\Y(1, \mathbf{Z}_{-i}); d)| \mathcal{F}) \\
& + \frac{1}{N^2 (1-p)^2}\sum_{i=1}^N \Var((1-Z_i)\mu_i(\Y(0, \mathbf{Z}_{-i}); d) | \mathcal{F})\bigg]  \\
& - \E\left[\frac{2}{N^2 p(1-p)}\sum_{i=1}^N 
%\sum_{j=1}^N 
\Cov(Z_i\mu_i(\Y(1, \mathbf{Z}_{-i}); d), (1-Z_i)\mu_i(\Y(0, \mathbf{Z}_{-i}); d)| \mathcal{F}) \right]  \\
= & \frac{1-p}{N^2p}\sum_{i=1}^N \E[\mu_i^2(\Y(1, \Z_{-i}); d)] + \frac{p}{N^2(1-p)}\sum_{i=1}^N \E[\mu_i^2(\Y(0, \Z_{-i}); d)] \\
& + \frac{2}{N^2}\sum_{i=1}^N \E[\mu_i(\Y(1, \Z_{-i}); d) \mu_i(\Y(0, \Z_{-i}); d)].
\end{align*}
%where the last line follows from the Cauchy-Schwartz inequality.  Also,
%\begin{align*}
%\Var[\E(\widehat{\tau}(d) | \mathcal{F})] = & \Var\left[\frac{1}{Np}\sum_{i=1}^N \E\left(Z_i\mu_i(1, \mathbf{Z}_{-i}; d) | \mathcal{F}\right) - \frac{1}{N(1-p)}\sum_{i=1}^N \E\left((1-Z_i)\mu_i(0, \mathbf{Z}_{-i}; d) | \mathcal{F}\right)\right] \\
%= & \frac{1}{N^2} \Var\left[\sum_{i=1}^N \left(\mu_i(\Y(1, \Z_{-i}); d) - \mu_i(\Y(0, \Z_{-i}); d)\right)\right]. \\
%\end{align*}
%The first part is the conventional Neyman standard errors that can be estimated by:
%\begin{align*}
% \frac{1-p}{Np}\frac{\sum_{Z_i=1}[\mu_i(\Y(1, \Z_{-i}); d) - \bar{\mu}(\Y(1, \Z_{-i}); d)]^2}{Np-1} + \frac{p}{N(1-p)}\frac{\sum_{Z_i=0}[\mu_i(\Y(0, \Z_{-i}); d) - \bar{\mu}(\Y(0, \Z_{-i}); d)]^2}{N(1-p)-1}
%\end{align*}
The above part is the uncertainty induced by interference, which can be further expanded as follows:
\begin{align*}
& \frac{1}{N^2} \Var\left[\sum_{i=1} \left(\mu_i(\Y(1, \Z_{-i}); d) - \mu_i(\Y(0, \Z_{-i}); d)\right)\right] \\
= & \frac{1}{N^2} \sum_{i=1} \Var[\mu_i(\Y(1, \Z_{-i}); d) - \mu_i(\Y(0, \Z_{-i}); d)]  \\
+ & \frac{1}{N^2} \sum_{i=1} \sum_{i \neq j} \Cov[\left(\mu_i(\Y(1, \Z_{-i}); d) - \mu_i(\Y(0, \Z_{-i}); d)\right),  \left(\mu_j(\Y(1, \Z_{-j}); d) - \mu_j(\Y(0, \Z_{-j}); d)\right)] \\
= & \frac{1}{N^2} \sum_{i=1} \Var[\mu_i(\Y(1, \Z_{-i}); d) - \mu_i(\Y(0, \Z_{-i}); d)] \\
+ & \frac{1}{N^2} \sum_{i=1} \sum_{i \neq j}\{ \Cov[\mu_i(\Y(1, \Z_{-i}); d), \mu_j(\Y(1, \Z_{-j}); d)] - \Cov[\mu_i(\Y(1, \Z_{-i}); d), \mu_j(\Y(0, \Z_{-j}); d)] \\
- & \Cov[\mu_i(\Y(0, \Z_{-i}); d), \mu_j(\Y(1, \Z_{-j}); d)] + \Cov[\mu_i(\Y(0, \Z_{-i}); d), \mu_j(\Y(0, \Z_{-j}); d)] \} \\
= & \frac{1}{N^2} \sum_{i=1} \Var[\mu_i(\Y(1, \Z_{-i}); d) - \mu_i(\Y(0, \Z_{-i}); d)] \\
+ & \frac{1}{N^2} \sum_{i=1} \sum_{j \in \mathbf{B}(i;d)}\{ \Cov[\mu_i(\Y(1, \Z_{-i}); d), \mu_j(\Y(1, \Z_{-j}); d)] - \Cov[\mu_i(\Y(1, \Z_{-i}); d), \mu_j(\Y(0, \Z_{-j}); d)] \\
- & \Cov[\mu_i(\Y(0, \Z_{-i}); d), \mu_j(\Y(1, \Z_{-j}); d)] + \Cov[\mu_i(\Y(0, \Z_{-i}); d), \mu_j(\Y(0, \Z_{-j}); d)] \}.
\end{align*}
Clearly, the first term is due to the heterogeneity of the treatment effect caused by interference, and the remaining terms capture the interference among units. 
To summarize,
\begin{align*}
& \Var(\hat{\tau}(d)) \\
= & \frac{1-p}{N^2p}\sum_{i=1}^N \E[\mu_i^2(\Y(1, \Z_{-i}); d)] + \frac{p}{N^2(1-p)}\sum_{i=1}^N \E[\mu_i^2(\Y(0, \Z_{-i}); d)] \\
& + \frac{2}{N^2}\sum_{i=1}^N \E[\mu_i(\Y(1, \Z_{-i}); d) \mu_i(\Y(0, \Z_{-i}); d)] + \frac{1}{N^2} \sum_{i=1} \Var[\mu_i(\Y(1, \Z_{-i}); d) - \mu_i(\Y(0, \Z_{-i}); d)] \\
& + \frac{1}{N^2} \sum_{i=1} \sum_{j \in \mathbf{B}(i)}\{ \Cov[\mu_i(\Y(1, \Z_{-i}); d), \mu_j(\Y(1, \Z_{-j}); d)] - \Cov[\mu_i(\Y(1, \Z_{-i}); d), \mu_j(\Y(0, \Z_{-j}); d)] \\
& -  \Cov[\mu_i(\Y(0, \Z_{-i}); d), \mu_j(\Y(1, \Z_{-j}); d)] + \Cov[\mu_i(\Y(0, \Z_{-i}); d), \mu_j(\Y(0, \Z_{-j}); d)] \} \\
\leq & \frac{1}{N^2p}\sum_{i=1}^N \E[\mu_i^2(\Y(1, \Z_{-i}); d)] + \frac{1}{N^2(1-p)}\sum_{i=1}^N \E[\mu_i^2(\Y(0, \Z_{-i}); d)] \\
& + \frac{1}{N^2} \sum_{i=1} \sum_{j \in \mathbf{B}(i)}\{ \Cov[\mu_i(\Y(1, \Z_{-i}); d), \mu_j(\Y(1, \Z_{-j}); d)] - \Cov[\mu_i(\Y(1, \Z_{-i}); d), \mu_j(\Y(0, \Z_{-j}); d)] \\
& -  \Cov[\mu_i(\Y(0, \Z_{-i}); d), \mu_j(\Y(1, \Z_{-j}); d)] + \Cov[\mu_i(\Y(0, \Z_{-i}); d), \mu_j(\Y(0, \Z_{-j}); d)] \}.
\end{align*}
where the last line follows from the definition of variance:
\begin{align*}
& \frac{2}{N^2}\sum_{i=1}^N \E[\mu_i(\Y(1, \Z_{-i}); d) \mu_i(\Y(0, \Z_{-i}); d)] + \frac{1}{N^2} \sum_{i=1} \Var[\mu_i(\Y(1, \Z_{-i}); d) - \mu_i(\Y(0, \Z_{-i}); d)] \\
= & \frac{2}{N^2}\sum_{i=1}^N \E[\mu_i(\Y(1, \Z_{-i}); d) \mu_i(\Y(0, \Z_{-i}); d)] + \frac{1}{N^2} \sum_{i=1} \E[\mu_i(\Y(1, \Z_{-i}); d) - \mu_i(\Y(0, \Z_{-i}); d)]^2 \\
&  - \frac{1}{N^2} \sum_{i=1} \E^2[\mu_i(\Y(1, \Z_{-i}); d) - \mu_i(\Y(0, \Z_{-i}); d)] \\
= & \frac{1}{N^2} \sum_{i=1} \E[\mu_i^2(\Y(1, \Z_{-i}); d) + \mu_i^2(\Y(0, \Z_{-i}); d)]  - \frac{1}{N^2} \sum_{i=1} \E^2[\mu_i(\Y(1, \Z_{-i}); d) - \mu_i(\Y(0, \Z_{-i}); d)] \\
\leq & \frac{1}{N^2} \sum_{i=1} \E[\mu_i^2(\Y(1, \Z_{-i}); d) + \mu_i^2(\Y(0, \Z_{-i}); d)]
\end{align*}
\end{proof}

The limiting variance of the Hajek estimator is similar, as captured by the following

\begin{lemma}
Define
\begin{align*}
\tilde{V} = & \frac{1}{N^2p}\sum_{i=1}^N \E\left[\left(\mu_i(\Y(1, \Z_{-i}); d) - \bar {\mu}_1\right)^2\right] + \frac{1}{N^2(1-p)}\sum_{i=1}^N \E\left[\left(\mu_i(\Y(0, \Z_{-i}); d)- \bar {\mu}_0\right)^2\right] \\
+ & \frac{1}{N^2} \sum_{i=1} \sum_{j \in \mathbf{B}(i;d)}\{ \Cov[\mu_i(\Y(1, \Z_{-i}); d), \mu_j(\Y(1, \Z_{-j}); d)] - \Cov[\mu_i(\Y(1, \Z_{-i}); d), \mu_j(\Y(0, \Z_{-j}); d)] \\
- & \Cov[\mu_i(\Y(0, \Z_{-i}); d), \mu_j(\Y(1, \Z_{-j}); d)] + \Cov[\mu_i(\Y(0, \Z_{-i}); d), \mu_j(\Y(0, \Z_{-j}); d)] \}.
\end{align*}
Under conditions C1-C4 as defined in the main text, and for the estimator $\widehat{\tau}_{HA}(d)$ defined in the main text, as $N \rightarrow \infty$, 
$$
\mathrm{Pr}(\Var(\widehat{\tau}_{HA}(d)) \le \tilde{V}) \rightarrow 1.
$$
\end{lemma}

\begin{proof}
Applying the same decomposition as for the proof of Lemma \ref{lemma:ht-var}, conditional on $\mathcal{F}$, there is no interference, thus we can apply all the asymptotic results obtained under SUTVA. Now the first part becomes:
\begin{align*}
& \E[\Var(\hat{\tau}_{HA}(d) | \mathcal{F})] \\
= & \frac{1}{N^2p}\sum_{i=1}^N \E\left[\left(\mu_i(\Y(1, \Z_{-i}); d) - \bar {\mu}_1^0\right)^2\right] + \frac{1}{N^2(1-p)}\sum_{i=1}^N \E\left[\left(\mu_i(\Y(0, \Z_{-i}); d)- \bar {\mu}_0^0\right)^2\right]  \\
& + \frac{2}{N^2}\sum_{i=1}^N \E\left[\left(\mu_i(\Y(1, \Z_{-i}); d) - \bar {\mu}_1^0\right) \left(\mu_i(\Y(0, \Z_{-i}); d)- \bar {\mu}_0^0\right)\right].+ o(N^{-1}) \\
= & \frac{1}{N^2p}\sum_{i=1}^N \E\left[\left(\mu_i(\Y(1, \Z_{-i}); d) - \bar {\mu}_1^0\right)^2\right] + \frac{1}{N^2(1-p)}\sum_{i=1}^N \E\left[\left(\mu_i(\Y(0, \Z_{-i}); d)- \bar {\mu}_0^0\right)^2\right]  \\
& + \frac{2}{N^2}\sum_{i=1}^N \E\left[\mu_i(\Y(1, \Z_{-i}); d) \mu_i(\Y(0, \Z_{-i}); d)\right] \\
& - \frac{2}{N^3}\sum_{i=1}^N \sum_{j=1}^N \E\left[\mu_i(\Y(1, \Z_{-i}); d) \mu_j(\Y(0, \Z_{-j}); d)\right].+ o(N^{-1}) \\
= & \frac{1}{N^2p}\sum_{i=1}^N \E\left[\left(\mu_i(\Y(1, \Z_{-i}); d) - \bar {\mu}_1^0\right)^2\right] + \frac{1}{N^2(1-p)}\sum_{i=1}^N \E\left[\left(\mu_i(\Y(0, \Z_{-i}); d)- \bar {\mu}_0^0\right)^2\right]  \\
& + \frac{2}{N^2}\sum_{i=1}^N \E\left[\mu_i(\Y(1, \Z_{-i}); d) \mu_i(\Y(0, \Z_{-i}); d)\right] + o(N^{-1}),
\end{align*}
where $\bar {\mu}_1^0 = \frac{1}{N}\sum_{i=1}^N \mu_i(\Y(1, \Z_{-i}); d)$ and $\bar {\mu}_0^0 = \frac{1}{N}\sum_{i=1}^N \mu_i(\Y(0, \Z_{-i}); d)$. The last equality uses the boundedness of $Y_i$ (C2) and $c(d)$ (C4).

For the second part, we know that:
\begin{align*}
& \E(\widehat{\tau}_{HA}(d) | \mathcal{F}) \\
& =  \frac{1}{Np}\sum_{i=1}^N \E\left(Z_i\mu_i(\Y(1, \mathbf{Z}_{-i}); d) | \mathcal{F}\right) - \frac{1}{N(1-p)}\sum_{i=1}^N \E\left((1-Z_i)\mu_i(\Y(0, \mathbf{Z}_{-i}); d) | \mathcal{F}\right) + o_P(1)\\
\end{align*}
Therefore,
\begin{align*}
\Var[\E(\widehat{\tau}_{HA}(d) | \mathcal{F})] = & \Var\bigg[\frac{1}{Np}\sum_{i=1}^N \E\left(Z_i\mu_i(\Y(1, \mathbf{Z}_{-i}); d) | \mathcal{F}\right) \\
& - \frac{1}{N(1-p)}\sum_{i=1}^N \E\left((1-Z_i)\mu_i(\Y(0, \mathbf{Z}_{-i}); d) | \mathcal{F}\right)\bigg] \\
= & \frac{1}{N^2} \Var\left[\sum_{i=1}^N \left(\mu_i(\Y(1, \Z_{-i}); d) - \mu_i(\Y(0, \Z_{-i}); d)\right)\right] + o_P(N^{-1})\\
\end{align*}
and
\begin{align*}
& \Var(\widehat{\tau}_{HA}(d)) \\
\leq & \frac{1}{N^2p}\sum_{i=1}^N \E\left[\left(\mu_i(\Y(1, \Z_{-i}); d) - \bar {\mu}_1\right)^2\right] + \frac{1}{N^2(1-p)}\sum_{i=1}^N \E\left[\left(\mu_i(\Y(0, \Z_{-i}); d)- \bar {\mu}_0\right)^2\right] \\
+ & \frac{1}{N^2} \sum_{i=1} \sum_{j \in \mathbf{B}(i;d)}\{ \Cov[\mu_i(\Y(1, \Z_{-i}); d), \mu_j(\Y(1, \Z_{-j}); d)] - \Cov[\mu_i(\Y(1, \Z_{-i}); d), \mu_j(\Y(0, \Z_{-j}); d)] \\
- & \Cov[\mu_i(\Y(0, \Z_{-i}); d), \mu_j(\Y(1, \Z_{-j}); d)] + \Cov[\mu_i(\Y(0, \Z_{-i}); d), \mu_j(\Y(0, \Z_{-j}); d)] \}+ o_P(N^{-1})
\end{align*}.
\end{proof}



%\end{document}




==> proofs/reference/variance_expression.tex <==
\input{tex-header}
\begin{document}
We first derive the expectation and Neyman variance for the Hajek estimator under Bernoulli design and SUTVA. The estimator can be written as:
\begin{align*}
\hat \tau_{HA} = \frac{1}{N_1}\sum_{i=1}^{N}Z_i Y_i - \frac{1}{N_0}\sum_{i=1}^{N}(1-Z_i) Y_i
\end{align*}
where $N_1 = \sum_{i=1}^{N}Z_i$ and $N_0 = \sum_{i=1}^{N}(1-Z_i)$.

It is easy to see that $\E(\frac{1}{N} \sum_{i=1}^{N}Z_i Y_i) = \frac{p}{N} \sum_{i=1}^{N}Y_i(1) = p\bar{Y}_i(1)$ and $\E(\frac{1}{N}\sum_{i=1}^{N}Z_i ) = p$. Using the law of large numbers, we know that $\frac{1}{N} \sum_{i=1}^{N}Z_i Y_i - p\bar{Y}_i(1) = o_P(1)$ and $\frac{1}{N}\sum_{i=1}^{N}Z_i  - p = o_P(1)$ when $Y_i$ has bounded variance. Let $f(a, b) = \frac{a}{b}$, then $\frac{1}{N_1}\sum_{i=1}^{N}Z_i Y_i = f(\frac{1}{N}\sum_{i=1}^{N}Z_i Y_i, \frac{1}{N}\sum_{i=1}^{N}Z_i )$. Taylor expansion around $(p\bar{Y}_i(1), p)$ results in $\frac{1}{N_1}\sum_{i=1}^{N}Z_i Y_i = \bar{Y}_i(1) + \frac{1}{p}(\frac{1}{N}\sum_{i=1}^{N}Z_i Y_i - p\bar{Y}_i(1) ) - \frac{\bar{Y}_i(1)}{p}(\frac{1}{N}\sum_{i=1}^{N}Z_i - p) + r_1$, where $r_1 = o_P(\frac{1}{N}\sum_{i=1}^{N}Z_i Y_i - p\bar{Y}_i(1))+ o_P(\frac{1}{N}\sum_{i=1}^{N}Z_i - p) = o_P(\frac{1}{\sqrt N})$ is the high-order remainder. Similarly,  $\frac{1}{N_0}\sum_{i=1}^{N}(1-Z_i) Y_i = \bar{Y}_i(0) + \frac{1}{1-p}(\frac{1}{N}\sum_{i=1}^{N}(1-Z_i) Y_i - (1-p)\bar{Y}_i(0) ) - \frac{\bar{Y}_i(0)}{1-p}(\frac{1}{N}\sum_{i=1}^{N}(1-Z_i) - (1-p)) + r_0$, where $r_0 = o_P(\frac{1}{N}\sum_{i=1}^{N}(1-Z_i) Y_i - (1-p)\bar{Y}_i(0) )+ o_P(\frac{1}{N}\sum_{i=1}^{N}(1-Z_i) - (1-p)) = o_P(\frac{1}{\sqrt N})$. Then $\E\left(\hat \tau_{HA}\right) = \E\left( \frac{1}{N_1}\sum_{i=1}^{N}Z_i Y_i - \frac{1}{N_0}\sum_{i=1}^{N}(1-Z_i) Y_i\right) \overset{P}{\rightarrow}  \bar{Y}_i(1) - \bar{Y}_i(0)$.

We know that:
\begin{align*}
\Var \begin{pmatrix}
\frac{1}{N} \sum_{i=1}^{N}Z_i Y_i \\
\frac{1}{N}\sum_{i=1}^{N}Z_i 
\end{pmatrix} = \begin{pmatrix}
\frac{p(1-p)}{N}\bar{Y}_i^2(1) & \frac{p(1-p)}{N}\bar{Y}_i(1) \\
\frac{p(1-p)}{N}\bar{Y}_i(1) & \frac{p(1-p)}{N}
\end{pmatrix}
\end{align*}
where $\bar{Y}_i^2(1) = \frac{1}{N}\sum_{i=1}^N Y_i^2(1)$.

As $\frac{1}{N_1}\sum_{i=1}^{N}Z_i Y_i = f(\frac{1}{N} \sum_{i=1}^{N}Z_i Y_i,  \frac{1}{N}\sum_{i=1}^{N}Z_i)$, we can apply the delta method to obtain: 

\begin{align*}
N \Var\left(\frac{1}{N_1}\sum_{i=1}^{N}Z_i Y_i\right) =  & N \begin{pmatrix}
\frac{1}{p} \\
-\frac{\bar{Y}_i(1)}{p}
\end{pmatrix}^{'} \Var \begin{pmatrix}
\frac{1}{N} \sum_{i=1}^{N}Z_i Y_i \\
\frac{1}{N}\sum_{i=1}^{N}Z_i 
\end{pmatrix} \begin{pmatrix}
\frac{1}{p} \\
-\frac{\bar{Y}_i(1)}{p}
\end{pmatrix} + o_P(1) \\ 
= & \begin{pmatrix}
\frac{1}{p} \\
-\frac{\bar{Y}_i(1)}{p}
\end{pmatrix}^{'} \begin{pmatrix}
\frac{p(1-p)}{N}\bar{Y}_i^2(1) & \frac{p(1-p)}{N}\bar{Y}_i(1) \\
\frac{p(1-p)}{N}\bar{Y}_i(1) & \frac{p(1-p)}{N}
\end{pmatrix} \begin{pmatrix}
\frac{1}{p} \\
-\frac{\bar{Y}_i(1)}{p}
\end{pmatrix}  + o_P(1) \\
= & \frac{1-p}{p}\begin{pmatrix}
1 \\
-\bar{Y}_i(1)
\end{pmatrix}^{'} \begin{pmatrix}
\bar{Y}_i^2(1) & \bar{Y}_i(1) \\
\bar{Y}_i(1) & 1
\end{pmatrix} \begin{pmatrix}
1 \\
-\bar{Y}_i(1)
\end{pmatrix}  + o_P(1) \\
= & \frac{1-p}{p} \frac{\sum_{i=1}^{N}\left[Y_i(1) - \bar{Y}_i(1)\right]^2}{N}  + o_P(1)
\end{align*}

Similarly, 
\begin{align*}
\Var\left(\frac{1}{N_0}\sum_{i=1}^{N}(1-Z_i) Y_i\right)
= \frac{p}{N(1-p)} \frac{\sum_{i=1}^{N}\left[Y_i(0) - \bar{Y}_i(0)\right]^2}{N} + o_P(N^{-1}),
\end{align*}

\begin{align*}
\Cov\left(\frac{1}{N_1}\sum_{i=1}^{N}Z_i Y_i,  \frac{1}{N_0}\sum_{i=1}^{N}(1-Z_i) Y_i\right)
= -\frac{1}{N^2} \sum_{i=1}^{N}\left[Y_i(1) - \bar{Y}_i(1)\right]\left[Y_i(0) - \bar{Y}_i(0)\right] + o_P(N^{-1}).
\end{align*}
Therefore,  
\begin{align*}
\Var(\hat \tau_{HA}) = & \Var\left(\frac{1}{N_1}\sum_{i=1}^{N}Z_i Y_i\right) + \Var\left(\frac{1}{N_0}\sum_{i=1}^{N}(1-Z_i) Y_i\right) \\ - & 2\Cov\left(\frac{1}{N_1}\sum_{i=1}^{N}Z_i Y_i,  \frac{1}{N_0}\sum_{i=1}^{N}(1-Z_i) Y_i\right) \\
= & \frac{1}{Np} \frac{\sum_{i=1}^{N}\left[Y_i(1) - \bar{Y}_i(1)\right]^2}{N} + \frac{1}{N(1-p)} \frac{\sum_{i=1}^{N}\left[Y_i(0) - \bar{Y}_i(0)\right]^2}{N}  \\
& + \frac{2}{N^2} \sum_{i=1}^{N}\left[Y_i(1) - \bar{Y}_i(1)\right]\left[Y_i(0) - \bar{Y}_i(0)\right]  + o_P(N^{-1}).
\end{align*}
%\begin{align*}
%\Var(\hat \tau_{HA}) = & \Var\left(\frac{1}{N_1}\sum_{i=1}^{N}Z_i Y_i\right) + \Var\left(\frac{1}{N_0}\sum_{i=1}^{N}(1-Z_i) Y_i\right) \\ - & 2\Cov\left(\frac{1}{N_1}\sum_{i=1}^{N}Z_i Y_i,  \frac{1}{N_0}\sum_{i=1}^{N}(1-Z_i) Y_i\right) \\
%\leq & \frac{1}{Np} \frac{\sum_{i=1}^{N}\left[Y_i(1) - \bar{Y}_i(1)\right]^2}{N} + \frac{1}{N(1-p)} \frac{\sum_{i=1}^{N}\left[Y_i(0) - \bar{Y}_i(0)\right]^2}{N}  + o_P(N^{-1}).
%\end{align*}
\newpage
Following the derivation in Chin (2017), we set $\mathcal{F} = \{\mu_i(\Y(1, \Z_{-i}); d), \mu_i(\Y(0, \Z_{-i}); d), i \in \{1,2,\dots,N\}\}$, then:
\begin{align*}
\Var(\hat{\tau}_d) = &  \E[\Var(\hat{\tau}_d | \mathcal{F})] + \Var[\E(\hat{\tau}_d | \mathcal{F})] \\
\end{align*}
Since $\{Z_i\}$ are independent to each other, we have:
\begin{align*}
\E[\Var\hat{\tau}_d | \mathcal{F})] = & \E\left[\Var\left(\frac{1}{Np}\sum_{i=1}^N Z_i\mu_i(1, \mathbf{Z}_{-i}; d) - \frac{1}{N(1-p)}\sum_{i=1}^N (1-Z_i)\mu_i(0, \mathbf{Z}_{-i}; d) | \mathcal{F}\right)\right]  \\
= & \E\left[\frac{1}{N^2 p^2}\sum_{i=1}^N \Var(Z_i\mu_i(1, \mathbf{Z}_{-i}; d)| \mathcal{F}) + \frac{1}{N^2 (1-p)^2}\sum_{i=1}^N \Var((1-Z_i)\mu_i(0, \mathbf{Z}_{-i}; d) | \mathcal{F})\right]  \\
& - \E\left[\frac{2}{N^2 p(1-p)}\sum_{i=1}^N \sum_{j=1}^N \Cov(Z_i\mu_i(1, \mathbf{Z}_{-i}; d), (1-Z_i)\mu_i(0, \mathbf{Z}_{-i}; d)| \mathcal{F}) \right]  \\
= & \frac{1-p}{N^2p}\sum_{i=1}^N \E[\mu_i^2(\Y(1, \Z_{-i}); d)] + \frac{p}{N^2(1-p)}\sum_{i=1}^N \E[\mu_i^2(\Y(0, \Z_{-i}); d)] \\
& + \frac{2}{N^2}\sum_{i=1}^N \E[\mu_i(\Y(1, \Z_{-i}); d) \mu_i(\Y(0, \Z_{-i}); d)].
\end{align*}
And,
\begin{align*}
\Var[\E(\hat{\tau}_d | \mathcal{F})] = & \Var\left[\frac{1}{Np}\sum_{i=1}^N \E\left(Z_i\mu_i(1, \mathbf{Z}_{-i}; d) | \mathcal{F}\right) - \frac{1}{N(1-p)}\sum_{i=1}^N \E\left((1-Z_i)\mu_i(0, \mathbf{Z}_{-i}; d) | \mathcal{F}\right)\right] \\
= & \frac{1}{N^2} \Var\left[\sum_{i=1}^N \left(\mu_i(\Y(1, \Z_{-i}); d) - \mu_i(\Y(0, \Z_{-i}); d)\right)\right] \\
\end{align*}
%The first part is the conventional Neyman standard errors that can be estimated by:
%\begin{align*}
% \frac{1-p}{Np}\frac{\sum_{Z_i=1}[\mu_i(\Y(1, \Z_{-i}); d) - \bar{\mu}(\Y(1, \Z_{-i}); d)]^2}{Np-1} + \frac{p}{N(1-p)}\frac{\sum_{Z_i=0}[\mu_i(\Y(0, \Z_{-i}); d) - \bar{\mu}(\Y(0, \Z_{-i}); d)]^2}{N(1-p)-1}
%\end{align*}
The above part is the uncertainty induced by interference, which can be further expanded as follows:
\begin{align*}
& \frac{1}{N^2} \Var\left[\sum_{i=1} \left(\mu_i(\Y(1, \Z_{-i}); d) - \mu_i(\Y(0, \Z_{-i}); d)\right)\right] \\
= & \frac{1}{N^2} \sum_{i=1} \Var[\mu_i(\Y(1, \Z_{-i}); d) - \mu_i(\Y(0, \Z_{-i}); d)]  \\
+ & \frac{1}{N^2} \sum_{i=1} \sum_{i \neq j} \Cov[\left(\mu_i(\Y(1, \Z_{-i}); d) - \mu_i(\Y(0, \Z_{-i}); d)\right),  \left(\mu_j(\Y(1, \Z_{-j}); d) - \mu_j(\Y(0, \Z_{-j}); d)\right)] \\
= & \frac{1}{N^2} \sum_{i=1} \Var[\mu_i(\Y(1, \Z_{-i}); d) - \mu_i(\Y(0, \Z_{-i}); d)] \\
+ & \frac{1}{N^2} \sum_{i=1} \sum_{i \neq j}\{ \Cov[\mu_i(\Y(1, \Z_{-i}); d), \mu_j(\Y(1, \Z_{-j}); d)] - \Cov[\mu_i(\Y(1, \Z_{-i}); d), \mu_j(\Y(0, \Z_{-j}); d)] \\
- & \Cov[\mu_i(\Y(0, \Z_{-i}); d), \mu_j(\Y(1, \Z_{-j}); d)] + \Cov[\mu_i(\Y(0, \Z_{-i}); d), \mu_j(\Y(0, \Z_{-j}); d)] \} \\
= & \frac{1}{N^2} \sum_{i=1} \Var[\mu_i(\Y(1, \Z_{-i}); d) - \mu_i(\Y(0, \Z_{-i}); d)] \\
+ & \frac{1}{N^2} \sum_{i=1} \sum_{j \in \mathbf{B}(i)}\{ \Cov[\mu_i(\Y(1, \Z_{-i}); d), \mu_j(\Y(1, \Z_{-j}); d)] - \Cov[\mu_i(\Y(1, \Z_{-i}); d), \mu_j(\Y(0, \Z_{-j}); d)] \\
- & \Cov[\mu_i(\Y(0, \Z_{-i}); d), \mu_j(\Y(1, \Z_{-j}); d)] + \Cov[\mu_i(\Y(0, \Z_{-i}); d), \mu_j(\Y(0, \Z_{-j}); d)] \}
\end{align*}
Clearly, the first term is due to the heterogeneity of the treatment effect caused by interference, and the remaining terms capture the interference among units. 
To summarize,
\begin{align*}
& \Var(\hat{\tau}_d) \\
= & \frac{1-p}{N^2p}\sum_{i=1}^N \E[\mu_i^2(\Y(1, \Z_{-i}); d)] + \frac{p}{N^2(1-p)}\sum_{i=1}^N \E[\mu_i^2(\Y(0, \Z_{-i}); d)] \\
& + \frac{2}{N^2}\sum_{i=1}^N \E[\mu_i(\Y(1, \Z_{-i}); d) \mu_i(\Y(0, \Z_{-i}); d)] + \frac{1}{N^2} \sum_{i=1} \Var[\mu_i(\Y(1, \Z_{-i}); d) - \mu_i(\Y(0, \Z_{-i}); d)] \\
& + \frac{1}{N^2} \sum_{i=1} \sum_{j \in \mathbf{B}(i)}\{ \Cov[\mu_i(\Y(1, \Z_{-i}); d), \mu_j(\Y(1, \Z_{-j}); d)] - \Cov[\mu_i(\Y(1, \Z_{-i}); d), \mu_j(\Y(0, \Z_{-j}); d)] \\
& -  \Cov[\mu_i(\Y(0, \Z_{-i}); d), \mu_j(\Y(1, \Z_{-j}); d)] + \Cov[\mu_i(\Y(0, \Z_{-i}); d), \mu_j(\Y(0, \Z_{-j}); d)] \} \\
\leq & \frac{1}{N^2p}\sum_{i=1}^N \E[\mu_i^2(\Y(1, \Z_{-i}); d)] + \frac{1}{N^2(1-p)}\sum_{i=1}^N \E[\mu_i^2(\Y(0, \Z_{-i}); d)] \\
& + \frac{1}{N^2} \sum_{i=1} \sum_{j \in \mathbf{B}(i)}\{ \Cov[\mu_i(\Y(1, \Z_{-i}); d), \mu_j(\Y(1, \Z_{-j}); d)] - \Cov[\mu_i(\Y(1, \Z_{-i}); d), \mu_j(\Y(0, \Z_{-j}); d)] \\
& -  \Cov[\mu_i(\Y(0, \Z_{-i}); d), \mu_j(\Y(1, \Z_{-j}); d)] + \Cov[\mu_i(\Y(0, \Z_{-i}); d), \mu_j(\Y(0, \Z_{-j}); d)] \}.
\end{align*}
The last inequality is due to the following derivation:
\begin{align*}
& \frac{2}{N^2}\sum_{i=1}^N \E[\mu_i(\Y(1, \Z_{-i}); d) \mu_i(\Y(0, \Z_{-i}); d)] + \frac{1}{N^2} \sum_{i=1} \Var[\mu_i(\Y(1, \Z_{-i}); d) - \mu_i(\Y(0, \Z_{-i}); d)] \\
= & \frac{2}{N^2}\sum_{i=1}^N \E[\mu_i(\Y(1, \Z_{-i}); d) \mu_i(\Y(0, \Z_{-i}); d)] + \frac{1}{N^2} \sum_{i=1} \E[\mu_i(\Y(1, \Z_{-i}); d) - \mu_i(\Y(0, \Z_{-i}); d)]^2 \\
&  - \frac{1}{N^2} \sum_{i=1} \E^2[\mu_i(\Y(1, \Z_{-i}); d) - \mu_i(\Y(0, \Z_{-i}); d)] \\
= & \frac{1}{N^2} \sum_{i=1} \E[\mu_i^2(\Y(1, \Z_{-i}); d) + \mu_i^2(\Y(0, \Z_{-i}); d)]  - \frac{1}{N^2} \sum_{i=1} \E^2[\mu_i(\Y(1, \Z_{-i}); d) - \mu_i(\Y(0, \Z_{-i}); d)] \\
\leq & \frac{1}{N^2} \sum_{i=1} \E[\mu_i^2(\Y(1, \Z_{-i}); d) + \mu_i^2(\Y(0, \Z_{-i}); d)]
\end{align*}

The variance of the Hajek estimator is similar. Conditional on $\mathcal{F}$, there is no interference, thus we can apply all the asymptotic results obtained under SUTVA. Now the first part becomes:
\begin{align*}
& \E[\Var(\hat{\tau}_{d, HA} | \mathcal{F})] \\
= & \frac{1}{N^2p}\sum_{i=1}^N \E\left[\left(\mu_i(\Y(1, \Z_{-i}); d) - \bar {\mu}_1^0\right)^2\right] + \frac{1}{N^2(1-p)}\sum_{i=1}^N \E\left[\left(\mu_i(\Y(0, \Z_{-i}); d)- \bar {\mu}_0^0\right)^2\right]  \\
& + \frac{2}{N^2}\sum_{i=1}^N \E\left[\left(\mu_i(\Y(1, \Z_{-i}); d) - \bar {\mu}_1^0\right) \left(\mu_i(\Y(0, \Z_{-i}); d)- \bar {\mu}_0^0\right)\right].+ o(N^{-1}) \\
= & \frac{1}{N^2p}\sum_{i=1}^N \E\left[\left(\mu_i(\Y(1, \Z_{-i}); d) - \bar {\mu}_1^0\right)^2\right] + \frac{1}{N^2(1-p)}\sum_{i=1}^N \E\left[\left(\mu_i(\Y(0, \Z_{-i}); d)- \bar {\mu}_0^0\right)^2\right]  \\
& + \frac{2}{N^2}\sum_{i=1}^N \E\left[\mu_i(\Y(1, \Z_{-i}); d) \mu_i(\Y(0, \Z_{-i}); d)\right] \\
& - \frac{2}{N^3}\sum_{i=1}^N \sum_{j=1}^N \E\left[\mu_i(\Y(1, \Z_{-i}); d) \mu_j(\Y(0, \Z_{-j}); d)\right].+ o(N^{-1}) \\
= & \frac{1}{N^2p}\sum_{i=1}^N \E\left[\left(\mu_i(\Y(1, \Z_{-i}); d) - \bar {\mu}_1^0\right)^2\right] + \frac{1}{N^2(1-p)}\sum_{i=1}^N \E\left[\left(\mu_i(\Y(0, \Z_{-i}); d)- \bar {\mu}_0^0\right)^2\right]  \\
& + \frac{2}{N^2}\sum_{i=1}^N \E\left[\mu_i(\Y(1, \Z_{-i}); d) \mu_i(\Y(0, \Z_{-i}); d)\right] + o(N^{-1}),
\end{align*}
where $\bar {\mu}_1^0 = \frac{1}{N}\sum_{i=1}^N \mu_i(\Y(1, \Z_{-i}); d)$ and $\bar {\mu}_0^0 = \frac{1}{N}\sum_{i=1}^N \mu_i(\Y(0, \Z_{-i}); d)$.

For the second part, we know that:
\begin{align*}
\E(\hat{\tau}_{d, HA} | \mathcal{F}) = \frac{1}{Np}\sum_{i=1}^N \E\left(Z_i\mu_i(1, \mathbf{Z}_{-i}; d) | \mathcal{F}\right) - \frac{1}{N(1-p)}\sum_{i=1}^N \E\left((1-Z_i)\mu_i(0, \mathbf{Z}_{-i}; d) | \mathcal{F}\right)  + o_P(1) \\
\end{align*}
Therefore,
\begin{align*}
& \Var[\E(\hat{\tau}_{d, HA} | \mathcal{F})] \\
= & \Var\left[\frac{1}{Np}\sum_{i=1}^N \E\left(Z_i\mu_i(1, \mathbf{Z}_{-i}; d) | \mathcal{F}\right) - \frac{1}{N(1-p)}\sum_{i=1}^N \E\left((1-Z_i)\mu_i(0, \mathbf{Z}_{-i}; d) | \mathcal{F}\right)\right]  + o_P(N^{-1}) \\
= & \frac{1}{N^2} \Var\left[\sum_{i=1}^N \left(\mu_i(\Y(1, \Z_{-i}); d) - \mu_i(\Y(0, \Z_{-i}); d)\right)\right] + o_P(N^{-1})\\
\end{align*}
and
\begin{align*}
& \Var(\hat{\tau}_{d, HA}) \\
\leq & \frac{1}{N^2p}\sum_{i=1}^N \E\left[\left(\mu_i(\Y(1, \Z_{-i}); d) - \bar {\mu}_1^0\right)^2\right] + \frac{1}{N^2(1-p)}\sum_{i=1}^N \E\left[\left(\mu_i(\Y(0, \Z_{-i}); d)- \bar {\mu}_0^0\right)^2\right] \\
+ & \frac{1}{N^2} \sum_{i=1} \sum_{j \in \mathbf{B}(i)}\{ \Cov[\mu_i(\Y(1, \Z_{-i}); d), \mu_j(\Y(1, \Z_{-j}); d)] - \Cov[\mu_i(\Y(1, \Z_{-i}); d), \mu_j(\Y(0, \Z_{-j}); d)] \\
- & \Cov[\mu_i(\Y(0, \Z_{-i}); d), \mu_j(\Y(1, \Z_{-j}); d)] + \Cov[\mu_i(\Y(0, \Z_{-i}); d), \mu_j(\Y(0, \Z_{-j}); d)] \} + o_P(N^{-1}).
\end{align*}

Our estimation of $\tau_d$ could be seen as a two-step process. In the first step, we construct the circle mean for each intervention node: $\mu_i(d) = \frac{\sum_x \mathbf{1}\{d_{ix} = d\}Y_x}{\sum_x \mathbf{1}\{d_{ix} = d\}}$. In the second step, we apply the Horvitz-Thompson estimator or the Hajek estimator to all the $(Z_i, \mu_i)$.

It is well-known that regression could be used to generate unbiased estimate of the average treatment effect in experiments. Treating $\mu_i(d)$ as nuisance parameters, we can estimate the following regression equation:

\begin{align*}
\mu_i(d) = \alpha + \tau_d Z_i + \varepsilon_i(d).
\end{align*}

It is easy to show that under OLS, $\hat{\alpha} = \frac{1}{N_0}\sum_{i=1}^{N} (1-Z_i) \mu_i(d) = \bar{\mu}_0(d)$ and $\hat{\tau}_{d, OLS} = \frac{1}{N_1}\sum_{i=1}^{N} Z_i \mu_i(d) - \frac{1}{N_0}\sum_{i=1}^{N} (1-Z_i) \mu_i(d) = \bar{\mu}_1(d) - \bar{\mu}_0(d)$, where $N_0 = \sum_{i=1}^{N} (1-Z_i)$ and $N_1 = \sum_{i=1}^{N}Z_i$. Clearly, $\hat{\tau}_{d, OLS} = \hat{\tau}_{d, HA}$. Then the residual for each observation $\hat{e}_i = \mu_i - \hat{\alpha} - \hat{\tau}_{d, OLS} Z_i = \mu_i - \bar{\mu}_0(d) - [\bar{\mu}_1(d) - \bar{\mu}_0(d)] Z_i $. The strong law of large numbers renders that as $N \rightarrow \infty$, $\bar{\mu}_1(d) \overset{a.s.}{\rightarrow} \frac{\sum_{i=1}^N \E\left[\mu_i (1,\mathbf{Z}_{-i};d) \right]}{N}$ and $\bar{\mu}_0(d) \overset{a.s.}{\rightarrow} \frac{\sum_{i=1}^N \E\left[\mu_i (0,\mathbf{Z}_{-i};d) \right]}{N}$.

Denote $\begin{pmatrix}
1, Z_1 \\
1, Z_2 \\
\dots \\
1, Z_N
\end{pmatrix}$ as $\mathbf{X}$, the spatial HAC standard errors of $(\hat{\alpha}, \hat{\tau}_{d, OLS})$ can be expressed as:

\begin{align*}
\sigma \begin{pmatrix}
\hat{\alpha} \\
\hat{\tau}_{d, OLS}
\end{pmatrix} = & \sqrt{\Var \begin{pmatrix}
\hat{\alpha} \\
\hat{\tau}_{d, OLS}
\end{pmatrix}} \\
 \widehat{\Var} \begin{pmatrix}
\hat{\alpha} \\
\hat{\tau}_{d, OLS}
\end{pmatrix} = & (\mathbf{X}' \mathbf{X})^{-1}(\mathbf{X}' \Sigma \mathbf{X})(\mathbf{X}' \mathbf{X})^{-1} \\
= & \begin{pmatrix}
N, N_1 \\
N_1, N_1
\end{pmatrix}^{-1}\left(\sum_{i=1}^N \sum_{j=1}^N \mathbf{X}_{i} \mathbf{X}_{j}^{'}\hat{e}_i \hat{e}_j \mathbf{1}\{j \in \mathcal{B}(i) \}\right)\begin{pmatrix}
N, N_1 \\
N_1, N_1
\end{pmatrix}^{-1} \\
= & \frac{1}{N_1^2 N_0^2}\begin{pmatrix}
N_1, -N_1 \\
-N_1, N
\end{pmatrix}\left(\sum_{i=1}^N \sum_{j=1}^N \begin{pmatrix}
1, Z_j \\
Z_i, Z_i Z_j
\end{pmatrix}\hat{e}_i \hat{e}_j \mathbf{1}\{j \in \mathcal{B}(i) \}\right)\begin{pmatrix}
N_1, -N_1 \\
-N_1, N
\end{pmatrix}
\end{align*}
Note that the $(2,2)$ entry of $\begin{pmatrix}
N_1, -N_1 \\
-N_1, N
\end{pmatrix} \begin{pmatrix}
1, Z_j \\
Z_i, Z_i Z_j
\end{pmatrix} \begin{pmatrix}
N_1, -N_1 \\
-N_1, N
\end{pmatrix}$ equals to $N_1^2 - N_1 N Z_i - - N_1 N Z_j + N^2 Z_i Z_j$. Rearrange the sample such that treated observations lie before observations under control and plug in the expression of $\hat{e}_i$ , we can see that:
\begin{align*}
\widehat{\Var}(\hat{\tau}_{d, OLS}) = & \frac{1}{N_1^2} \sum_{i=1}^{N_1} \hat{e}_i^2 + \frac{1}{N_0^2} \sum_{i=N_1+1}^{N} \hat{e}_i^2 + \frac{1}{N_1^2} \sum_{i=1}^{N_1} \sum_{j \neq i, Z_j = 1}\hat{e}_i\hat{e}_j \\
- & \frac{1}{N_1 N_0} \sum_{i=1}^{N_1} \sum_{j \neq i, Z_j = 0}\hat{e}_i\hat{e}_j - \frac{1}{N_1 N_0} \sum_{i=N_1+1}^{N} \sum_{j \neq i, Z_j = 1}\hat{e}_i\hat{e}_j  + \frac{1}{N_0^2} \sum_{i=N_1+1}^{N} \sum_{j \neq i, Z_j = 0}\hat{e}_i\hat{e}_j \\
= & \frac{1}{N_1^2} \sum_{i=1}^{N_1} \left(\mu_i (d) - \bar{\mu}_1 (d)\right)^2 + \frac{1}{N_0^2} \sum_{i=N_1+1}^{N} \left(\mu_i (d) - \bar{\mu}_0 (d)\right)^2  \\
+ & \frac{1}{N_1^2} \sum_{i=1}^{N_1} \sum_{j \in \mathcal{B}(i), Z_j = 1} \left(\mu_i (d) - \bar{\mu}_1 (d)\right) \left(\mu_j (d) - \bar{\mu}_1 (d)\right) \\
- & \frac{1}{N_1 N_0} \sum_{i=1}^{N_1} \sum_{j \in \mathcal{B}(i), Z_j = 0} \left(\mu_i (d) - \bar{\mu}_1 (d)\right) \left(\mu_j (d) - \bar{\mu}_0 (d)\right) \\
- & \frac{1}{N_1 N_0} \sum_{i=N_1+1}^{N} \sum_{j \in \mathcal{B}(i), Z_j = 1} \left(\mu_i (d) - \bar{\mu}_0 (d)\right) \left(\mu_j (d) - \bar{\mu}_1 (d)\right) \\
+ & \frac{1}{N_0^2} \sum_{i=N_1+1}^{N} \sum_{j \in \mathcal{B}(i), Z_j = 0} \left(\mu_i (d) - \bar{\mu}_0 (d)\right) \left(\mu_j (d) - \bar{\mu}_0 (d)\right)
\end{align*}

Finally, we show that the variance estimate $\widehat{\Var}(\hat{\tau}_{d, OLS})$ is asymptotically unbiased for the true variance of the Hajek estimator: $\Var(\hat{\tau}_{d, HA})$. Note that the first part in the true variance for the Hajek estimator can be written as:
\begin{align*}
& \frac{1}{N^2p}\sum_{i=1}^N \E\left[\left(\mu_i(\Y(1, \Z_{-i}); d)- \bar {\mu}_1^0\right)^2\right] \\
= & \frac{1}{N^2p}\sum_{i=1}^N \E\left[\mu_i^2(\Y(1, \Z_{-i}); d)\right] - \frac{2}{N^2p}\sum_{i=1}^N \E\left[\mu_i(\Y(1, \Z_{-i}); d)\frac{1}{N}\sum_{i=1}^N \mu_i(\Y(1, \Z_{-i}); d)\right] \\
& + \frac{1}{N^2p}\sum_{i=1}^N \E\left[\left(\frac{1}{N}\sum_{i=1}^N \mu_i(\Y(1, \Z_{-i}); d)\right)^2\right] \\
= & \frac{1}{N^2p}\sum_{i=1}^N \E\left[\mu_i^2(\Y(1, \Z_{-i}); d)\right]  - \frac{1}{N^3p} \E\left[\left(\sum_{i=1}^N \mu_i(\Y(1, \Z_{-i}); d)\right)^2\right] \\
= & \frac{1}{N^2p}(1-\frac{1}{N})\sum_{i=1}^N \E\left[\mu_i^2(\Y(1, \Z_{-i}); d)\right] - \frac{1}{N^3p}\sum_{i=1}^N \sum_{j\neq i}^N \E\left[\mu_i(\Y(1, \Z_{-i}); d)\mu_j(\Y(1, \Z_{-j}); d)\right]
\end{align*}

Taking expectation on the first term of the variance estimate, we have:
% Note that $\E\left[\frac{N_1^2}{N^2} \right] = p$, 
%\begin{align*}
%& \E\left[ \sum_{i=1}^{N_1} \left(\mu_i (d) - \bar{\mu}_1 (d)\right)^2\right] \\
%= & \E\left[ \sum_{i=1}^{N} Z_i\left(\mu_i (1, \mathbf{Z}_{-i};d) - \bar{\mu}_1 (d)\right)^2\right] \\
%= & \sum_{i=1}^{N}\E\left[Z_i \left(\mu_i (1, \mathbf{Z}_{-i};d) - \bar{\mu}_1 (d)\right)^2\right] \\
%= & p\sum_{i=1}^{N}\E\left[\left(\mu_i (1, \mathbf{Z}_{-i};d) - \bar{\mu}_1 (d)\right)^2\right]
%\end{align*}
%and $\E\left[ N_1^2\right] = N^2 p^2$. Therefore,
%\begin{align*}
%& \E\left[\frac{1}{N_1^2} \sum_{i=1}^{N_1} \left(\mu_i (d) - \bar{\mu}_1 (d)\right)^2\right] \\
%\rightarrow & \frac{p\sum_{i=1}^{N}\E\left[\left(\mu_i (1, \mathbf{Z}_{-i};d) - \bar{\mu}_1 (d)\right)^2\right]}{N^2 p^2}  \\
%= & \frac{1}{N^2 p}\sum_{i=1}^{N}\E\left[\left(\mu_i (1, \mathbf{Z}_{-i};d) - \bar{\mu}_1 (d)\right)^2 \right]
%\end{align*}
%Similarly,
%\begin{align*}
%& \E\left[\frac{1}{N_0^2} \sum_{i=N_1+1}^{N} \left(\mu_i (d) - \bar{\mu}_1 (d)\right)^2\right] \\
%\rightarrow & \frac{(1-p)\sum_{i=1}^{N}\E\left[\left(\mu_i (0, \mathbf{Z}_{-i};d) - \bar{\mu}_0 (d)\right)^2\right]}{N^2 (1-p)^2}  \\
%= & \frac{1}{N^2 (1-p)}\sum_{i=1}^{N}\E\left[\left(\mu_i (0, \mathbf{Z}_{-i};d) - \bar{\mu}_0 (d)\right)^2 \right]
%\end{align*}
%and
%\begin{align*}
%& \E\left[\frac{1}{N_1^2} \sum_{i=1}^{N_1} \sum_{j \in \mathcal{B}(i), Z_j = 1} \left(\mu_i (d) - \bar{\mu}_1 (d)\right) \left(\mu_j (d) - \bar{\mu}_1 (d)\right)\right] \\
%\rightarrow & \frac{p^2 \sum_{i=1}^{N}\E\left[\left(\mu_i (d) - \bar{\mu}_1 (d)\right) \left(\mu_j (d) - \bar{\mu}_1 (d)\right)\right]}{N^2 p^2}  \\
%= & \frac{1}{N^2}\sum_{i=1}^{N}\E\left[\left(\mu_i (d) - \bar{\mu}_1 (d)\right) \left(\mu_j (d) - \bar{\mu}_1 (d)\right)\right]
%\end{align*}
\begin{align*}
& \E\left[\frac{1}{N_1^2} \sum_{i=1}^{N_1} \left(\mu_i (1, \mathbf{Z}_{-i};d) - \bar{\mu}_1 (d)\right)^2\right] \\
= & \E\left[\frac{1}{N_1^2} \left(\sum_{i=1}^{N_1} \mu_i^2 (1, \mathbf{Z}_{-i};d) - 2\bar{\mu}_1 (d)\sum_{i=1}^{N_1}\mu_i (1, \mathbf{Z}_{-i};d) + \sum_{i=1}^{N_1}(\bar{\mu}_1 (d))^2 \right)\right] \\
= & \E\left[\frac{1}{N_1^2} \left(\sum_{i=1}^{N_1} \mu_i^2 (1, \mathbf{Z}_{-i};d) - N_1\bar{\mu}_1^2 (d)\right)\right] \\
= & \E\left[\frac{1}{N_1^2} \sum_{i=1}^{N_1} \mu_i^2 (1, \mathbf{Z}_{-i};d) \right] - \E\left[\frac{1}{N_1}\bar{\mu}_1^2 (d)\right] \\
= & \E\left[\frac{1}{N_1^2}(1-\frac{1}{N_1}) \sum_{i=1}^{N_1} \mu_i^2 (1, \mathbf{Z}_{-i};d) \right] - \E\left[\frac{1}{N_1^3}\sum_{i=1}^{N_1}\sum_{j\neq i}^{N_1} \mu_i (1, \mathbf{Z}_{-i};d) \mu_j (1, \mathbf{Z}_{-j};d)\right] \\
= & \frac{1}{N^2p^2}(1-\frac{1}{N}) \sum_{i=1}^{N} \E\left[  Z_i\mu_i^2 (1, \mathbf{Z}_{-i};d)\right] - \frac{1}{N^3p^3}\sum_{i=1}^{N}\sum_{j\neq i}^{N} \E\left[  Z_iZ_j\mu_i (Z_i, \mathbf{Z}_{-i};d) \mu_j (Z_j, \mathbf{Z}_{-j};d)\right] + o_P(1) \\
= & \frac{1}{N^2p}(1-\frac{1}{N}) \sum_{i=1}^{N} \E\left[ \mu_i^2 (1, \mathbf{Z}_{-i};d)\right] - \frac{1}{N^3p}\sum_{i=1}^{N}\sum_{j\neq i}^{N} \E\left[  \mu_i (1,1, \mathbf{Z}_{-(i,j)};d) \mu_j (1, 1,\mathbf{Z}_{-(i,j)};d)\right]  + o_P(1)
\end{align*}
which is the first part of the Hajek estimator's variance when the sample size is large.

The second part can be shown to be asymptotically unbiased in the same way. Now consider the first covariance part in the true variance, we have:
\begin{align*}
& \frac{1}{N^2} \sum_{i=1} \sum_{j \in \mathbf{B}(i)} \Cov[\mu_i(\Y(1, \Z_{-i}); d), \mu_j(\Y(1, \Z_{-j}); d)] \\
= & \frac{1}{N^2} \sum_{i=1} \sum_{j \in \mathbf{B}(i)} \E[\mu_i(\Y(1, \Z_{-i}); d)\mu_j(\Y(1, \Z_{-j}); d)] \\
& - \frac{1}{N^2} \sum_{i=1}\E[\mu_i(\Y(1, \Z_{-i}); d)] \sum_{j \in \mathbf{B}(i)} \E[\mu_j(\Y(1, \Z_{-j}); d)]. 
\end{align*}.

Notice that $\sum_{i=1}^{N_1}\sum_{j \in \mathcal{B}(i), Z_j = 1} \mu_i (d) = \sum_{i=1}^{N_1}\sum_{j \in \mathcal{B}(i), Z_j = 1} \mu_j (d) = \sum_{i=1}^{N_1} c_i^1 \mu_i (d)$, where $c_i^1 = \sum_{j \in \mathcal{B}(i)} Z_j$ is the number of treated nodes that depend on node $i$. It is easy to see that $\frac{c_i^1}{c_i} = \frac{\sum_{j \in \mathcal{B}(i) } Z_j}{c_i} = p + o_P(N^{-1/2})$.  The expectation of the corresponding estimate equals to:
\begin{align*}
&\E\left[ \frac{1}{N_1^2} \sum_{i=1}^{N_1} \sum_{j \in \mathcal{B}(i), Z_j = 1} \left(\mu_i (d) - \bar{\mu}_1 (d)\right) \left(\mu_j (d) - \bar{\mu}_1 (d)\right)\right]\\
= & \E\left[ \frac{1}{N^2p^2} \sum_{i=1}^{N_1} \sum_{j \in \mathcal{B}(i), Z_j = 1} \left(\mu_i (d) - \bar{\mu}_1 (d)\right) \left(\mu_j (d) - \bar{\mu}_1 (d)\right)\right]  + o_P(1) \\
= & \frac{1}{N^2 p^2} \sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)} \E \left[Z_iZ_j\mu_i (d)\mu_j (d)\right] \\
& - \frac{1}{N^2 p^2} \E \left[\sum_{i=1}^{N_1}\sum_{j \in \mathcal{B}(i), Z_j = 1} \bar{\mu}_1 (d) \left(\mu_i (d) - \bar{\mu}_1 (d) +\mu_j (d)\right) \right]  + o_P(1) \\
= & \frac{1}{N^2} \sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)} \E \left[\mu_i (1, 1, \mathbf{Z}_{-(i,j)};d)\mu_j (1, 1, \mathbf{Z}_{-(i,j)};d)\right] \\
& - \frac{1}{N^2 p^2} \E \left[\bar{\mu}_1 (d) \sum_{i=1}^{N_1}\left(2c_i^1  -  \frac{\sum_{i=1}^{N_1}c_i^1}{N_1} \right)\mu_i (d)\right]  + o_P(1) 
\end{align*}
The first part is exactly the corresponding term in the covariance's expression. For the second part to be asymptotically unbiased, we need an extra assumption on the asymptotic homogeneity of the dependency graph: $c_i = \tilde{c} + o_P(N^{-1})$ and $\sum_{j \in \mathbf{B}(i)} \E[\mu_j(\Y(1, \Z_{-j}); d)] = \frac{\sum_{i=1}^N\sum_{j \in \mathbf{B}(i)} \E[\mu_j(\Y(1, \Z_{-j}); d)] }{N}  + o_P(1)$. Under this assumption, $\frac{\sum_{i=1}^{N_1}c_i^1}{N_1} = \tilde{c} + o_P(N^{-1})$ and $\sum_{i=1}^{N_1}\left(2c_i^1  -  \frac{\sum_{i=1}^{N_1}c_i^1}{N_1} \right)\mu_i (d) = \sum_{i=1}^{N_1}\tilde{c}p\mu_i (d) + o_P(1)$. Moreover,
\begin{align*}
& \frac{1}{N^2} \sum_{i=1}\E[\mu_i(\Y(1, \Z_{-i}); d)] \sum_{j \in \mathbf{B}(i)} \E[\mu_j(\Y(1, \Z_{-j}); d)] \\
= & \left(\frac{1}{N} \sum_{i=1}\E[\mu_i(\Y(1, \Z_{-i}); d)]\right)\left(\frac{1}{N^2} \sum_{i=1} \sum_{j \in \mathbf{B}(i)} \E[\mu_j(\Y(1, \Z_{-j}); d)]\right) + o_P(1) \\
= & \left(\frac{1}{N} \sum_{i=1}\E[\mu_i(\Y(1, \Z_{-i}); d)]\right)\left(\frac{\tilde{c}}{N^2} \sum_{i=1} \E[\mu_j(\Y(1, \Z_{-j}); d)]\right) + o_P(1).
\end{align*}.
Remeber that $\bar{\mu}_1 (d) = \frac{1}{N} \sum_{i=1}\E[\mu_i(\Y(1, \Z_{-i}); d)] + o_P(1)$, we have:
\begin{align*}
& \frac{1}{N^2 p^2} \E \left[\bar{\mu}_1 (d) \sum_{i=1}^{N_1}\left(2c_i^1  -  \frac{\sum_{i=1}^{N_1}c_i^1}{N_1} \right)\mu_i (d)\right]  + o_P(1)  \\
= & \frac{1}{N^2 p^2} \E \left[\bar{\mu}_1 (d) \sum_{i=1}^{N_1}\tilde{c}p\mu_i (d)\right]  + o_P(1)  \\
= & \left(\frac{1}{N} \sum_{i=1}\E[\mu_i(\Y(1, \Z_{-i}); d)]\right)  \frac{1}{N^2 p^2} \E \left[\sum_{i=1}^{N_1}\tilde{c}p \mu_i (d)\right]  + o_P(1)  \\
= & \left(\frac{1}{N} \sum_{i=1}\E[\mu_i(\Y(1, \Z_{-i}); d)]\right)  \left(\frac{\tilde{c}}{N^2} \sum_{i=1} \E[\mu_j(\Y(1, \Z_{-j}); d)]\right) + o_P(1).
\end{align*}
%\begin{align*}
%&\E\left[ \frac{1}{N_1^2} \sum_{i=1}^{N_1} \sum_{j \in \mathcal{B}(i), Z_j = 1} \left(\mu_i (1, \mathbf{Z}_{-i};d) - \bar{\mu}_1 (d)\right) \left(\mu_j (1, \mathbf{Z}_{-j};d) - \bar{\mu}_1 (d)\right)\right]\\
%= & \frac{1}{N^2 p^2} \sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)} \E \left[Z_i\left(\mu_i (1, \mathbf{Z}_{-i};d) - \bar{\mu}_1 (d)\right)Z_j \left(\mu_j (1, \mathbf{Z}_{-j};d) - \bar{\mu}_1 (d)\right)\right]  + o_P(1) \\
%= & \frac{1}{N^2 p^2} \sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)} \E \left[Z_iZ_j\mu_i (1, \mathbf{Z}_{-i};d)\mu_j (1, \mathbf{Z}_{-j};d)\right] - \frac{1}{N^2 p^2} \sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)} \E \left[Z_iZ_j\mu_i (1, \mathbf{Z}_{-i};d)\bar{\mu}_1 (d)\right] \\
%& - \frac{1}{N^2 p^2} \sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)} \E \left[Z_iZ_j\mu_j (1, \mathbf{Z}_{-j};d)\bar{\mu}_1 (d)\right] + \frac{1}{N^2 p^2} \sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)} \E \left[Z_iZ_j\bar{\mu}_1^2 (d)\right]  + o_P(1) \\
%= & \frac{1}{N^2} \sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)} \E \left[\mu_i (1, 1, \mathbf{Z}_{-(i,j)};d)\mu_j (1, 1, \mathbf{Z}_{-(i,j)};d)\right] \\
%& - \frac{1}{N^2 p^2} \sum_{i=1}^{N}\E \left[\bar{\mu}_1 (d) \sum_{j \in \mathcal{B}(i)} Z_iZ_j\left(\mu_i (1, \mathbf{Z}_{-i};d) - \bar{\mu}_1 (d) +\mu_j (1, \mathbf{Z}_{-j};d)\right) \right]  + o_P(1) \\
%\end{align*}
%= & \frac{1}{N^2} \sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)} \E \left[\mu_i (1, \mathbf{Z}_{-i};d)\mu_j (1, \mathbf{Z}_{-j};d)\right] - \frac{1}{N^3 p^3} \sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)} \sum_{k=1}^{N} \E \left[Z_iZ_jZ_k\mu_i (1, \mathbf{Z}_{-i};d)\mu_k (1, \mathbf{Z}_{-k};d)\right] \\
%& - \frac{1}{N^3 p^3} \sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)}\sum_{k=1}^{N} \E \left[Z_iZ_jZ_k\mu_j (1, \mathbf{Z}_{-j};d)\mu_k (1, \mathbf{Z}_{-k};d)\right] + \frac{1}{N^2 p^2} \sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)} \E \left[Z_iZ_j\bar{\mu}_1^2 (d)\right] \\
%= & \frac{1}{N^2} \sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)} \E \left[\mu_i (1, \mathbf{Z}_{-i};d)\mu_j (1, \mathbf{Z}_{-j};d)\right] - \frac{1}{N^3 p} \sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)} \E \left[\mu_i (1, 1, 1, \mathbf{Z}_{-i};d)\mu_k (1, \mathbf{Z}_{-k};d)\right] \\
%When $N \rightarrow \infty$, we can apply the dominated convergence theorem to the second term above, then:
%\begin{align*}
%& \lim_{N \rightarrow \infty} \frac{1}{N^2 p^2} \sum_{i=1}^{N}\E \left[\bar{\mu}_1 (d) \sum_{j \in \mathcal{B}(i)} Z_iZ_j\left(\mu_i (1, \mathbf{Z}_{-i};d) - \bar{\mu}_1 (d) +\mu_j (1, \mathbf{Z}_{-j};d)\right) \right] \\
%= & \frac{1}{N^2 p^2} \sum_{i=1}^{N}\E \left[\lim_{N \rightarrow \infty} \bar{\mu}_1 (d) \sum_{j \in \mathcal{B}(i)} Z_iZ_j\left(\mu_i (1, \mathbf{Z}_{-i};d) - \bar{\mu}_1 (d) +\mu_j (1, \mathbf{Z}_{-j};d)\right) \right] \\
%= & \frac{1}{N^2 p^2} \sum_{i=1}^{N} \E\left[\mu_i(1, \mathbf{Z}_{-i};d) \right] \E \left[ \sum_{j \in \mathcal{B}(i)} Z_iZ_j\left(\mu_i (1, \mathbf{Z}_{-i};d) - \E\left[\mu_i(1, \mathbf{Z}_{-i};d) \right] +\mu_j (1, \mathbf{Z}_{-j};d)\right) \right] \\
%= & \frac{1}{N^2} \sum_{i=1}^{N} \E\left[\mu_i(1, \mathbf{Z}_{-i};d) \right] \sum_{j \in \mathcal{B}(i)} \E \left[ \mu_j (1,1, \mathbf{Z}_{-(i,j)};d) \right] \\
%\end{align*}

%(What remains to be shown here is that $\sum_{i=1}^N \sum_{j\neq i}^N \E\left[\mu_i(\Y(1, \Z_{-i}); d)\mu_j(\Y(1, \Z_{-j}); d)\right] = \sum_{i=1}^N \sum_{j\neq i}^N \E\left[\mu_i(\Y(1, 1, \Z_{-(i,j)}); d)\mu_j(\Y(1, 1, \Z_{-(i,j)}); d)\right]$).

The other terms can be similarly shown. Hence, the spatial HAC variance is an unbiased estimate of the Hajek estimator's variance when $N$ is sufficiently large.
\end{document}




==> proofs/reference/variance_expression2.tex <==
\input{tex-header}
\begin{document}
\section{Variance of the Horvitz-Thompson estimator}
We start from the Horvitz-Thompson estimator:
$$\hat{\tau}_{HT}(d) = \frac{1}{Np}\sum_{i=1}^N Z_i \mu_i(\Y(\Z); d) - \frac{1}{N(1-p)}\sum_{i=1}^N (1-Z_i) \mu_i(\Y(\Z); d).
$$
We know that 
\begin{align*}
\E\left[ \hat{\tau}_{HT}(d)\right] = & \E\left[ \frac{1}{Np}\sum_{i=1}^N Z_i \mu_i(\Y(\Z); d) - \frac{1}{N(1-p)}\sum_{i=1}^N (1-Z_i) \mu_i(\Y(\Z); d)\right] \\
= &\frac{1}{N} \E\left[\sum_{i=1}^N \mu_i(\Y(1, \Z_{-i}); d) - \sum_{i=1}^N\mu_i(\Y(0, \Z_{-i}); d)\right] \\
= & \tau(d).
\end{align*}
Hence,
\begin{align*}
& \Var\left[\hat{\tau}_{HT}(d) \right] \\
= &\frac{1}{N^2} \Var\left[\sum_{i=1}^N \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y(\Z); d) \right] \\
= & \frac{1}{N^2} \sum_{i=1}^N \Var\left[ \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y(\Z); d) \right] \\
& + \frac{1}{N^2} \sum_{i=1}^N \sum_{j \neq i} \Cov\left[ \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y(\Z); d), \left(\frac{Z_j}{p} - \frac{1-Z_j}{1-p}\right)\mu_j(\Y(\Z); d) \right] \\
= & \frac{1}{N^2} \sum_{i=1}^N \E\left[ \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y(\Z); d) \right]^2 - \frac{1}{N^2} \sum_{i=1}^N \E^2\left[ \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y(\Z); d) \right] \\
& + \frac{1}{N^2} \sum_{i=1}^N \sum_{j \neq i} \Cov\left[ \frac{Z_i}{p}\mu_i(\Y(\Z); d), \frac{Z_j}{p} \mu_j(\Y(\Z); d) \right] \\
& - \frac{1}{N^2} \sum_{i=1}^N \sum_{j \neq i} \Cov\left[ \frac{Z_i}{p}\mu_i(\Y(\Z); d), \frac{1-Z_j}{1-p} \mu_j(\Y(\Z); d) \right] \\
& - \frac{1}{N^2} \sum_{i=1}^N \sum_{j \neq i} \Cov\left[ \frac{1-Z_i}{1-p}\mu_i(\Y(\Z); d), \frac{Z_j}{p} \mu_j(\Y(\Z); d) \right] \\
& + \frac{1}{N^2} \sum_{i=1}^N \sum_{j \neq i} \Cov\left[ \frac{1-Z_i}{1-p}\mu_i(\Y(\Z); d), \frac{1-Z_j}{1-p} \mu_j(\Y(\Z); d) \right].
\end{align*}

The first two terms can be further expanded as
\begin{align*}
& \frac{1}{N^2} \sum_{i=1}^N \E\left[ \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y(\Z); d) \right]^2 - \frac{1}{N^2} \sum_{i=1}^N \E^2\left[ \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y(\Z); d) \right] \\
= & \frac{1}{N^2} \sum_{i=1}^N \E\left[ \frac{Z_i^2}{p^2} \mu_i^2(\Y(\Z); d) \right] + \frac{1}{N^2} \sum_{i=1}^N \E\left[ \frac{(1-Z_i)^2}{(1-p)^2} \mu_i^2(\Y(\Z); d) \right] \\
& - \frac{1}{N^2} \sum_{i=1}^N \E^2\left[ \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y(\Z); d) \right] \\
= & \frac{1}{N^2p} \sum_{i=1}^N \E\left[\mu_i^2(\Y(1, \Z_{-i}); d) \right] + \frac{1}{N^2(1-p)} \sum_{i=1}^N \E\left[ \mu_i^2(\Y(0, \Z_{-i}); d) \right] \\
& - \frac{1}{N^2} \sum_{i=1}^N \E^2\left[ \mu_i(\Y(1, \Z_{-i}); d) - \mu_i(\Y(0, \Z_{-i}); d) \right] \\
\leq & \frac{1}{N^2p} \sum_{i=1}^N \E\left[\mu_i^2(\Y(1, \Z_{-i}); d) \right] + \frac{1}{N^2(1-p)} \sum_{i=1}^N \E\left[ \mu_i^2(\Y(0, \Z_{-i}); d) \right].
\end{align*}
The first covariance term equals to
\begin{align*}
& \frac{1}{N^2} \sum_{i=1}^N \sum_{j \neq i} \Cov\left[ \frac{Z_i}{p}\mu_i(\Y(\Z); d), \frac{Z_j}{p} \mu_j(\Y(\Z); d) \right] \\
= & \frac{1}{N^2} \sum_{i=1}^N \sum_{j \neq i} \E\left[ \frac{Z_i Z_j}{p^2}\mu_i(\Y(\Z); d) \mu_j(\Y(\Z); d) \right] - \frac{1}{N^2} \sum_{i=1}^N \sum_{j \neq i} \E\left[ \frac{Z_i}{p}\mu_i(\Y(\Z); d) \right]\E\left[ \frac{Z_j}{p}\mu_j(\Y(\Z); d) \right] \\
= & \frac{1}{N^2} \sum_{i=1}^N \sum_{j \neq i} \E\left[\mu_i(\Y(1,1,\Z_{-(i,j)}); d) \mu_j(\Y(1,1,\Z_{-(i,j)}); d) \right] \\
& - \frac{1}{N^2} \sum_{i=1}^N \sum_{j \neq i} \E\left[\mu_i(\Y(1,\Z_{-i}); d) \right]\E\left[\mu_j(\Y(1, \Z_{-i}); d) \right] \\
= & \frac{1}{N^2} \sum_{i=1}^N \sum_{j \neq i} \Cov\left[\mu_i(\Y(1,\Z_{-i}); d), \mu_j(\Y(1,\Z_{-j}); d) \right] \\
= & \frac{1}{N^2} \sum_{i=1}^N \sum_{j \in \mathcal{B}(i)} \Cov\left[\mu_i(\Y(1,\Z_{-i}); d), \mu_j(\Y(1,\Z_{-j}); d) \right].
%= & \frac{1}{N^2} \sum_{i=1}^N \sum_{j \in \mathcal{B}(i)} \Cov\left[\mu_i(\Y(1,1,\Z_{-(i,j)}); d), \mu_j(\Y(1,1,\Z_{-(i,j)}); d) \right] \\
%& + \frac{1}{N^2} \sum_{i=1}^N \sum_{j \neq i} \E\left[\mu_i(\Y(1,1,\Z_{-(i,j)}); d) \right]\E\left[\mu_j(\Y(1, 1, \Z_{-(i, j)}); d) \right] \\
%& - \frac{1}{N^2} \sum_{i=1}^N \sum_{j \neq i} \E\left[\mu_i(\Y(1,\Z_{-i}); d) \right]\E\left[\mu_j(\Y(1, \Z_{-i}); d) \right].
\end{align*}
The second to last equality holds since 
$$
\E\left[\mu_i(\Y(1,\Z_{-i}); d) \mu_j(\Y(1,\Z_{-j}); d) \right] = \E\left[\mu_i(\Y(1,1,\Z_{-(i,j)}); d) \mu_j(\Y(1,1,\Z_{-(i,j)}); d) \right].
$$

To sum up,
\begin{align*}
& \Var\left[\hat{\tau}_{HT}(d) \right] \\
\leq & \frac{1}{N^2p} \sum_{i=1}^N \E\left[\mu_i^2(\Y(1, \Z_{-i}); d) \right] + \frac{1}{N^2(1-p)} \sum_{i=1}^N \E\left[ \mu_i^2(\Y(0, \Z_{-i}); d) \right] \\
& + \frac{1}{N^2} \sum_{i=1}^N \sum_{j \in \mathcal{B}(i)} \Cov\left[\mu_i(\Y(1,\Z_{-i}); d), \mu_j(\Y(1,\Z_{-j}); d) \right] \\
& - \frac{1}{N^2} \sum_{i=1}^N \sum_{j \in \mathcal{B}(i)} \Cov\left[\mu_i(\Y(1,\Z_{-i}); d), \mu_j(\Y(0,\Z_{-j}); d) \right] \\
& - \frac{1}{N^2} \sum_{i=1}^N \sum_{j \in \mathcal{B}(i)} \Cov\left[\mu_i(\Y(0,\Z_{-i}); d), \mu_j(\Y(1,\Z_{-j}); d) \right] \\
& + \frac{1}{N^2} \sum_{i=1}^N \sum_{j \in \mathcal{B}(i)} \Cov\left[\mu_i(\Y(0,\Z_{-i}); d), \mu_j(\Y(0,\Z_{-j}); d) \right].
\end{align*}
%\begin{align*}
%& \Var\left[\hat{\tau}_{HT}(d) \right] \\
%\leq & \frac{1}{N^2p} \sum_{i=1}^N \E\left[\mu_i^2(\Y(1, \Z_{-i}); d) \right] + \frac{1}{N^2(1-p)} \sum_{i=1}^N \E\left[ \mu_i^2(\Y(0, \Z_{-i}); d) \right] \\
%& + \frac{1}{N^2} \sum_{i=1}^N \sum_{j \neq i} \E\left[\mu_i(\Y(1,1,\Z_{-(i,j)}); d) \mu_j(\Y(1,1,\Z_{-(i,j)}); d) \right] \\
%& - \frac{1}{N^2} \sum_{i=1}^N \sum_{j \neq i} \E\left[\mu_i(\Y(1,\Z_{-i}); d) \right]\E\left[\mu_j(\Y(1, \Z_{-i}); d) \right] \\
%& - \frac{1}{N^2} \sum_{i=1}^N \sum_{j \neq i} \E\left[\mu_i(\Y(1,0,\Z_{-(i,j)}); d) \mu_j(\Y(1,0,\Z_{-(i,j)}); d) \right] \\
%& + \frac{1}{N^2} \sum_{i=1}^N \sum_{j \neq i} \E\left[\mu_i(\Y(1,\Z_{-i}); d) \right]\E\left[\mu_j(\Y(0, \Z_{-i}); d) \right] \\
%& - \frac{1}{N^2} \sum_{i=1}^N \sum_{j \neq i} \E\left[\mu_i(\Y(0,1,\Z_{-(i,j)}); d) \mu_j(\Y(0,1,\Z_{-(i,j)}); d) \right] \\
%& + \frac{1}{N^2} \sum_{i=1}^N \sum_{j \neq i} \E\left[\mu_i(\Y(0,\Z_{-i}); d) \right]\E\left[\mu_j(\Y(1, \Z_{-i}); d) \right] \\
%& + \frac{1}{N^2} \sum_{i=1}^N \sum_{j \neq i} \E\left[\mu_i(\Y(0,0,\Z_{-(i,j)}); d) \mu_j(\Y(0,0,\Z_{-(i,j)}); d) \right] \\
%& - \frac{1}{N^2} \sum_{i=1}^N \sum_{j \neq i} \E\left[\mu_i(\Y(0,\Z_{-i}); d) \right]\E\left[\mu_j(\Y(0, \Z_{-i}); d) \right] .
%\end{align*}
\newpage
\section{Variance of the Hajek estimator}
Next, we derive the variance of the Hajek estimator:
$$\hat{\tau}_{HA}(d) = \frac{1}{N_1}\sum_{i=1}^N Z_i \mu_i(\Y(\Z); d) - \frac{1}{N_0}\sum_{i=1}^N (1-Z_i) \mu_i(\Y(\Z); d),
$$ where $N_1 = \sum_{i=1}^N Z_i$ and $N_0 = \sum_{i=1}^N (1-Z_i)$.

Denote $\frac{1}{Np}\sum_{i=1}^N Z_i \mu_i(\Y(\Z); d)$ as $\tilde{\mu}^1(d)$, $\frac{1}{N(1-p)}\sum_{i=1}^N (1-Z_i) \mu_i(\Y(\Z); d)$ as $\tilde{\mu}^0(d)$, $\frac{N_1}{Np}$ as $\tilde{N}_1$, $\frac{N_0}{N(1-p)}$ as $\tilde{N}_0$, and $\W = (\tilde{\mu}^1(d), \tilde{\mu}^0(d), \tilde{N}_1, \tilde{N}_0)$. Define $f(a, b, c, d) = \frac{a}{c} - \frac{b}{d}$. Then the Hajek estimator equals to $f(\tilde{\mu}^1(d), \tilde{\mu}^0(d), \tilde{N}_1, \tilde{N}_0) = f(\W)$.  We know that $\E \left[\tilde{\mu}^1(d) \right] = \frac{1}{N}\sum_{i=1}^N \E \left[\mu_i(\Y(1,\Z_{-i}); d) = \bar{\mu}^1(d)\right]$, $\E \left[\tilde{\mu}^0(d) \right] = \frac{1}{N}\sum_{i=1}^N \E \left[\mu_i(\Y(0,\Z_{-i}); d) = \bar{\mu}^0(d)\right]$, $\E[\tilde{N}_1] = \E[\tilde{N}_0] =1$. Thus, $\E[ \W] = (\bar{\mu}^1(d), \bar{\mu}^0(d)), 1, 1)$.

Using Taylor expansion, we have:
\begin{align*}
& \sqrt{N}\hat{\tau}_{HA}(d) = f(\tilde{\mu}^1(d), \tilde{\mu}^0(d), \tilde{N}_1, \tilde{N}_0) = \sqrt{N}f(\W) \\
= & \sqrt{N}f(\E[ \W]) + \sqrt{N}\frac{\partial f}{\partial \W}|_{\E[ \W]}(\W - \E[ \W]) + o_P(\sqrt{N}||\W - \E[ \W]||).
\end{align*}
Then,
\begin{align*}
& N \Var \left[\hat{\tau}_{HA}(d)\right] \\
= & N\E\left[ f(\W) - f(\E[ \W]) \right]^2  \\
= &  N\left(\frac{\partial f}{\partial \W}|_{\E[ \W]}\right)^{'}\E\left[\W - \E[ \W]\right]^2\frac{\partial f}{\partial \W}|_{\E[ \W]} + o_P(1)\\
= &  N\left(\frac{\partial f}{\partial \W}|_{\E[ \W]}\right)^{'}\Var\left[\W\right]\frac{\partial f}{\partial \W}|_{\E[ \W]} + o_P(1).
\end{align*}

It is easy to see that $\frac{\partial f}{\partial \W}|_{\E[ \W]} = (1, -1, -\bar{\mu}^1(d), \bar{\mu}^0(d))^{'}$, and

\begin{align*}
& \Var\left[\W\right] = \\
& \begin{pmatrix}
\Var\left[\tilde{\mu}^1(d)\right] & \Cov\left[\tilde{\mu}^1(d), \tilde{\mu}^0(d)\right] & \Cov\left[\tilde{\mu}^1(d), \tilde{N}_1\right] & \Cov\left[\tilde{\mu}^1(d), \tilde{N}_0\right] \\
\Cov\left[\tilde{\mu}^1(d), \tilde{\mu}^0(d)\right] & \Var\left[\tilde{\mu}^0(d)\right] & \Cov\left[\tilde{\mu}^0(d), \tilde{N}_1\right] & \Cov\left[\tilde{\mu}^0(d), \tilde{N}_0\right] \\
\Cov\left[\tilde{\mu}^1(d), \tilde{N}_1\right]  & \Cov\left[\tilde{\mu}^0(d), \tilde{N}_1\right] & \Var\left[\tilde{N}_1\right] & \Cov\left[\tilde{N}_1, \tilde{N}_0\right] \\
\Cov\left[\tilde{\mu}^1(d), \tilde{N}_0\right] & \Cov\left[\tilde{\mu}^0(d), \tilde{N}_0\right] & \Cov\left[\tilde{N}_1, \tilde{N}_0\right] & \Var\left[\tilde{N}_0\right]
\end{pmatrix} 
\end{align*}
%We can calculate each term in the matrix as follows:
%\begin{align*}
%& \Var\left[\tilde{\mu}^1(d)\right] \\
%= &  \frac{1}{N^2p} \sum_{i=1}^N \E\left[\mu_i^2(\Y(1, \Z_{-i}); d) \right] - \frac{1}{N^2} \sum_{i=1}^N \E^2\left[\mu_i(\Y(1, \Z_{-i}); d) \right] \\
%& + \frac{1}{N^2} \sum_{i=1}^N \sum_{j \in \mathcal{B}(i)} \Cov\left[\mu_i(\Y(1,\Z_{-i}); d), \mu_j(\Y(1,\Z_{-j}); d) \right]
%\end{align*}
%
%\begin{align*}
%& \Var\left[\tilde{\mu}^0(d)\right] \\
%= &  \frac{1}{N^2(1-p)} \sum_{i=1}^N \E\left[\mu_i^2(\Y(0, \Z_{-i}); d) \right] - \frac{1}{N^2} \sum_{i=1}^N \E^2\left[\mu_i(\Y(0, \Z_{-i}); d) \right] \\
%& + \frac{1}{N^2} \sum_{i=1}^N \sum_{j \in \mathcal{B}(i)} \Cov\left[\mu_i(\Y(0,\Z_{-i}); d), \mu_j(\Y(0,\Z_{-j}); d) \right].
%\end{align*}
%
%\begin{align*}
%& \Cov\left[\tilde{\mu}^1(d), \tilde{\mu}^0(d)\right] \\
%= & \frac{1}{N^2} \sum_{i=1}^N \sum_{j \in \mathcal{B}(i)} \Cov\left[\mu_i(\Y(1,\Z_{-i}); d), \mu_j(\Y(0,\Z_{-j}); d) \right] \\
%& - \frac{1}{N^2} \sum_{i=1}^N \E\left[\mu_i(\Y(1, \Z_{-i}); d) \right] \E\left[\mu_i(\Y(0, \Z_{-i}); d) \right] 
%\end{align*}
%
%\begin{align*}
%& \Cov\left[\tilde{\mu}^1(d), \tilde{N}_1\right] \\
%= & \frac{1}{N^2p} \sum_{i=1}^N \E\left[\mu_i(\Y(1, \Z_{-i}); d) \right] + \frac{1}{N^2} \sum_{i=1}^N \sum_{j\neq i} \E\left[\mu_i(\Y(1,1, \Z_{-(i,j)}); d) \right] \\
%& - \frac{1}{N} \sum_{i=1}^N \E\left[\mu_i(\Y(1, \Z_{-i}); d) \right]
%\end{align*}
%\begin{align*}
%& \Cov\left[\tilde{\mu}^1(d), \tilde{N}_1\right] \\
%= & \frac{1-p}{N^2p} \sum_{i=1}^N \E\left[\mu_i(\Y(1, \Z_{-i}); d) \right] \\
%& + \frac{1}{N^2} \sum_{i=1}^N \sum_{j\in \mathcal{B}(i)} \left(\E\left[\mu_i(\Y(1,1, \Z_{-(i,j)}); d) \right] - \E\left[\mu_i(\Y(1, \Z_{-i}); d) \right]\right)
%\end{align*}
%
%%\begin{align*}
%%& \Cov\left[\tilde{\mu}^0(d), \tilde{N}_0\right] \\
%%= & \frac{1}{N^2(1-p)} \sum_{i=1}^N \E\left[\mu_i(\Y(0, \Z_{-i}); d) \right] + \frac{1}{N^2} \sum_{i=1}^N \sum_{j\neq i} \E\left[\mu_i(\Y(0,0, \Z_{-(i,j)}); d) \right] \\
%%& - \frac{1}{N} \sum_{i=1}^N \E\left[\mu_i(\Y(0, \Z_{-i}); d) \right]
%%\end{align*}
%\begin{align*}
%& \Cov\left[\tilde{\mu}^0(d), \tilde{N}_0\right] \\
%= & \frac{p}{N^2(1-p)} \sum_{i=1}^N \E\left[\mu_i(\Y(0, \Z_{-i}); d) \right] \\
%& + \frac{1}{N^2} \sum_{i=1}^N \sum_{j\in \mathcal{B}(i)} \left(\E\left[\mu_i(\Y(0,0, \Z_{-(i,j)}); d) \right] - \E\left[\mu_i(\Y(0, \Z_{-i}); d) \right]\right)
%\end{align*}


%\begin{align*}
%& \Cov\left[\tilde{\mu}^1(d), \tilde{N}_0\right] \\
%= & \frac{1}{N^2} \sum_{i=1}^N \sum_{j\neq i} \E\left[\mu_i(\Y(1,0, \Z_{-(i,j)}); d) \right]  - \frac{1}{N} \sum_{i=1}^N \E\left[\mu_i(\Y(1, \Z_{-i}); d) \right]
%\end{align*}
%\begin{align*}
%& \Cov\left[\tilde{\mu}^1(d), \tilde{N}_0\right] \\
%= & -\frac{1}{N^2} \sum_{i=1}^N \E\left[\mu_i(\Y(1, \Z_{-i}); d) \right] \\
%& + \frac{1}{N^2} \sum_{i=1}^N \sum_{j\in \mathcal{B}(i)} \left(\E\left[\mu_i(\Y(1,0, \Z_{-(i,j)}); d) \right] - \E\left[\mu_i(\Y(1, \Z_{-i}); d) \right]\right)
%\end{align*}

%\begin{align*}
%& \Cov\left[\tilde{\mu}^0(d), \tilde{N}_1\right] \\
%= & \frac{1}{N^2} \sum_{i=1}^N \sum_{j\neq i} \E\left[\mu_i(\Y(0,1, \Z_{-(i,j)}); d) \right]  - \frac{1}{N} \sum_{i=1}^N \E\left[\mu_i(\Y(0, \Z_{-i}); d) \right]
%\end{align*}
%\begin{align*}
%& \Cov\left[\tilde{\mu}^0(d), \tilde{N}_1\right] \\
%= & -\frac{1}{N^2} \sum_{i=1}^N \E\left[\mu_i(\Y(0, \Z_{-i}); d) \right] \\
%& + \frac{1}{N^2} \sum_{i=1}^N \sum_{j\in \mathcal{B}(i)} \left(\E\left[\mu_i(\Y(0, 1, \Z_{-(i,j)}); d) \right] - \E\left[\mu_i(\Y(0, \Z_{-i}); d) \right]\right)
%\end{align*}
%
%\begin{align*}
%& \Var\left[\tilde{N}_1\right] = \frac{1-p}{Np}
%\end{align*}
%
%\begin{align*}
%& \Var\left[\tilde{N}_0\right] = \frac{p}{N(1-p)}
%\end{align*}
%
%\begin{align*}
%& \Cov\left[\tilde{N}_1, \tilde{N}_0\right] = -\frac{1}{N}
%\end{align*}

Therefore,
\begin{align*}
& N\left(\frac{\partial f}{\partial \W}|_{\E[ \W]}\right)^{'}\Var\left[\W\right]\frac{\partial f}{\partial \W}|_{\E[ \W]} \\
= & N\Var\left[\tilde{\mu}^1(d)\right] + N\Var\left[\tilde{\mu}^0(d)\right] + N\left(\bar{\mu}^1(d) \right)^2\Var\left[\tilde{N}_1\right]  + N\left(\bar{\mu}^0(d) \right)^2\Var\left[\tilde{N}_0\right]  \\
& -2N\Cov\left[\tilde{\mu}^1(d), \tilde{\mu}^0(d)\right] - 2N\bar{\mu}^1(d) \Cov\left[\tilde{\mu}^1(d), \tilde{N}_1\right] + 2N\bar{\mu}^0(d) \Cov\left[\tilde{\mu}^1(d), \tilde{N}_0\right] \\
& + 2N\bar{\mu}^1(d) \Cov\left[\tilde{\mu}^0(d), \tilde{N}_1\right] - 2N\bar{\mu}^0(d) \Cov\left[\tilde{\mu}^0(d), \tilde{N}_0\right] - 2N\left(\bar{\mu}^1(d) \bar{\mu}^0(d)\right)\Cov\left[ \tilde{N}_1, \tilde{N}_0\right] \\
= & N\Var\left[\tilde{\mu}^1(d) - \bar{\mu}^1(d) \tilde{N}_1\right] + N\Var\left[\tilde{\mu}^0(d) - \bar{\mu}^0(d) \tilde{N}_0\right] \\
& - 2N\Cov\left[\tilde{\mu}^1(d) - \bar{\mu}^1(d) \tilde{N}_1, \tilde{\mu}^0(d) - \bar{\mu}^0(d) \tilde{N}_0\right] 
\end{align*}

%And
%\begin{align*}
%& N\Var \left[\hat{\tau}_{HA}(d)\right]  \\
%= & N\E\left[\tilde{\mu}^1(d) - \bar{\mu}^1(d) \tilde{N}_1\right]^2 + N\E\left[\tilde{\mu}^0(d) - \bar{\mu}^0(d) \tilde{N}_0\right]^2 \\
%& - 2N\E\left[\left(\tilde{\mu}^1(d) - \bar{\mu}^1(d) \tilde{N}_1\right) \left(\tilde{\mu}^0(d) - \bar{\mu}^0(d) \tilde{N}_0\right)\right] + o_P(1) \\
%\end{align*}
where
\begin{align*}
& N\Var\left[\tilde{\mu}^1(d) - \bar{\mu}^1(d) \tilde{N}_1\right] \\
= & \frac{1}{Np^2}\Var\left[\sum_{i=1}^N Z_i\left(\mu_i(\Y(\Z); d) - \bar{\mu}^1(d) \right)\right] \\
= & \frac{1}{Np^2}\sum_{i=1}^N\Var\left[ Z_i\left(\mu_i(\Y(\Z); d) - \bar{\mu}^1(d) \right)\right] \\
& + \frac{1}{Np^2}\sum_{i=1}^N\sum_{j\neq i}\Cov\left[ Z_i\left(\mu_i(\Y(\Z); d) - \bar{\mu}^1(d) \right), Z_j\left(\mu_j(\Y(\Z); d) - \bar{\mu}^1(d) \right)\right] \\
= & \frac{1}{Np^2}\sum_{i=1}^N\E\left[ Z_i\left(\mu_i(\Y(\Z); d) - \bar{\mu}^1(d) \right)\right]^2 - \frac{1}{Np^2}\sum_{i=1}^N\E^2\left[ Z_i\left(\mu_i(\Y(\Z); d) - \bar{\mu}^1(d) \right)\right] \\
& + \frac{1}{Np^2}\sum_{i=1}^N\sum_{j\neq i}\E\left[ Z_iZ_j\left(\mu_i(\Y(\Z); d) - \bar{\mu}^1(d) \right)\left(\mu_j(\Y(\Z); d) - \bar{\mu}^1(d) \right)\right] \\
& - \frac{1}{Np^2}\sum_{i=1}^N\sum_{j\neq i}\E\left[ Z_i\left(\mu_i(\Y(\Z); d) - \bar{\mu}^1(d) \right)\right] \E\left[ Z_j\left(\mu_j(\Y(\Z); d) - \bar{\mu}^1(d) \right)\right] \\
= & \frac{1}{Np}\sum_{i=1}^N\E\left[\mu_i(\Y(1, \Z_{-i}); d) - \bar{\mu}^1(d) \right]^2  - \frac{1}{N}\sum_{i=1}^N\E^2\left[ \mu_i(\Y(1, \Z_{-i}); d) - \bar{\mu}^1(d) \right] \\
& + \frac{1}{N}\sum_{i=1}^N\sum_{j\neq i}\E\left[ \left(\mu_i(\Y(1, 1,\Z_{-(i,j)}); d) - \bar{\mu}^1(d) \right)\left(\mu_j(\Y(1, 1, \Z_{-(i,j)}); d) - \bar{\mu}^1(d) \right)\right] \\
& - \frac{1}{N}\sum_{i=1}^N\sum_{j\neq i}\E\left[\mu_i(\Y(1, \Z_{-i}); d) - \bar{\mu}^1(d) \right] \E\left[ \mu_j(\Y(1, \Z_{-j}); d) - \bar{\mu}^1(d) \right] \\
= & \frac{1}{Np}\sum_{i=1}^N\E\left[\mu_i(\Y(1, \Z_{-i}); d) - \bar{\mu}^1(d) \right]^2  - \frac{1}{N}\sum_{i=1}^N\E^2\left[ \mu_i(\Y(1, \Z_{-i}); d) - \bar{\mu}^1(d) \right] \\
& + \frac{1}{N}\sum_{i=1}^N\sum_{j\in \mathcal{B}(i)}\E\left[ \left(\mu_i(\Y(1, 1,\Z_{-(i,j)}); d) - \bar{\mu}^1(d) \right)\left(\mu_j(\Y(1, 1, \Z_{-(i,j)}); d) - \bar{\mu}^1(d) \right)\right] \\
& - \frac{1}{N}\sum_{i=1}^N\sum_{j\in \mathcal{B}(i)}\E\left[\mu_i(\Y(1, \Z_{-i}); d) - \bar{\mu}^1(d)\right] \E\left[ \mu_j(\Y(1, \Z_{-j}); d) - \bar{\mu}^1(d) \right]
\end{align*}
The last equality is due to the fact that
\begin{align*}
& \frac{1}{N}\sum_{i=1}^N\sum_{j\notin \mathcal{B}(i)}\E\left[ \left(\mu_i(\Y(1, 1,\Z_{-(i,j)}); d) - \bar{\mu}^1(d) \right)\left(\mu_j(\Y(1, 1, \Z_{-(i,j)}); d) - \bar{\mu}^1(d) \right)\right] \\
= & \frac{1}{N}\sum_{i=1}^N\sum_{j\notin \mathcal{B}(i)}\E\left[ \left(\mu_i(\Y(1, \Z_{-i}); d) - \bar{\mu}^1(d) \right)\left(\mu_j(\Y(1, \Z_{-j}); d) - \bar{\mu}^1(d) \right)\right] \\
= & \frac{1}{N}\sum_{i=1}^N\sum_{j\notin \mathcal{B}(i)}\E\left[ \mu_i(\Y(1, \Z_{-i}); d) - \bar{\mu}^1(d) \right]\E\left[\mu_j(\Y(1, \Z_{-j}); d) - \bar{\mu}^1(d) \right]
\end{align*}
%\begin{align*}
%& N\Var\left[\tilde{\mu}^1(d) - \bar{\mu}^1(d) \tilde{N}_1\right] \\
%= & \frac{1}{Np} \sum_{i=1}^N \E\left[\mu_i^2(\Y(1, \Z_{-i}); d) \right] - \frac{1}{N} \sum_{i=1}^N \E^2\left[\mu_i(\Y(1, \Z_{-i}); d) \right] \\
%& + \frac{1}{N} \sum_{i=1}^N \sum_{j\in \mathcal{B}(i)} \Cov\left[\mu_i(\Y(1,1, \Z_{-(i,j)}); d), \mu_j(\Y(1,1, \Z_{-(i,j)}); d)\right] \\
%& + \frac{1}{N} \sum_{i=1}^N \sum_{j\in \mathcal{B}(i)}\E\left[\mu_i(\Y(1,1, \Z_{-(i,j)}); d)\right] \E\left[\mu_j(\Y(1,1, \Z_{-(i,j)}); d)\right]  \\
%& - \frac{1}{N} \sum_{i=1}^N \sum_{j\in \mathcal{B}(i)}\E\left[\mu_i(\Y(1, \Z_{-i}); d) \right] \E\left[\mu_j(\Y(1, \Z_{-j}); d) \right] \\
%& - \frac{1-p}{N^2p} \left(\sum_{i=1}^N \E\left[\mu_i(\Y(1, \Z_{-i}); d) \right] \right)^2 \\
%& - \frac{2}{N^2} \sum_{i=1}^N \sum_{j\in \mathcal{B}(i)}\left( \E\left[\mu_i(\Y(1, 1, \Z_{-(i,j)}); d) \right] - \E\left[\mu_i(\Y(1, \Z_{-i}); d) \right] \right) \sum_{i=1}^N \E\left[\mu_i(\Y(1, \Z_{-i}); d) \right] \\
%= & \frac{1}{Np} \sum_{i=1}^N \E\left[\mu_i^2(\Y(1, \Z_{-i}); d) \right] - \frac{1}{N} \sum_{i=1}^N \E^2\left[\mu_i(\Y(1, \Z_{-i}); d) \right] \\
%& + \frac{1}{N} \sum_{i=1}^N \sum_{j\in \mathcal{B}(i)} \Cov\left[\mu_i(\Y(1,\Z_{-i}); d), \mu_j(\Y(1,\Z_{-j}); d)\right] \\
%& - \frac{1-p}{N^2p} \left(\sum_{i=1}^N \E\left[\mu_i(\Y(1, \Z_{-i}); d) \right] \right)^2 \\
%& - \frac{2}{N^2} \sum_{i=1}^N \sum_{j\in \mathcal{B}(i)}\left( \E\left[\mu_i(\Y(1, 1, \Z_{-(i,j)}); d) \right] - \E\left[\mu_i(\Y(1, \Z_{-i}); d) \right] \right) \sum_{i=1}^N \E\left[\mu_i(\Y(1, \Z_{-i}); d) \right] 
%\end{align*}
%\begin{align*}
%& N\E\left[\tilde{\mu}^1(d) - \bar{\mu}^1(d) \tilde{N}_1\right]^2 \\
%= & \frac{1}{Np^2}\E\left[\sum_{i=1}^N Z_i \mu_i(\Y(\Z); d) - \frac{N_1}{N} \sum_{i=1}^N \E\left[\mu_i(\Y(1, \Z_{-i}); d)\right]\right]^2 \\
%= & \frac{1}{Np^2}\sum_{i=1}^N\E\left[ Z_i \mu_i(\Y(\Z); d) - \frac{N_1}{N} \E\left[\mu_i(\Y(1, \Z_{-i}); d)\right]\right]^2 \\
%& + \frac{1}{Np^2}\sum_{i=1}^N\sum_{j \neq i}\E\left[Z_i Z_j  \mu_i(\Y(\Z); d) \mu_j(\Y(\Z); d) + \frac{N_1^2}{N^2} \E\left[\mu_i(\Y(1, \Z_{-i}); d)\right] \E\left[\mu_j(\Y(1, \Z_{-j}); d)\right]\right] \\
%& - \frac{2}{Np^2}\sum_{i=1}^N\sum_{j \neq i}\E\left[\frac{Z_i N_1}{N} \mu_i(\Y(\Z); d) \E\left[\mu_j(\Y(1, \Z_{-j}); d)\right]\right] \\
%= & \frac{1}{Np}\sum_{i=1}^N\E\left[ \mu_i^2(\Y(1, \Z_{-i}); d)\right] - \frac{2}{N^2}\sum_{i=1}^N \sum_{j \neq i} \E\left[ \mu_i(\Y(1,1, \Z_{-(i,j)}); d)\right] \E\left[ \mu_i(\Y(1, \Z_{-i}); d)\right]  \\
%& - \frac{1}{N^2p}\sum_{i=1}^N\E^2\left[ \mu_i(\Y(1, \Z_{-i}); d)\right] + \frac{N-1}{N^2}\sum_{i=1}^N \E^2\left[ \mu_i(\Y(1, \Z_{-i}); d)\right] \\
%& + \frac{1}{N}\sum_{i=1}^N\sum_{j \neq i}\E\left[ \mu_i(\Y(1,1,\Z_{-(i,j)}); d) \mu_j(\Y(1,1,\Z_{-(i,j)}); d) \right] \\
%& + \frac{(N-1)p-1}{N^2p}\sum_{i=1}^N\sum_{j \neq i}\E\left[ \mu_i(\Y(1,\Z_{-i}); d)\right] \E\left[\mu_j(\Y(1,\Z_{-j}); d) \right] \\
%& - \frac{2}{N^2}\sum_{i=1}^N\sum_{j \neq i}\sum_{k \neq i}\E\left[ \mu_i(\Y(1,1,\Z_{-(i,k)}); d)\right] \E\left[\mu_j(\Y(1,\Z_{-j}); d) \right] \\
%= & \frac{1}{Np}\sum_{i=1}^N\E\left[ \mu_i^2(\Y(1, \Z_{-i}); d)\right] - \frac{1}{N}\sum_{i=1}^N \E^2\left[ \mu_i(\Y(1, \Z_{-i}); d)\right]  \\
%& + \frac{1}{N}\sum_{i=1}^N\sum_{j \in \mathcal{B}(i)}\E\left[ \mu_i(\Y(1,1,\Z_{-(i,j)}); d) \mu_j(\Y(1,1,\Z_{-(i,j)}); d) \right] \\
%& + \frac{1}{N}\sum_{i=1}^N\sum_{j \notin \mathcal{B}(i)}\E\left[ \mu_i(\Y(1,\Z_{-i}); d) \mu_j(\Y(1,\Z_{-j}); d) \right] \\
%& + \frac{1}{N}\sum_{i=1}^N\sum_{j \neq i}\E\left[ \mu_i(\Y(1,\Z_{-i}); d)\right] \E\left[\mu_j(\Y(1,\Z_{-j}); d) \right] \\
%& - \frac{2}{N^2}\sum_{i=1}^N\sum_{j \neq i}\sum_{k \neq i}\E\left[ \mu_i(\Y(1,1,\Z_{-(i,k)}); d)\right] \E\left[\mu_j(\Y(1,\Z_{-j}); d) \right] \\
%\end{align*}


%\begin{align*}
%& N\Var\left[\tilde{\mu}^0(d) - \bar{\mu}^0(d) \tilde{N}_1\right] \\
%= & \frac{1}{N(1-p)} \sum_{i=1}^N \E\left[\mu_i^2(\Y(0, \Z_{-i}); d) \right] - \frac{1}{N} \sum_{i=1}^N \E^2\left[\mu_i(\Y(0, \Z_{-i}); d) \right] \\
%& + \frac{1}{N} \sum_{i=1}^N \sum_{j\in \mathcal{B}(i)} \Cov\left[\mu_i(\Y(0, \Z_{-i}); d), \mu_j(\Y(0, \Z_{-j}); d)\right] \\
%& - \frac{p}{N^2(1-p)} \left(\sum_{i=1}^N \E\left[\mu_i(\Y(0, \Z_{-i}); d) \right] \right)^2 \\
%& - \frac{2}{N^2} \sum_{i=1}^N \sum_{j\in \mathcal{B}(i)}\left( \E\left[\mu_i(\Y(0, 0, \Z_{-(i,j)}); d) \right] - \E\left[\mu_i(\Y(0, \Z_{-i}); d) \right] \right) \sum_{i=1}^N \E\left[\mu_i(\Y(0, \Z_{-i}); d) \right] 
%\end{align*}

Similarly,
\begin{align*}
& N\Var\left[\tilde{\mu}^0(d) - \bar{\mu}^0(d) \tilde{N}_1\right] \\
= & \frac{1}{N(1-p)}\sum_{i=1}^N\E\left[\mu_i(\Y(0, \Z_{-i}); d) - \bar{\mu}^0(d) \right]^2  - \frac{1}{N}\sum_{i=1}^N\E^2\left[ \mu_i(\Y(0, \Z_{-i}); d) - \bar{\mu}^0(d) \right] \\
& + \frac{1}{N}\sum_{i=1}^N\sum_{j\in \mathcal{B}(i)}\E\left[ \left(\mu_i(\Y(0, 0,\Z_{-(i,j)}); d) - \bar{\mu}^0(d) \right)\left(\mu_j(\Y(0, 0, \Z_{-(i,j)}); d) - \bar{\mu}^0(d) \right)\right] \\
& - \frac{1}{N}\sum_{i=1}^N\sum_{j\in \mathcal{B}(i)}\E\left[\mu_i(\Y(0, \Z_{-i}); d) - \bar{\mu}^0(d) \right] \E\left[ \mu_j(\Y(0, \Z_{-j}); d) - \bar{\mu}^0(d) \right]
\end{align*}
and 
\begin{align*}
& N\Cov\left[\left(\tilde{\mu}^1(d) - \bar{\mu}^1(d) \tilde{N}_1\right) ,\left(\tilde{\mu}^0(d) - \bar{\mu}^0(d) \tilde{N}_0\right)\right] \\
= & \frac{1}{Np(1-p)}\Cov\left[\sum_{i=1}^N Z_i\left(\mu_i(\Y(\Z); d) - \bar{\mu}^1(d) \right), \sum_{j=1}^N (1-Z_j)\left(\mu_j(\Y(\Z); d) - \bar{\mu}^0(d) \right)\right]  \\
= & \frac{1}{Np(1-p)}\sum_{i=1}^N \sum_{j=1}^N \E\left[Z_i (1-Z_j) \left(\mu_i(\Y(\Z); d) - \bar{\mu}^1(d) \right)\left(\mu_j(\Y(\Z); d) - \bar{\mu}^0(d) \right)\right]  \\
& - \frac{1}{Np(1-p)}\sum_{i=1}^N \sum_{j=1}^N\E\left[Z_i\left(\mu_i(\Y(\Z); d) - \bar{\mu}^1(d) \right)\right] \E\left[(1-Z_j)\left(\mu_j(\Y(\Z); d) - \bar{\mu}^0(d) \right)\right]  \\
= & \frac{1}{N}\sum_{i=1}^N \sum_{j\neq i} \E\left[ \left(\mu_i(\Y(1,0,\Z_{-(i,j)}); d) - \bar{\mu}^1(d) \right)\left(\mu_j(\Y(1,0,\Z_{-(i,j)}); d) - \bar{\mu}^0(d) \right)\right]  \\
& - \frac{1}{N}\sum_{i=1}^N \sum_{j=1}^N\E\left[\mu_i(\Y(1,\Z_{-i}); d) - \bar{\mu}^1(d)\right] \E\left[\mu_j(\Y(0,\Z_{-j}); d) - \bar{\mu}^0(d) \right]  \\
= & \frac{1}{N}\sum_{i=1}^N \sum_{j\in \mathcal{B}(i)} \E\left[ \left(\mu_i(\Y(1,0,\Z_{-(i,j)}); d) - \bar{\mu}^1(d) \right)\left(\mu_j(\Y(1,0,\Z_{-(i,j)}); d) - \bar{\mu}^0(d) \right)\right]  \\
& - \frac{1}{N}\sum_{i=1}^N \sum_{j\in \mathcal{B}(i)}\E\left[\mu_i(\Y(1,\Z_{-i}); d) - \bar{\mu}^1(d) \right] \E\left[\mu_j(\Y(0,\Z_{-j}); d) - \bar{\mu}^0(d)\right] \\
& - \frac{1}{N}\sum_{i=1}^N \E\left[\mu_i(\Y(1,\Z_{-i}); d) - \bar{\mu}^1(d) \right] \E\left[\mu_i(\Y(0,\Z_{-i}); d) - \bar{\mu}^0(d) \right].
\end{align*}
%Notice that for any $a, b \in \{0, 1\}$, we have
%\begin{align*}
%& \frac{1}{N}\sum_{i=1}^N \sum_{j\in \mathcal{B}(i)}\E\left[\mu_i(\Y(a,\Z_{-i}); d) - \bar{\mu}^a(d) \right] \E\left[\mu_j(\Y(b,\Z_{-j}); d) - \bar{\mu}^b(d)\right] \\
%= & 
%\end{align*}
%\begin{align*}
%& N\Cov\left[\left(\tilde{\mu}^1(d) - \bar{\mu}^1(d) \tilde{N}_1\right) ,\left(\tilde{\mu}^0(d) - \bar{\mu}^0(d) \tilde{N}_0\right)\right] \\
%= & N\Cov\left[\tilde{\mu}^1(d), \tilde{\mu}^0(d) \right] - N\Cov\left[\tilde{\mu}^1(d), \tilde{N}_0 \right]\bar{\mu}^0(d) \\
%& - N\Cov\left[\tilde{\mu}^0(d), \tilde{N}_1\right]\bar{\mu}^1(d) + N\Cov\left[ \tilde{N}_1, \tilde{N}_0\right]\bar{\mu}^1(d) \bar{\mu}^0(d) \\
%= & \frac{1}{N} \sum_{i=1}^N \sum_{j \in \mathcal{B}(i)} \Cov\left[\mu_i(\Y(1, \Z_{-i}); d) \mu_j(\Y(0, \Z_{-j}); d)\right] - \frac{1}{N}\sum_{i=1}^N  \E\left[\mu_i(\Y(1,\Z_{-i}); d) \right] \E\left[\mu_i(\Y(0,\Z_{-i}); d) \right] \\
%& + \frac{1}{N^2} \sum_{i=1}^N \E\left[\mu_i(\Y(1,\Z_{-i}); d) \right]  \sum_{i=1}^N\E\left[\mu_i(\Y(0,\Z_{-i}); d) \right] \\ 
%& - \frac{1}{N^2} \sum_{i=1}^N \sum_{j\in \mathcal{B}(i)}\left( \E\left[\mu_i(\Y(1, 0, \Z_{-(i,j)}); d) \right] - \E\left[\mu_i(\Y(1, \Z_{-i}); d) \right] \right) \sum_{i=1}^N \E\left[\mu_i(\Y(0, \Z_{-i}); d) \right] \\
%& - \frac{1}{N^2} \sum_{i=1}^N \sum_{j\in \mathcal{B}(i)}\left( \E\left[\mu_i(\Y(0, 1, \Z_{-(i,j)}); d) \right] - \E\left[\mu_i(\Y(0, \Z_{-i}); d) \right] \right) \sum_{i=1}^N \E\left[\mu_i(\Y(1, \Z_{-i}); d) \right] 
%\end{align*}

To summarize,
\begin{align*}
& N \Var \left[\hat{\tau}_{HA}(d)\right] \\
= & \frac{1}{Np}\sum_{i=1}^N\E\left[\mu_i(\Y(1, \Z_{-i}); d) - \bar{\mu}^1(d) \right]^2 + \frac{1}{N(1-p)}\sum_{i=1}^N\E\left[\mu_i(\Y(0, \Z_{-i}); d) - \bar{\mu}^0(d) \right]^2 \\
& - \frac{1}{N}\sum_{i=1}^N\left(\E\left[ \mu_i(\Y(1, \Z_{-i}); d) - \bar{\mu}^1(d) \right] - \E\left[ \mu_i(\Y(0, \Z_{-i}); d) - \bar{\mu}^0(d) \right]\right)^2 \\
& + \frac{1}{N}\sum_{i=1}^N\sum_{j\in \mathcal{B}(i)}\E\left[ \left(\mu_i(\Y(1, 1,\Z_{-(i,j)}); d) - \bar{\mu}^1(d) \right)\left(\mu_j(\Y(1, 1, \Z_{-(i,j)}); d) - \bar{\mu}^1(d) \right)\right] \\
& - \frac{1}{N}\sum_{i=1}^N\sum_{j\in \mathcal{B}(i)}\E\left[\mu_i(\Y(1, \Z_{-i}); d) - \bar{\mu}^1(d) \right] \E\left[ \mu_j(\Y(1, \Z_{-j}); d) - \bar{\mu}^1(d) \right] \\
& + \frac{1}{N}\sum_{i=1}^N\sum_{j\in \mathcal{B}(i)}\E\left[ \left(\mu_i(\Y(0, 0,\Z_{-(i,j)}); d) - \bar{\mu}^0(d) \right)\left(\mu_j(\Y(0, 0, \Z_{-(i,j)}); d) - \bar{\mu}^0(d) \right)\right] \\
& - \frac{1}{N}\sum_{i=1}^N\sum_{j\in \mathcal{B}(i)}\E\left[\mu_i(\Y(0, \Z_{-i}); d) - \bar{\mu}^0(d) \right] \E\left[ \mu_j(\Y(0, \Z_{-j}); d) - \bar{\mu}^0(d) \right] \\
& - \frac{2}{N}\sum_{i=1}^N \sum_{j\in \mathcal{B}(i)} \E\left[ \left(\mu_i(\Y(1,0,\Z_{-(i,j)}); d) - \bar{\mu}^1(d) \right)\left(\mu_j(\Y(1,0,\Z_{-(i,j)}); d) - \bar{\mu}^0(d) \right)\right]  \\
& + \frac{2}{N}\sum_{i=1}^N \sum_{j\in \mathcal{B}(i)}\E\left[\mu_i(\Y(1,\Z_{-i}); d) - \bar{\mu}^1(d)\right] \E\left[\mu_j(\Y(0,\Z_{-j}); d) - \bar{\mu}^0(d) \right] 
\end{align*}
Under the assumption on homogeneous interference, for any $a, b \in \{0, 1\}$, we have
\begin{align*}
& \frac{1}{N}\sum_{i=1}^N \sum_{j\in \mathcal{B}(i)}\E\left[\mu_i(\Y(a,\Z_{-i}); d) - \bar{\mu}^a(d)\right] \E\left[\mu_j(\Y(b,\Z_{-j}); d) - \bar{\mu}^b(d) \right]  \\
= & \frac{1}{N}\sum_{i=1}^N \sum_{j\in \mathcal{B}(i)}\E\left[\mu_i(\Y(a,\Z_{-i}); d)\right] \E\left[\mu_j(\Y(b,\Z_{-j}); d) \right] \\
& - \frac{1}{N^2} \left(\sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)} \E \left[\mu_i (\Y(a, \mathbf{Z}_{-i});d)\right]\right)\sum_{k=1}^N \E \left[\mu_k (\Y(b, \mathbf{Z}_{-k});d)\right] \\
& - \frac{1}{N^2} \left(\sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)} \E \left[\mu_j (\Y(b, \mathbf{Z}_{-j});d)\right]\right)\sum_{k=1}^N \E \left[\mu_k (\Y(a, \mathbf{Z}_{-k});d)\right] \\
& + \frac{1}{N}\sum_{i=1}^N \sum_{j\in \mathcal{B}(i)}\frac{1}{N^2} \left(\sum_{k=1}^N \E \left[\mu_k (\Y(a, \mathbf{Z}_{-k});d)\right]\right) \left(\sum_{l=1}^N \E \left[\mu_l (\Y(b, \mathbf{Z}_{-k});d)\right]\right)  + o_P(1) \\
= & \frac{1}{N^2} \left(\sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)} \E \left[\mu_i (\Y(b, \mathbf{Z}_{-i});d)\right]\right)\sum_{k=1}^N \E \left[\mu_k (\Y(a, \mathbf{Z}_{-k});d)\right] \\
& - \frac{1}{N^2} \left(\sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)} \E \left[\mu_i (\Y(a, \mathbf{Z}_{-i});d)\right]\right)\sum_{k=1}^N \E \left[\mu_k (\Y(b, \mathbf{Z}_{-k});d)\right] \\
& - \frac{1}{N^2} \left(\sum_{i=1}^{N} \sum_{i \in \mathcal{B}(i)} \E \left[\mu_i (\Y(b, \mathbf{Z}_{-i});d)\right]\right)\sum_{k=1}^N \E \left[\mu_k (\Y(a, \mathbf{Z}_{-k});d)\right] \\
& + \bar{c}\frac{1}{N^2} \left(\sum_{k=1}^N \E \left[\mu_k (\Y(a, \mathbf{Z}_{-k});d)\right]\right) \left(\sum_{l=1}^N \E \left[\mu_l (\Y(b, \mathbf{Z}_{-k});d)\right]\right)  + o_P(1) \\
= & \frac{1}{N^2} \sum_{i=1}^{N}\sum_{k=1}^N (c_i - \bar{c}) \E \left[\mu_i (\Y(a, \mathbf{Z}_{-i});d)\right] \E \left[\mu_k (\Y(b, \mathbf{Z}_{-k});d)\right] + o_P(1) \\
= & o_P(1).
\end{align*}
Hence,
\begin{align*}
& N \Var \left[\hat{\tau}_{HA}(d)\right] \\
\leq & \frac{1}{Np}\sum_{i=1}^N\E\left[\mu_i(\Y(1, \Z_{-i}); d) - \bar{\mu}^1(d) \right]^2 + \frac{1}{N(1-p)}\sum_{i=1}^N\E\left[\mu_i(\Y(0, \Z_{-i}); d) - \bar{\mu}^0(d) \right]^2 \\
& + \frac{1}{N}\sum_{i=1}^N\sum_{j\in \mathcal{B}(i)}\E\left[ \left(\mu_i(\Y(1, 1,\Z_{-(i,j)}); d) - \bar{\mu}^1(d) \right)\left(\mu_j(\Y(1, 1, \Z_{-(i,j)}); d) - \bar{\mu}^1(d) \right)\right] \\
& + \frac{1}{N}\sum_{i=1}^N\sum_{j\in \mathcal{B}(i)}\E\left[ \left(\mu_i(\Y(0, 0,\Z_{-(i,j)}); d) - \bar{\mu}^0(d) \right)\left(\mu_j(\Y(0, 0, \Z_{-(i,j)}); d) - \bar{\mu}^0(d) \right)\right] \\
& - \frac{2}{N}\sum_{i=1}^N \sum_{j\in \mathcal{B}(i)} \E\left[ \left(\mu_i(\Y(1,0,\Z_{-(i,j)}); d) - \bar{\mu}^1(d) \right)\left(\mu_j(\Y(1,0,\Z_{-(i,j)}); d) - \bar{\mu}^0(d) \right)\right] + o_P(1).
\end{align*}
%\begin{align*}
%& N \Var \left[\hat{\tau}_{HA}(d)\right] \\
%= & \frac{1}{Np} \sum_{i=1}^N \E\left[\mu_i^2(\Y(1, \Z_{-i}); d) \right] + \frac{1}{N(1-p)} \sum_{i=1}^N \E\left[\mu_i^2(\Y(0, \Z_{-i}); d) \right] \\
%& - \frac{1}{N} \sum_{i=1}^N \E^2\left[\mu_i(\Y(1, \Z_{-i}); d) - \mu_i(\Y(0, \Z_{-i}); d)\right] \\
%& - \frac{1}{N^2p(1-p)}\left((1-p)\sum_{i=1}^N \E\left[\mu_i(\Y(1, \Z_{-i}); d) \right] + p\sum_{i=1}^N \E\left[\mu_i(\Y(0, \Z_{-i}); d) \right] \right)^2 \\
%& + \frac{1}{N} \sum_{i=1}^N \sum_{j\in \mathcal{B}(i)} \{\Cov\left[\mu_i(\Y(1,\Z_{-i}); d), \mu_j(\Y(1,\Z_{-j}); d)\right] + \Cov\left[\mu_i(\Y(0,\Z_{-i}); d), \mu_j(\Y(0,\Z_{-j}); d)\right]\} \\
%& - \frac{2}{N} \sum_{i=1}^N \sum_{j\in \mathcal{B}(i)} \{\Cov\left[\mu_i(\Y(1,\Z_{-i}); d), \mu_j(\Y(0,\Z_{-j}); d)\right]\} \\
%& + \frac{2}{N^2} \sum_{i=1}^N \sum_{j\in \mathcal{B}(i)} (\E\left[\mu_i(\Y(1, 0, \Z_{-(i,j)}); d) \right] + \E\left[\mu_i(\Y(0, 1, \Z_{-(i,j)}); d) \right] \\
%& - \E\left[\mu_i(\Y(1, 1, \Z_{-(i,j)}); d) \right] - \E\left[\mu_i(\Y(0, 0, \Z_{-(i,j)}); d) \right] ) ) \\
%& * \left((1-p)\sum_{i=1}^N  \E\left[\mu_i(\Y(1, \Z_{-i}); d) \right] + p\sum_{i=1}^N  \E\left[\mu_i(\Y(0, \Z_{-i}); d) \right]\right) \\
%= & \frac{1}{Np} \sum_{i=1}^N \E\left[\mu_i(\Y(1, \Z_{-i}); d) - \frac{1}{N}\sum_{k=1}^N \mu_k(\Y(1, \Z_{-k}); d)\right]^2 \\
%& + \frac{1}{N(1-p)} \sum_{i=1}^N \E\left[\mu_i(\Y(0, \Z_{-i}); d)  - \frac{1}{N}\sum_{k=1}^N \mu_k(\Y(0, \Z_{-k}); d)\right]^2 \\
%& - \frac{1}{N} \sum_{i=1}^N \E^2\left[\mu_i(\Y(1, \Z_{-i}); d) - \mu_i(\Y(0, \Z_{-i}); d) - \frac{1}{N}\sum_{k=1}^N \mu_k(\Y(0, \Z_{-k}); d) + \frac{1}{N}\sum_{k=1}^N \mu_k(\Y(0, \Z_{-k}); d) \right] \\
%& + \frac{1}{N} \sum_{i=1}^N \sum_{j\in \mathcal{B}(i)}\sum_{a,b=0}^1 (-1)^{a+b} \Cov\left[\mu_i(\Y(a,\Z_{-i}); d), \mu_j(\Y(b,\Z_{-j}); d)\right] \\
%& + \frac{2}{N^2} \sum_{i=1}^N \sum_{j\in \mathcal{B}(i)} (\E\left[\mu_i(\Y(1, 0, \Z_{-(i,j)}); d) \right] + \E\left[\mu_i(\Y(0, 1, \Z_{-(i,j)}); d) \right] \\
%& - \E\left[\mu_i(\Y(1, 1, \Z_{-(i,j)}); d) \right] - \E\left[\mu_i(\Y(0, 0, \Z_{-(i,j)}); d) \right] ) ) \\
%& * \left((1-p)\sum_{i=1}^N  \E\left[\mu_i(\Y(1, \Z_{-i}); d) \right] + p\sum_{i=1}^N \E\left[\mu_i(\Y(0, \Z_{-i}); d) \right]\right) \\
%\end{align*}
\newpage
\section{Consistenty of the spatial HAC variance estimator}
Our estimation of $\tau_d$ could be seen as a two-step process. In the first step, we construct the circle mean for each intervention node: $\mu_i(d) = \mu_i(\Y(\Z); d) = \frac{\sum_x \mathbf{1}\{d_{ix} = d\}Y_x}{\sum_x \mathbf{1}\{d_{ix} = d\}}$. In the second step, we apply the Horvitz-Thompson estimator or the Hajek estimator to all the $(Z_i, \mu_i(d))$.

It is well-known that regression could be used to generate unbiased estimate of the average treatment effect in experiments. Treating $\mu_i(d)$ as nuisance parameters, we can estimate the following regression equation:

\begin{align*}
\mu_i(d) = \alpha + \tau_d Z_i + \varepsilon_i(d).
\end{align*}

It is easy to show that under OLS, $\hat{\alpha} = \frac{1}{N_0}\sum_{i=1}^{N} (1-Z_i) \mu_i(d) = \bar{\mu}_0(d)$ and $\hat{\tau}_{d, OLS} = \frac{1}{N_1}\sum_{i=1}^{N} Z_i \mu_i(d) - \frac{1}{N_0}\sum_{i=1}^{N} (1-Z_i) \mu_i(d) = \bar{\mu}_1(d) - \bar{\mu}_0(d)$, where $N_0 = \sum_{i=1}^{N} (1-Z_i)$ and $N_1 = \sum_{i=1}^{N}Z_i$. Clearly, $\hat{\tau}_{d, OLS} = \hat{\tau}_{d, HA}$. Then the residual for each observation $\hat{e}_i = \mu_i - \hat{\alpha} - \hat{\tau}_{d, OLS} Z_i = \mu_i - \bar{\mu}_0(d) - [\bar{\mu}_1(d) - \bar{\mu}_0(d)] Z_i $. 
%The strong law of large numbers renders that as $N \rightarrow \infty$, $\bar{\mu}_1(d) \overset{a.s.}{\rightarrow} \frac{\sum_{i=1}^N \E\left[\mu_i (1,\mathbf{Z}_{-i};d) \right]}{N}$ and $\bar{\mu}_0(d) \overset{a.s.}{\rightarrow} \frac{\sum_{i=1}^N \E\left[\mu_i (0,\mathbf{Z}_{-i};d) \right]}{N}$.

Denote $\begin{pmatrix}
1, Z_1 \\
1, Z_2 \\
\dots \\
1, Z_N
\end{pmatrix}$ as $\mathbf{X}$, the spatial HAC standard errors of $(\hat{\alpha}, \hat{\tau}_{d, OLS})$ can be expressed as:

\begin{align*}
\sigma \begin{pmatrix}
\hat{\alpha} \\
\hat{\tau}_{d, OLS}
\end{pmatrix} = & \sqrt{\Var \begin{pmatrix}
\hat{\alpha} \\
\hat{\tau}_{d, OLS}
\end{pmatrix}} \\
 \widehat{\Var} \begin{pmatrix}
\hat{\alpha} \\
\hat{\tau}_{d, OLS}
\end{pmatrix} = & (\mathbf{X}' \mathbf{X})^{-1}(\mathbf{X}' \Sigma \mathbf{X})(\mathbf{X}' \mathbf{X})^{-1} \\
= & \begin{pmatrix}
N, N_1 \\
N_1, N_1
\end{pmatrix}^{-1}\left(\sum_{i=1}^N \sum_{j=1}^N \mathbf{X}_{i} \mathbf{X}_{j}^{'}\hat{e}_i \hat{e}_j \mathbf{1}\{j \in \mathcal{B}(i) \}\right)\begin{pmatrix}
N, N_1 \\
N_1, N_1
\end{pmatrix}^{-1} \\
= & \frac{1}{N_1^2 N_0^2}\begin{pmatrix}
N_1, -N_1 \\
-N_1, N
\end{pmatrix}\left(\sum_{i=1}^N \sum_{j=1}^N \begin{pmatrix}
1, Z_j \\
Z_i, Z_i Z_j
\end{pmatrix}\hat{e}_i \hat{e}_j \mathbf{1}\{j \in \mathcal{B}(i) \}\right)\begin{pmatrix}
N_1, -N_1 \\
-N_1, N
\end{pmatrix}
\end{align*}
Note that the $(2,2)$ entry of $\begin{pmatrix}
N_1, -N_1 \\
-N_1, N
\end{pmatrix} \begin{pmatrix}
1, Z_j \\
Z_i, Z_i Z_j
\end{pmatrix} \begin{pmatrix}
N_1, -N_1 \\
-N_1, N
\end{pmatrix}$ equals to $N_1^2 - N_1 N Z_i - - N_1 N Z_j + N^2 Z_i Z_j$. Rearrange the sample such that treated observations lie before observations under control and plug in the expression of $\hat{e}_i$ , we can see that:
\begin{align*}
\widehat{\Var}(\hat{\tau}_{d, OLS}) = & \frac{1}{N_1^2} \sum_{i=1}^{N_1} \hat{e}_i^2 + \frac{1}{N_0^2} \sum_{i=N_1+1}^{N} \hat{e}_i^2 + \frac{1}{N_1^2} \sum_{i=1}^{N_1} \sum_{j \neq i, Z_j = 1}\hat{e}_i\hat{e}_j \\
- & \frac{1}{N_1 N_0} \sum_{i=1}^{N_1} \sum_{j \neq i, Z_j = 0}\hat{e}_i\hat{e}_j - \frac{1}{N_1 N_0} \sum_{i=N_1+1}^{N} \sum_{j \neq i, Z_j = 1}\hat{e}_i\hat{e}_j  + \frac{1}{N_0^2} \sum_{i=N_1+1}^{N} \sum_{j \neq i, Z_j = 0}\hat{e}_i\hat{e}_j \\
= & \frac{1}{N_1^2} \sum_{i=1}^{N_1} \left(\mu_i (d) - \bar{\mu}_1 (d)\right)^2 + \frac{1}{N_0^2} \sum_{i=N_1+1}^{N} \left(\mu_i (d) - \bar{\mu}_0 (d)\right)^2  \\
+ & \frac{1}{N_1^2} \sum_{i=1}^{N_1} \sum_{j \in \mathcal{B}(i), Z_j = 1} \left(\mu_i (d) - \bar{\mu}_1 (d)\right) \left(\mu_j (d) - \bar{\mu}_1 (d)\right) \\
- & \frac{1}{N_1 N_0} \sum_{i=1}^{N_1} \sum_{j \in \mathcal{B}(i), Z_j = 0} \left(\mu_i (d) - \bar{\mu}_1 (d)\right) \left(\mu_j (d) - \bar{\mu}_0 (d)\right) \\
- & \frac{1}{N_1 N_0} \sum_{i=N_1+1}^{N} \sum_{j \in \mathcal{B}(i), Z_j = 1} \left(\mu_i (d) - \bar{\mu}_0 (d)\right) \left(\mu_j (d) - \bar{\mu}_1 (d)\right) \\
+ & \frac{1}{N_0^2} \sum_{i=N_1+1}^{N} \sum_{j \in \mathcal{B}(i), Z_j = 0} \left(\mu_i (d) - \bar{\mu}_0 (d)\right) \left(\mu_j (d) - \bar{\mu}_0 (d)\right)
\end{align*}

Finally, we show that the variance estimate $N\widehat{\Var}(\hat{\tau}_{d, OLS})$ is asymptotically unbiased for the rescaled variance of the Hajek estimator: $N\Var(\hat{\tau}_{d, HA})$. 

%Note that the first part in the true variance for the Hajek estimator can be written as:
%\begin{align*}
%& \frac{1}{Np}\sum_{i=1}^N \E\left[\left(\mu_i(\Y(1, \Z_{-i}); d)-  \frac{1}{N}\sum_{k=1}^N \mu_k(\Y(1, \Z_{-k}); d)\right)^2\right] \\
%= & \frac{1}{Np}\sum_{i=1}^N \E\left[\mu_i^2(\Y(1, \Z_{-i}); d)\right]  - \frac{1}{N^2p} \E\left[\left(\sum_{i=1}^N \mu_i(\Y(1, \Z_{-i}); d)\right)^2\right] \\
%= & \frac{1}{Np}(1-\frac{1}{N})\sum_{i=1}^N \E\left[\mu_i^2(\Y(1, \Z_{-i}); d)\right] - \frac{1}{N^2p}\sum_{i=1}^N \sum_{j\neq i}^N \E\left[\mu_i(\Y(1, \Z_{-i}); d)\mu_j(\Y(1, \Z_{-j}); d)\right]
%\end{align*}

Taking expectation on the first term of the variance estimate, we have:
\begin{align*}
& N\E\left[\frac{1}{N_1^2} \sum_{i=1}^{N_1} \left(\mu_i(\Y(\Z); d) - \bar{\mu}_1 (d)\right)^2\right] \\
= & N\E\left[\frac{1}{N_1^2} \left(\sum_{i=1}^{N_1} \mu_i^2(\Y(\Z); d) - 2\bar{\mu}_1 (d)\sum_{i=1}^{N_1}\mu_i(\Y(\Z); d) + \sum_{i=1}^{N_1}(\bar{\mu}_1 (d))^2 \right)\right] \\
= & N\E\left[\frac{1}{N_1^2} \left(\sum_{i=1}^{N_1} \mu_i^2(\Y(\Z); d) - N_1\bar{\mu}_1^2 (d)\right)\right] \\
= & N\E\left[\frac{1}{N_1^2} \sum_{i=1}^{N_1} \mu_i^2(\Y(\Z); d) \right] - N\E\left[\frac{1}{N_1}\bar{\mu}_1^2 (d)\right] \\
= & \frac{1}{Np^2} \sum_{i=1}^{N} \E\left[  Z_i\mu_i^2(\Y(\Z); d)\right] - \frac{1}{N^2p^3}\sum_{i=1}^{N}\sum_{j = 1}^{N} \E\left[  Z_iZ_j\mu_i(\Y(\Z); d) \mu_j(\Y(\Z); d)\right] + o_P(1) \\
= & \frac{1}{Np} \sum_{i=1}^{N} \E\left[ \mu_i^2(\Y(1, \Z_{-i}); d)\right] - \frac{1}{N^2p}\sum_{i=1}^{N}\sum_{j = 1}^{N} \E\left[ \mu_i(\Y(1, 1, \Z_{-(i, j)}); d) \mu_j(\Y(1, 1, \Z_{-(i, j)}); d)\right] + o_P(1) \\
= & \frac{1}{Np} \sum_{i=1}^{N} \E\left[ \mu_i^2(\Y(1, \Z_{-i}); d)\right] - \frac{1}{N^2p}\sum_{i=1}^{N}\sum_{j = 1}^{N} \E\left[ \mu_i(\Y(1, \Z_{-i}); d)\right] \E\left[\mu_j(\Y(1, \Z_{-j}); d)\right] + o_P(1) \\
= & \frac{1}{Np}\sum_{i=1}^N\E\left[\mu_i(\Y(1, \Z_{-i}); d) - \bar{\mu}^1(d) \right]^2  + o_P(1).
\end{align*}
The second to the last equality holds as
\begin{align*}
& \frac{1}{N^2p}\sum_{i=1}^{N}\sum_{j = 1}^{N} \E\left[ \mu_i(\Y(1, 1, \Z_{-(i, j)}); d) \mu_j(\Y(1, 1, \Z_{-(i, j)}); d)\right] \\
= & \frac{1}{N^2p}\sum_{i=1}^N\sum_{j\notin \mathcal{B}(i)}\E\left[ \mu_i(\Y(1, 1, \Z_{-(i, j)}); d) \mu_j(\Y(1, 1, \Z_{-(i, j)}); d)\right] \\
& + \frac{1}{N^2p}\sum_{i=1}^N\sum_{j\in \mathcal{B}(i)}\E\left[ \mu_i(\Y(1, 1, \Z_{-(i, j)}); d) \mu_j(\Y(1, 1, \Z_{-(i, j)}); d)\right] \\
= & \frac{1}{N^2p}\sum_{i=1}^N\sum_{j\notin \mathcal{B}(i)}\E\left[ \mu_i(\Y(1, \Z_{-i}); d)\right] \E\left[\mu_j(\Y(1, \Z_{-j}); d)\right]  + o_P(1) \\
= & \frac{1}{N^2p}\sum_{i=1}^N\sum_{j\notin \mathcal{B}(i)}\E\left[ \mu_i(\Y(1, \Z_{-i}); d)\right] \E\left[\mu_j(\Y(1, \Z_{-j}); d)\right] \\
& + \frac{1}{N^2p}\sum_{i=1}^N\sum_{j\in \mathcal{B}(i)}\E\left[ \mu_i(\Y(1, \Z_{-i}); d)\right] \E\left[\mu_j(\Y(1, \Z_{-j}); d)\right]  + o_P(1) \\
= & \frac{1}{N^2p}\sum_{i=1}^{N}\sum_{j = 1}^{N} \E\left[ \mu_i(\Y(1, \Z_{-i}); d)\right] \E\left[\mu_j(\Y(1, \Z_{-j}); d)\right] + o_P(1). 
\end{align*}
% Note that $\E\left[\frac{N_1^2}{N^2} \right] = p$, 
%\begin{align*}
%& \E\left[ \sum_{i=1}^{N_1} \left(\mu_i (d) - \bar{\mu}_1 (d)\right)^2\right] \\
%= & \E\left[ \sum_{i=1}^{N} Z_i\left(\mu_i (1, \mathbf{Z}_{-i};d) - \bar{\mu}_1 (d)\right)^2\right] \\
%= & \sum_{i=1}^{N}\E\left[Z_i \left(\mu_i (1, \mathbf{Z}_{-i};d) - \bar{\mu}_1 (d)\right)^2\right] \\
%= & p\sum_{i=1}^{N}\E\left[\left(\mu_i (1, \mathbf{Z}_{-i};d) - \bar{\mu}_1 (d)\right)^2\right]
%\end{align*}
%and $\E\left[ N_1^2\right] = N^2 p^2$. Therefore,
%\begin{align*}
%& \E\left[\frac{1}{N_1^2} \sum_{i=1}^{N_1} \left(\mu_i (d) - \bar{\mu}_1 (d)\right)^2\right] \\
%\rightarrow & \frac{p\sum_{i=1}^{N}\E\left[\left(\mu_i (1, \mathbf{Z}_{-i};d) - \bar{\mu}_1 (d)\right)^2\right]}{N^2 p^2}  \\
%= & \frac{1}{N^2 p}\sum_{i=1}^{N}\E\left[\left(\mu_i (1, \mathbf{Z}_{-i};d) - \bar{\mu}_1 (d)\right)^2 \right]
%\end{align*}
%Similarly,
%\begin{align*}
%& \E\left[\frac{1}{N_0^2} \sum_{i=N_1+1}^{N} \left(\mu_i (d) - \bar{\mu}_1 (d)\right)^2\right] \\
%\rightarrow & \frac{(1-p)\sum_{i=1}^{N}\E\left[\left(\mu_i (0, \mathbf{Z}_{-i};d) - \bar{\mu}_0 (d)\right)^2\right]}{N^2 (1-p)^2}  \\
%= & \frac{1}{N^2 (1-p)}\sum_{i=1}^{N}\E\left[\left(\mu_i (0, \mathbf{Z}_{-i};d) - \bar{\mu}_0 (d)\right)^2 \right]
%\end{align*}
%and
%\begin{align*}
%& \E\left[\frac{1}{N_1^2} \sum_{i=1}^{N_1} \sum_{j \in \mathcal{B}(i), Z_j = 1} \left(\mu_i (d) - \bar{\mu}_1 (d)\right) \left(\mu_j (d) - \bar{\mu}_1 (d)\right)\right] \\
%\rightarrow & \frac{p^2 \sum_{i=1}^{N}\E\left[\left(\mu_i (d) - \bar{\mu}_1 (d)\right) \left(\mu_j (d) - \bar{\mu}_1 (d)\right)\right]}{N^2 p^2}  \\
%= & \frac{1}{N^2}\sum_{i=1}^{N}\E\left[\left(\mu_i (d) - \bar{\mu}_1 (d)\right) \left(\mu_j (d) - \bar{\mu}_1 (d)\right)\right]
%\end{align*}
%\begin{align*}
%& N\E\left[\frac{1}{N_1^2} \sum_{i=1}^{N_1} \left(\mu_i(\Y(\Z); d) - \bar{\mu}_1 (d)\right)^2\right] \\
%= & N\E\left[\frac{1}{N_1^2} \left(\sum_{i=1}^{N_1} \mu_i^2(\Y(\Z); d) - 2\bar{\mu}_1 (d)\sum_{i=1}^{N_1}\mu_i(\Y(\Z); d) + \sum_{i=1}^{N_1}(\bar{\mu}_1 (d))^2 \right)\right] \\
%= & N\E\left[\frac{1}{N_1^2} \left(\sum_{i=1}^{N_1} \mu_i^2 (1, \mathbf{Z}_{-i};d) - N_1\bar{\mu}_1^2 (d)\right)\right] \\
%= & N\E\left[\frac{1}{N_1^2} \sum_{i=1}^{N_1} \mu_i^2 (1, \mathbf{Z}_{-i};d) \right] - N\E\left[\frac{1}{N_1}\bar{\mu}_1^2 (d)\right] \\
%= & N\E\left[\frac{1}{N_1^2}(1-\frac{1}{N_1}) \sum_{i=1}^{N_1} \mu_i^2 (1, \mathbf{Z}_{-i};d) \right] - N\E\left[\frac{1}{N_1^3}\sum_{i=1}^{N_1}\sum_{j\neq i}^{N_1} \mu_i (1, \mathbf{Z}_{-i};d) \mu_j (1, \mathbf{Z}_{-j};d)\right] \\
%= & \frac{1}{Np^2}(1-\frac{1}{N}) \sum_{i=1}^{N} \E\left[  Z_i\mu_i^2 (1, \mathbf{Z}_{-i};d)\right] - \frac{1}{N^2p^3}\sum_{i=1}^{N}\sum_{j\neq i}^{N} \E\left[  Z_iZ_j\mu_i (Z_i, \mathbf{Z}_{-i};d) \mu_j (Z_j, \mathbf{Z}_{-j};d)\right] + o_P(1) \\
%= & \frac{1}{Np}(1-\frac{1}{N}) \sum_{i=1}^{N} \E\left[ \mu_i^2 (1, \mathbf{Z}_{-i};d)\right] - \frac{1}{N^2p}\sum_{i=1}^{N}\sum_{j\neq i}^{N} \E\left[  \mu_i (1,1, \mathbf{Z}_{-(i,j)};d) \mu_j (1, 1,\mathbf{Z}_{-(i,j)};d)\right]  + o_P(1)
%\end{align*}
%= & \frac{1}{Np} \sum_{i=1}^{N} \E\left[ \mu_i^2 (1, \mathbf{Z}_{-i};d)\right] - \frac{1}{N^2p}\sum_{i=1}^{N}\sum_{j\in \mathcal{B}(i)}^{N} \Cov\left[  \mu_i (1,1, \mathbf{Z}_{-(i,j)};d) \mu_j (1, 1,\mathbf{Z}_{-(i,j)};d)\right]  \\
%& - \frac{1}{N^2p}\sum_{i=1}^{N}\sum_{j\neq i}^{N} \E\left[  \mu_i (1,1, \mathbf{Z}_{-(i,j)};d)\right] \E\left[ \mu_j (1, 1,\mathbf{Z}_{-(i,j)};d)\right] + o_P(1) \\
%= & \frac{1}{Np} \sum_{i=1}^{N} \E\left[ \mu_i^2 (1, \mathbf{Z}_{-i};d)\right] - \frac{1}{N^2p}\sum_{i=1}^{N}\sum_{j\neq i}^{N} \E\left[  \mu_i (1,1, \mathbf{Z}_{-(i,j)};d)\right] \E\left[ \mu_j (1, 1,\mathbf{Z}_{-(i,j)};d)\right] + o_P(1)

The second part can be shown to be asymptotically unbiased in the same way. Now consider the first covariance part in the variance estimate, we have:
%\begin{align*}
%& \frac{1}{N} \sum_{i=1} \sum_{j \in \mathbf{B}(i)} \Cov[\mu_i(\Y(1, \Z_{-i}); d), \mu_j(\Y(1, \Z_{-j}); d)] \\
%= & \frac{1}{N} \sum_{i=1} \sum_{j \in \mathbf{B}(i)} \E[\mu_i(\Y(1, \Z_{-i}); d)\mu_j(\Y(1, \Z_{-j}); d)] \\
%& - \frac{1}{N} \sum_{i=1}\E[\mu_i(\Y(1, \Z_{-i}); d)] \sum_{j \in \mathbf{B}(i)} \E[\mu_j(\Y(1, \Z_{-j}); d)]. 
%\end{align*}.
%
%Notice that $\sum_{i=1}^{N_1}\sum_{j \in \mathcal{B}(i), Z_j = 1} \mu_i (d) = \sum_{i=1}^{N_1}\sum_{j \in \mathcal{B}(i), Z_j = 1} \mu_j (d) = \sum_{i=1}^{N_1} c_i^1 \mu_i (d)$, where $c_i^1 = \sum_{j \in \mathcal{B}(i)} Z_j$ is the number of treated nodes that depend on node $i$. It is easy to see that $\frac{c_i^1}{c_i} = \frac{\sum_{j \in \mathcal{B}(i) } Z_j}{c_i} = p + o_P(N^{-1/2})$.  The expectation of the corresponding estimate equals to:
\begin{align*}
&N\E\left[ \frac{1}{N_1^2} \sum_{i=1}^{N_1} \sum_{j \in \mathcal{B}(i), Z_j = 1} \left(\mu_i(\Y(\Z); d)  - \bar{\mu}_1 (d)\right) \left(\mu_j(\Y(\Z); d)  - \bar{\mu}_1 (d)\right)\right]\\
= & \frac{1}{N p^2} \sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)} \E \left[Z_iZ_j\mu_i(\Y(\Z); d) \mu_j(\Y(\Z); d) \right] \\
& - \frac{1}{N p^2} \E \left[\sum_{i=1}^{N}\sum_{j \in \mathcal{B}(i)} Z_i Z_j \bar{\mu}_1 (d) \left(\mu_i(\Y(\Z); d)  - \bar{\mu}_1 (d) +\mu_j(\Y(\Z); d) \right) \right]  + o_P(1) \\
= & \frac{1}{N} \sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)} \E \left[\mu_i (\Y(1, 1, \mathbf{Z}_{-(i,j)});d)\mu_j (\Y(1, 1, \mathbf{Z}_{-(i,j)});d)\right] \\
& - \frac{1}{N^2} \sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)}\sum_{k=1}^N \E \left[\mu_i (\Y(1, 1, \mathbf{Z}_{-(i,j)});d) \mu_k (\Y(1, \mathbf{Z}_{-k});d)\right] \\
& - \frac{1}{N^2} \sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)}\sum_{k=1}^N \E \left[\mu_j (\Y(1, 1, \mathbf{Z}_{-(i,j)});d) \mu_k (\Y(1, \mathbf{Z}_{-k});d)\right] \\
& + \frac{1}{N^2} \E\left(\sum_{k=1}^N  \mu_k (\Y(1, \mathbf{Z}_{-k});d)\right)^2 \\
= & \frac{1}{N} \sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)} \E \left[\mu_i (\Y(1, 1, \mathbf{Z}_{-(i,j)});d)\mu_j (\Y(1, 1, \mathbf{Z}_{-(i,j)});d)\right] \\
& - \frac{1}{N^2} \left(\sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)} \E \left[\mu_i (\Y(1, 1, \mathbf{Z}_{-(i,j)});d)\right]\right)\sum_{k=1}^N \E \left[\mu_k (\Y(1, \mathbf{Z}_{-k});d)\right] \\
& - \frac{1}{N^2} \left(\sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)} \E \left[\mu_j (\Y(1, 1, \mathbf{Z}_{-(i,j)});d)\right]\right)\sum_{k=1}^N \E \left[\mu_k (\Y(1, \mathbf{Z}_{-k});d)\right] \\
& + \frac{1}{N^2} \left(\sum_{k=1}^N \E \left[\mu_k (\Y(1, \mathbf{Z}_{-k});d)\right]\right)^2  + o_P(1) \\
= & \frac{1}{N}\sum_{i=1}^N\sum_{j\in \mathcal{B}(i)}\E\left[ \left(\mu_i(\Y(1, 1,\Z_{-(i,j)}); d) - \bar{\mu}^1(d) \right)\left(\mu_j(\Y(1, 1, \Z_{-(i,j)}); d) - \bar{\mu}^1(d) \right)\right]  + o_P(1).
\end{align*}
Similarly, the second to the last equality holds since
\begin{align*}
& \frac{1}{N^2} \sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)}\sum_{k=1}^N \E \left[\mu_i (\Y(1, 1, \mathbf{Z}_{-(i,j)});d) \mu_k (\Y(1, \mathbf{Z}_{-k});d)\right] \\
= & \frac{1}{N^2} \sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)}\sum_{k \in \mathcal{B}(i)} \E \left[\mu_i (\Y(1, 1, \mathbf{Z}_{-(i,j)});d) \mu_k (\Y(1, \mathbf{Z}_{-k});d)\right] \\
& + \frac{1}{N^2} \sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)}\sum_{k \notin \mathcal{B}(i)} \E \left[\mu_i (\Y(1, 1, \mathbf{Z}_{-(i,j)});d)\right] \E \left[\mu_k (\Y(1, \mathbf{Z}_{-k});d)\right] \\
= & \frac{1}{N^2} \sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)}\sum_{k \in \mathcal{B}(i)} \E \left[\mu_i (\Y(1, 1, \mathbf{Z}_{-(i,j)});d)\right] \E \left[\mu_k (\Y(1, \mathbf{Z}_{-k});d)\right] \\
& + \frac{1}{N^2} \sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)}\sum_{k \notin \mathcal{B}(i)} \E \left[\mu_i (\Y(1, 1, \mathbf{Z}_{-(i,j)});d)\right] \E \left[\mu_k (\Y(1, \mathbf{Z}_{-k});d)\right] + o_P(1)\\
= & \frac{1}{N^2} \sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)}\sum_{k =1}^N \E \left[\mu_i (\Y(1, 1, \mathbf{Z}_{-(i,j)});d)\right] \E \left[\mu_k (\Y(1, \mathbf{Z}_{-k});d)\right] + o_P(1) \\
= & \frac{1}{N^2} \left(\sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)} \E \left[\mu_i (\Y(1, 1, \mathbf{Z}_{-(i,j)});d)\right]\right)\sum_{k=1}^N \E \left[\mu_k (\Y(1, \mathbf{Z}_{-k});d)\right] + o_P(1).
\end{align*}

\begin{align*}
& \frac{1}{N^2} \sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)}\sum_{k=1}^N \E \left[\mu_j (\Y(1, 1, \mathbf{Z}_{-(i,j)});d) \mu_k (\Y(1, \mathbf{Z}_{-k});d)\right] \\
= & \frac{1}{N^2} \sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)}\sum_{k \in \mathcal{B}(j)} \E \left[\mu_j (\Y(1, 1, \mathbf{Z}_{-(i,j)});d) \mu_k (\Y(1, \mathbf{Z}_{-k});d)\right] \\
& + \frac{1}{N^2} \sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)}\sum_{k \notin \mathcal{B}(j)} \E \left[\mu_j (\Y(1, 1, \mathbf{Z}_{-(i,j)});d)\right] \E \left[\mu_k (\Y(1, \mathbf{Z}_{-k});d)\right] \\
= & \frac{1}{N^2} \sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)}\sum_{k =1}^N \E \left[\mu_j (\Y(1, 1, \mathbf{Z}_{-(i,j)});d)\right] \E \left[\mu_k (\Y(1, \mathbf{Z}_{-k});d)\right] + o_P(1) \\
= & \frac{1}{N^2} \left(\sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)} \E \left[\mu_j (\Y(1, 1, \mathbf{Z}_{-(i,j)});d)\right]\right)\sum_{k=1}^N \E \left[\mu_k (\Y(1, \mathbf{Z}_{-k});d)\right] + o_P(1).
\end{align*}
and
\begin{align*}
& \frac{1}{N^2} \E\left(\sum_{k=1}^N  \mu_k (\Y(1, \mathbf{Z}_{-k});d)\right)^2 \\
= & \frac{1}{N^2} \E\left(\sum_{k=1}^N  \mu_k (\Y(1, \mathbf{Z}_{-k});d) \sum_{l=1}^N  \mu_l (\Y(1, \mathbf{Z}_{-k});d)\right) \\
= & \frac{1}{N^2} \sum_{k=1}^N \sum_{l \in \mathcal{B}(k)} \E\left[\mu_k (\Y(1, \mathbf{Z}_{-k});d)   \mu_l (\Y(1, \mathbf{Z}_{-k});d)\right] \\
& + \frac{1}{N^2} \sum_{k=1}^N \sum_{l \notin \mathcal{B}(k)} \E\left[\mu_k (\Y(1, \mathbf{Z}_{-k});d)\right]  \E\left[\mu_l (\Y(1, \mathbf{Z}_{-k});d)\right]  \\
= & \frac{1}{N^2} \left(\sum_{k=1}^N \E \left[\mu_k (\Y(1, \mathbf{Z}_{-k});d)\right]\right)^2 + o_P(1).
\end{align*}
%The first part is exactly the corresponding term in the covariance's expression. For the second part to be asymptotically unbiased, we need an extra assumption on the asymptotic homogeneity of the dependency graph: $c_i = \tilde{c} + o_P(N^{-1})$ and $\sum_{j \in \mathbf{B}(i)} \E[\mu_j(\Y(1, \Z_{-j}); d)] = \frac{\sum_{i=1}^N\sum_{j \in \mathbf{B}(i)} \E[\mu_j(\Y(1, \Z_{-j}); d)] }{N}  + o_P(1)$. Under this assumption, $\frac{\sum_{i=1}^{N_1}c_i^1}{N_1} = \tilde{c} + o_P(N^{-1})$ and $\sum_{i=1}^{N_1}\left(2c_i^1  -  \frac{\sum_{i=1}^{N_1}c_i^1}{N_1} \right)\mu_i (d) = \sum_{i=1}^{N_1}\tilde{c}p\mu_i (d) + o_P(1)$. Moreover,
%\begin{align*}
%& \frac{1}{N^2} \sum_{i=1}\E[\mu_i(\Y(1, \Z_{-i}); d)] \sum_{j \in \mathbf{B}(i)} \E[\mu_j(\Y(1, \Z_{-j}); d)] \\
%= & \left(\frac{1}{N} \sum_{i=1}\E[\mu_i(\Y(1, \Z_{-i}); d)]\right)\left(\frac{1}{N^2} \sum_{i=1} \sum_{j \in \mathbf{B}(i)} \E[\mu_j(\Y(1, \Z_{-j}); d)]\right) + o_P(1) \\
%= & \left(\frac{1}{N} \sum_{i=1}\E[\mu_i(\Y(1, \Z_{-i}); d)]\right)\left(\frac{\tilde{c}}{N^2} \sum_{i=1} \E[\mu_j(\Y(1, \Z_{-j}); d)]\right) + o_P(1).
%\end{align*}.
%Remeber that $\bar{\mu}_1 (d) = \frac{1}{N} \sum_{i=1}\E[\mu_i(\Y(1, \Z_{-i}); d)] + o_P(1)$, we have:
%\begin{align*}
%& \frac{1}{N^2 p^2} \E \left[\bar{\mu}_1 (d) \sum_{i=1}^{N_1}\left(2c_i^1  -  \frac{\sum_{i=1}^{N_1}c_i^1}{N_1} \right)\mu_i (d)\right]  + o_P(1)  \\
%= & \frac{1}{N^2 p^2} \E \left[\bar{\mu}_1 (d) \sum_{i=1}^{N_1}\tilde{c}p\mu_i (d)\right]  + o_P(1)  \\
%= & \left(\frac{1}{N} \sum_{i=1}\E[\mu_i(\Y(1, \Z_{-i}); d)]\right)  \frac{1}{N^2 p^2} \E \left[\sum_{i=1}^{N_1}\tilde{c}p \mu_i (d)\right]  + o_P(1)  \\
%= & \left(\frac{1}{N} \sum_{i=1}\E[\mu_i(\Y(1, \Z_{-i}); d)]\right)  \left(\frac{\tilde{c}}{N^2} \sum_{i=1} \E[\mu_j(\Y(1, \Z_{-j}); d)]\right) + o_P(1).
%\end{align*}
%\begin{align*}
%&\E\left[ \frac{1}{N_1^2} \sum_{i=1}^{N_1} \sum_{j \in \mathcal{B}(i), Z_j = 1} \left(\mu_i (1, \mathbf{Z}_{-i};d) - \bar{\mu}_1 (d)\right) \left(\mu_j (1, \mathbf{Z}_{-j};d) - \bar{\mu}_1 (d)\right)\right]\\
%= & \frac{1}{N^2 p^2} \sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)} \E \left[Z_i\left(\mu_i (1, \mathbf{Z}_{-i};d) - \bar{\mu}_1 (d)\right)Z_j \left(\mu_j (1, \mathbf{Z}_{-j};d) - \bar{\mu}_1 (d)\right)\right]  + o_P(1) \\
%= & \frac{1}{N^2 p^2} \sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)} \E \left[Z_iZ_j\mu_i (1, \mathbf{Z}_{-i};d)\mu_j (1, \mathbf{Z}_{-j};d)\right] - \frac{1}{N^2 p^2} \sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)} \E \left[Z_iZ_j\mu_i (1, \mathbf{Z}_{-i};d)\bar{\mu}_1 (d)\right] \\
%& - \frac{1}{N^2 p^2} \sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)} \E \left[Z_iZ_j\mu_j (1, \mathbf{Z}_{-j};d)\bar{\mu}_1 (d)\right] + \frac{1}{N^2 p^2} \sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)} \E \left[Z_iZ_j\bar{\mu}_1^2 (d)\right]  + o_P(1) \\
%= & \frac{1}{N^2} \sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)} \E \left[\mu_i (1, 1, \mathbf{Z}_{-(i,j)};d)\mu_j (1, 1, \mathbf{Z}_{-(i,j)};d)\right] \\
%& - \frac{1}{N^2 p^2} \sum_{i=1}^{N}\E \left[\bar{\mu}_1 (d) \sum_{j \in \mathcal{B}(i)} Z_iZ_j\left(\mu_i (1, \mathbf{Z}_{-i};d) - \bar{\mu}_1 (d) +\mu_j (1, \mathbf{Z}_{-j};d)\right) \right]  + o_P(1) \\
%\end{align*}
%= & \frac{1}{N^2} \sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)} \E \left[\mu_i (1, \mathbf{Z}_{-i};d)\mu_j (1, \mathbf{Z}_{-j};d)\right] - \frac{1}{N^3 p^3} \sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)} \sum_{k=1}^{N} \E \left[Z_iZ_jZ_k\mu_i (1, \mathbf{Z}_{-i};d)\mu_k (1, \mathbf{Z}_{-k};d)\right] \\
%& - \frac{1}{N^3 p^3} \sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)}\sum_{k=1}^{N} \E \left[Z_iZ_jZ_k\mu_j (1, \mathbf{Z}_{-j};d)\mu_k (1, \mathbf{Z}_{-k};d)\right] + \frac{1}{N^2 p^2} \sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)} \E \left[Z_iZ_j\bar{\mu}_1^2 (d)\right] \\
%= & \frac{1}{N^2} \sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)} \E \left[\mu_i (1, \mathbf{Z}_{-i};d)\mu_j (1, \mathbf{Z}_{-j};d)\right] - \frac{1}{N^3 p} \sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i)} \E \left[\mu_i (1, 1, 1, \mathbf{Z}_{-i};d)\mu_k (1, \mathbf{Z}_{-k};d)\right] \\
%When $N \rightarrow \infty$, we can apply the dominated convergence theorem to the second term above, then:
%\begin{align*}
%& \lim_{N \rightarrow \infty} \frac{1}{N^2 p^2} \sum_{i=1}^{N}\E \left[\bar{\mu}_1 (d) \sum_{j \in \mathcal{B}(i)} Z_iZ_j\left(\mu_i (1, \mathbf{Z}_{-i};d) - \bar{\mu}_1 (d) +\mu_j (1, \mathbf{Z}_{-j};d)\right) \right] \\
%= & \frac{1}{N^2 p^2} \sum_{i=1}^{N}\E \left[\lim_{N \rightarrow \infty} \bar{\mu}_1 (d) \sum_{j \in \mathcal{B}(i)} Z_iZ_j\left(\mu_i (1, \mathbf{Z}_{-i};d) - \bar{\mu}_1 (d) +\mu_j (1, \mathbf{Z}_{-j};d)\right) \right] \\
%= & \frac{1}{N^2 p^2} \sum_{i=1}^{N} \E\left[\mu_i(1, \mathbf{Z}_{-i};d) \right] \E \left[ \sum_{j \in \mathcal{B}(i)} Z_iZ_j\left(\mu_i (1, \mathbf{Z}_{-i};d) - \E\left[\mu_i(1, \mathbf{Z}_{-i};d) \right] +\mu_j (1, \mathbf{Z}_{-j};d)\right) \right] \\
%= & \frac{1}{N^2} \sum_{i=1}^{N} \E\left[\mu_i(1, \mathbf{Z}_{-i};d) \right] \sum_{j \in \mathcal{B}(i)} \E \left[ \mu_j (1,1, \mathbf{Z}_{-(i,j)};d) \right] \\
%\end{align*}

%(What remains to be shown here is that $\sum_{i=1}^N \sum_{j\neq i}^N \E\left[\mu_i(\Y(1, \Z_{-i}); d)\mu_j(\Y(1, \Z_{-j}); d)\right] = \sum_{i=1}^N \sum_{j\neq i}^N \E\left[\mu_i(\Y(1, 1, \Z_{-(i,j)}); d)\mu_j(\Y(1, 1, \Z_{-(i,j)}); d)\right]$).

The other terms can be similarly shown. Hence, 
\begin{align*}
& \E\left[ N\widehat{\Var}(\hat{\tau}_{d, OLS}) \right] \\
= & \frac{1}{Np}\sum_{i=1}^N\E\left[\mu_i(\Y(1, \Z_{-i}); d) - \bar{\mu}^1(d) \right]^2 + \frac{1}{N(1-p)}\sum_{i=1}^N\E\left[\mu_i(\Y(0, \Z_{-i}); d) - \bar{\mu}^0(d) \right]^2 \\
& + \frac{1}{N}\sum_{i=1}^N\sum_{j\in \mathcal{B}(i)}\E\left[ \left(\mu_i(\Y(1, 1,\Z_{-(i,j)}); d) - \bar{\mu}^1(d) \right)\left(\mu_j(\Y(1, 1, \Z_{-(i,j)}); d) - \bar{\mu}^1(d) \right)\right] \\
& + \frac{1}{N}\sum_{i=1}^N\sum_{j\in \mathcal{B}(i)}\E\left[ \left(\mu_i(\Y(0, 0,\Z_{-(i,j)}); d) - \bar{\mu}^0(d) \right)\left(\mu_j(\Y(0, 0, \Z_{-(i,j)}); d) - \bar{\mu}^0(d) \right)\right] \\
& - \frac{2}{N}\sum_{i=1}^N \sum_{j\in \mathcal{B}(i)} \E\left[ \left(\mu_i(\Y(1,0,\Z_{-(i,j)}); d) - \bar{\mu}^1(d) \right)\left(\mu_j(\Y(1,0,\Z_{-(i,j)}); d) - \bar{\mu}^0(d) \right)\right] + o_P(1)\\
\geq & N \Var \left[\hat{\tau}_{HA}(d)\right].
\end{align*}

%\begin{align*}
%& N \Var \left[\hat{\tau}_{HA}(d)\right] - N\widehat{\Var}(\hat{\tau}_{d, OLS}) \\
%= & \frac{2}{N^2} \sum_{i=1}^N \sum_{j\in \mathcal{B}(i)} (\E\left[\mu_i(\Y(1, 0, \Z_{-(i,j)}); d) \right] + \E\left[\mu_i(\Y(0, 1, \Z_{-(i,j)}); d) \right] \\
%& - \E\left[\mu_i(\Y(1, 1, \Z_{-(i,j)}); d) \right] - \E\left[\mu_i(\Y(0, 0, \Z_{-(i,j)}); d) \right] ) ) \\
%& * \left((1-p)\sum_{i=1}^N  \E\left[\mu_i(\Y(1, \Z_{-i}); d) \right] + p\sum_{i=1}^N \E\left[\mu_i(\Y(0, \Z_{-i}); d) \right]\right) 
%\end{align*}
%This term is the difference between the average indirect effect on the untreated units and that on the treated units. When it converges to zero, the spatial HAC variance is an asymptotically unbiased estimate of the Hajek estimator's variance.
\end{document}




==> proofs/reference/variance_expression_old.tex <==
\input{tex-header}
\begin{document}
We develop the derivation for the component in expression 1 that corresponds to the variance of the treated intervention points' circle averages.  Results for the control intervention points and then the covariance of the two would follow.  First, define $\mathcal{B}(i; d)$ as the set of intervention points whose treatment statuses affect the potential circle averages for intervention point $i$, and $c_i$ as the number of intervention points in $\mathcal{B}(i; d)$. (Note that intervention points outside of $\mathcal{B}(i; d)$ do not necessarily satisfy condition C3 with respect to $i$.)  Let $\z_{\mathcal{B}(i; d)}$ and $\mathcal{Z}_{\mathcal{B}(i; d)}$ correspond to realized and feasible ordered treatment vectors for units in $\mathcal{B}(i; d)$.  Then, let $I_j(\z_{\mathcal{B}(i; d)})$ be an indicator variable for whether the treatment indicator at intervention point $j$ equal's point $j$'s entry in the vector $\z_{\mathcal{B}(i; d)}$.  With these terms, we can rewrite  the expression for the total of treated circle averages in terms of random selection indicators and then fixed potential circle averages:
\begin{align*}
\sum_{i=1}^N Z_i \mu_i(\Y; d) & = \sum_{i=1}^N Z_i \sum_{\z_{-i}\in \mathcal{Z}_{-i}}I(\Z_{-i}=\z_{-i}) \mu_i(\Y(1, \z_{-i}); d)\\
& =  \sum_{i=1}^N Z_i \sum_{\z_{\mathcal{B}(i; d)} \in \mathcal{Z}_{\mathcal{B}(i; d)}} I(\Z_{\mathcal{B}(i; d)}=\z_{\mathcal{B}(i; d)}) \mu_i(\Y(1, \z_{\mathcal{B}(i; d)}); d) \\
& \equiv \sum_{i=1}^N T_i.
\end{align*}
In the expression above, only $Z_i$ and $I_j(\z_{\mathcal{B}(i; d)})$ are random, while $\mu_i(\Y(1, \z_{\mathcal{B}(i; d)}); d)$ is a fixed potential circle average.  Then we have,
\begin{align*}
\Var\left[\sum_{i=1}^N T_i\right] = \sum_{i=1}^N \Var[T_i] + \sum_{i=1}^N\sum_{j \ne i} \Cov[T_i, T_j]. 
\end{align*}
By Bernoulli assignment, we have that $\Cov[T_i, T_j] = 0$. (The logic is a straightforward extension of Frank (1977)  Then, applying the expression for the variance of a product of independent variables due to (Goodman, 1962), we have,
\begin{align*}
\Var\left[\sum_{i=1}^N T_i\right]  & =\sum_{i=1}^N \Var\bigg[ Z_i  \sum_{\z_{\mathcal{B}(i; d)} \in \mathcal{Z}_{\mathcal{B}(i; d)}} I(\Z_{\mathcal{B}(i; d)}=\z_{\mathcal{B}(i; d)})\mu_i(\Y(1, \z_{\mathcal{B}(i; d)}); d)\bigg] \\
& = \sum_{i=1}^N \bigg\{  \sum_{\z_{\mathcal{B}(i; d)} \in \mathcal{Z}_{\mathcal{B}(i; d)}} \Var\left[Z_i  I(\Z_{\mathcal{B}(i; d)}=\z_{\mathcal{B}(i; d)})\right]\mu_i(\Y(1, \z_{\mathcal{B}(i; d)}); d)^2\\
& \hspace{1em}+ \sum_{\z_{\mathcal{B}(i; d)} \in \mathcal{Z}_{\mathcal{B}(i; d)}} \sum_{\z'_{\mathcal{B}(i; d)} \ne  \z_{\mathcal{B}(i; d)}} \Cov \bigg[ Z_i  I(\Z_{\mathcal{B}(i; d)}=\z_{\mathcal{B}(i; d)}), Z_i  I(\Z_{\mathcal{B}(i; d)}=\z_{\mathcal{B}(i; d)}^{'})\bigg]\\
& \hspace{2em}\times \mu_i(\Y(1, \z_{\mathcal{B}(i; d)}); d)\mu_i(\Y(1, \z'_{\mathcal{B}(i; d)}); d) \bigg\}\\
& = \sum_{i=1}^N \bigg\{ \sum_{\z_{\mathcal{B}(i; d)}}\bigg[ p\E[I(\Z_{\mathcal{B}(i; d)}=\z_{\mathcal{B}(i; d)})] - p^2 \E[I(\Z_{\mathcal{B}(i; d)}=\z_{\mathcal{B}(i; d)})]^2\bigg] \mu_i(\Y(1, \z_{\mathcal{B}(i; d)}); d)^2 \\
& \hspace{3em} -  p^2  \bigg[ \sum_{\z_{\mathcal{B}(i; d)} \in \mathcal{Z}_{\mathcal{B}(i; d)}} \sum_{\z'_{\mathcal{B}(i; d)} \ne  \z_{\mathcal{B}(i; d)}} \E[I(\Z_{\mathcal{B}(i; d)}=\z_{\mathcal{B}(i; d)})]  \E[I(\Z_{\mathcal{B}(i; d)}=\z_{\mathcal{B}(i; d)}^{'})] \\
& \hspace{6em} \times \mu_i(\Y(1, \z_{\mathcal{B}(i; d)}); d)\mu_i(\Y(1, \z'_{\mathcal{B}(i; d)}); d)\bigg] \bigg\}.
\end{align*}
Denote the number of treated intervention points in $\mathcal{B}(i; d)$ as $n_{t, c_i}$. It is easy to see that 
\begin{align*}
& \sum_{\z_{\mathcal{B}(i; d)}}p\E[I(\Z_{\mathcal{B}(i; d)}=\z_{\mathcal{B}(i; d)})] \mu_i(\Y(1, \z_{\mathcal{B}(i; d)}); d)^2\\
= & \sum_{n_{t, c_i} = 0}^{c_i} \begin{pmatrix}
c_i \\ n_{t, c_i}
\end{pmatrix} p\prod_{j \in \mathcal{B}(i; d)}\E[I_j(\z_{\mathcal{B}(i; d)})] \\
= & \sum_{n_{t, c_i} = 0}^{c_i} \begin{pmatrix}
c_i \\ n_{t, c_i}
\end{pmatrix} p* p^{n_{t, c_i}}(1-p)^{c_i - n_{t, c_i}}
\end{align*}
Hence 
\begin{align*}
& \sum_{\z_{\mathcal{B}(i; d)}}\bigg[ p\prod_{j \in \mathcal{B}(i; d)}\E[I_j(\z_{\mathcal{B}(i; d)})] - p^2 \prod_{j \in \mathcal{B}(i; d)} \E[I_j(\z_{\mathcal{B}(i; d)})]^2\bigg] \mu_i(\Y(1, \z_{\mathcal{B}(i; d)}); d)^2 \\
= & \sum_{n_{t, c_i} = 0}^{c_i} \begin{pmatrix}
c_i \\ n_{t, c_i}
\end{pmatrix} p* p^{n_{t, c_i}}(1-p)^{c_i - n_{t, c_i}}\mu_i(\Y(1, \z_{\mathcal{B}(i; d)}); d)^2 \\
& - \sum_{n_{t, c_i} = 0}^{c_i} \begin{pmatrix}
c_i \\ n_{t, c_i}
\end{pmatrix} p^{2}* p^{2n_{t, c_i}}(1-p)^{2(c_i - n_{t, c_i})}\mu_i(\Y(1, \z_{\mathcal{B}(i; d)}); d)^2 \\
= & \sum_{n_{t, c_i} = 0}^{c_i} \begin{pmatrix}
c_i \\ n_{t, c_i}
\end{pmatrix} p* p^{n_{t, c_i}}(1-p)^{c_i - n_{t, c_i}}\left(1-p* p^{n_{t, c_i}}(1-p)^{c_i - n_{t, c_i}}\right)\mu_i(\Y(1, \z_{\mathcal{B}(i; d)}); d)^2
\end{align*}
Similarly
\begin{align*}
& \sum_{\z_{\mathcal{B}(i; d)} \in \mathcal{Z}_{\mathcal{B}(i; d)}} \sum_{\z'_{\mathcal{B}(i; d)} \ne  \z_{\mathcal{B}(i; d)}} \prod_{j \in \mathcal{B}(i; d)} \E[I_j(\z_{\mathcal{B}(i; d)})]\E[I_j(\z'_{\mathcal{B}(i; d)})] \times \mu_i(\Y(1, \z_{\mathcal{B}(i; d)}); d)\mu_i(\Y(1, \z'_{\mathcal{B}(i; d)}); d) \\
= & \sum_{n_{t, c_i} = 0}^{c_i} \begin{pmatrix}
c_i \\ n_{t, c_i}
\end{pmatrix} \left[ \begin{pmatrix}
c_i \\ n_{t, c_i}
\end{pmatrix} - 1 \right] p^{2n_{t, c_i}}(1-p)^{2(c_i - n_{t, c_i})}\mu_i(\Y(1, \z_{\mathcal{B}(i; d)}); d)\mu_i(\Y(1, \z'_{\mathcal{B}(i; d)}); d) \\
+ & \sum_{n_{t, c_i} = 0}^{c_i}\sum_{n_{t', c_i} = 0}^{c_i} \begin{pmatrix}
c_i \\ n_{t', c_i}
\end{pmatrix} \begin{pmatrix}
c_i \\ n_{t', c_i}
\end{pmatrix}  p^{n_{t, c_i}+n_{t', c_i}}(1-p)^{2c_i - n_{t, c_i} - - n_{t', c_i}}\mu_i(\Y(1, \z_{\mathcal{B}(i; d)}); d)\mu_i(\Y(1, \z'_{\mathcal{B}(i; d)}); d) \\
\end{align*}

For simplicity, we now rearrange the sample such that treated observations lie before observations under control and outcome points around the same intervention node stand next to each other. We also assume that each circle consists of the same number of outcome points. The number is denoted as $N_d$. Let's further denote the intervention node $i$ whose circle contains point $x$ as $i_x$, and its treatment status as $Z_x$.

From the regression representation, we know that $\mathbf{Y} = \mathbf{X}_d \hat{\tau}_d + \mathbf{e}_d$, where $\mathbf{Y}$ is the outcome values at all the points we take when constructing circle means, and $\mathbf{X}_d = \mathbf{W}_{d}^{'} (\mathbf{W}_d \mathbf{W}_{d}^{'})^{-1}$ is a $|\mathcal{X}|\times 1$ vector. Remeber that $\mathbf{W}_d = \frac{\mathbf{Z}' - p}{p(1-p)}\mathbf{M}_d$. Hence, the $x$th column of $\mathbf{W}_d$, $W_{dx}$, is equal to $\frac{N_{dx, tr} - pN_{dx}}{N_d p(1-p)}$, where $N_{dx, tr}$ is the number of treated nodes that are $d$ units away from point $x$, and $N_{dx, tr}$ is the total number of intervention nodes that are $d$ units away from point $x$. By the construction of $\mathbf{M}_d$, we know that $W_{dx} = \frac{Z_x - p}{N_d p(1-p)}$ In addition, $\mathbf{W}_d \mathbf{W}_{d}^{'}$ is a constant. Its value equals to $\frac{\mathbf{Z}' - p}{p(1-p)}\mathbf{M}_d \mathbf{M}_{d}^{'} \frac{\mathbf{Z} - p}{p(1-p)} = \frac{[N_1(1-p)+N_0 p]^2}{N_d p^2 (1-p)^2}$. We denote it as $c_W$. Then each row of $\mathbf{e}_d$, $e_{dx}$, is equal to $Y_x - \frac{Z_x - p}{c_W N_d p(1-p)} \hat{\tau}_d = Y_x - \frac{W_{dx}}{c_W}(\bar{\mu}_1- \bar{\mu}_0)$, where $\bar{\mu}_1 = \frac{1}{Np} \sum_i Z_i \mu_i(\mathbf{Y})$ and $\bar{\mu}_0 = \frac{1}{N(1-p)} \sum_i (1-Z_i) \mu_i(\mathbf{Y})$.

The spatial HAC, or Conley standard errors of $\hat{\tau}_d$ can be written as:

\begin{align*}
Var(\hat{\tau}_d) = & (\mathbf{X}_{d}\mathbf{X}_{d}^{'})^{-1}(\mathbf{X}_{d} \Sigma \mathbf{X}_{d}^{'})(\mathbf{X}_{d}\mathbf{X}_{d}^{'})^{-1} \\
= & \mathbf{W}_{d}^{'} \Sigma \mathbf{W}_{d} \\
= & \frac{1}{|\mathcal{X}|} \sum_x \sum_y W_{dx} W_{dy} e_{dx} e_{dy} \mathbf{1}\{d_{xy} \leq d_{cutoff} \} \\
= & \frac{1}{|\mathcal{X}|} \sum_x \sum_y W_{dx} W_{dy} \left[Y_x - \frac{W_{dx}}{c_W}(\bar{\mu}_1- \bar{\mu}_0)\right] \left[Y_y - \frac{W_{dy}}{c_W}(\bar{\mu}_1- \bar{\mu}_0)\right] \mathbf{1}\{d_{xy} \leq d_{cut} \}
\end{align*}
where $d_{xy}$ is the distance between point $x$ and $y$, $d_{cut}$ is the chosen threshold. We should choose $d_{cut}$ such that whenever $d_{xy} > d_{cut}$, $x_i$ and $y_i$ satisfy the local independence condition.

\end{document}




==> proofs/sampling-based-results.tex <==
%\input{tex-header}
%\begin{document}
%\section*{Population-based perspective}
%Consider a metric space $\mathcal{X}$ equipped with a distance metric $d$. For each point $x \in \mathcal{X}$, we observe its outcome $Y_x$. We assume that either of following two possibilities holds: First, there exists a (potentially irregular) lattice embedded in $\mathcal{X}$. The distance between any two vertexes in the lattice satisfies our condition C4: $d \geq d_0$. Second, there is a partition of $\mathcal{X}$. Each set in the partition is convex and has an area larger than $s_0$, hence satisfying our condition C4.a.  The total number of vertexes in the lattice or of convex sets in the partition is denoted as $n$, where $n$ is sufficiently large.
%
%We randomly sample $N$ vertexes from the lattice or $N$ convex sets from the partition with probability $\omega_N$ as intervention nodes in a spatial experiment, where $\omega_N \rightarrow \omega > 0$. We use $W_i \in \{0, 1\}$ to denote whether a node is sampled. Obviously, the two scenarios correspond to point and polygon interventions discussed in the main text. Each node $i \in \{1,2,\dots,N\}$ in assigned into the treatment group with probability $p$. The outcome at each point $x$ now is jointly  decided by the treatment assignment vector $\mathbf{Z}^{(N)}$: $Y_x = Y_x(\mathbf{Z}^{(N)})$. We use the superscript $(N)$ to emphasize the fact that the assignment is based on the given sample with size $N$.
%For each point $x$ in the set $\mathcal{X}$, we assume that there exist a continuum of potential outcomes: $\mu_x(1;d)$ and $\mu_x(0;d)$ for any $d \in [0, \bar d]$. In addition, $\mu_x(1; d) \sim f_1(x;d)$ and $\mu_x(0; d) \sim f_0(x;d)$, where $f_1(x;d)$ and $f_0(x;d)$ are density functions with finite moments up to the fourth one. Define $\theta_1(d) = \E \left[\mu_x(1;d)\right]$ and $\theta_0(d) = \E \left[\mu_x(0;d)\right]$. 

%Consider a population with $n$ units. Following the convention in spatial econometrics, we assume that the $n$ units are embedded in a (potentially irregular) lattice. The distance between any two vertexes in the lattice satisfies our condition C4: $d \geq d_0$. As $n$ grows, the lattice remains inside the set $\mathcal{X}$. In other words, each unit $i \in \{1,2,\dots, n\}$ is represented by a point $x(i)$ in $\mathcal{X}$ for any $n$. The individualistic treatment effect at $d$ is $\tau_{i}(d) = \mu_{x(i)}(1;d) - \mu_{x(i)}(0;d)$ and the population average treatment effect (PATE) at $d$ is defined as $\tau_{PATE,n}(d) = \frac{1}{n}\sum_{i=1}^n  \tau_{i}(d)$.

%We define $\mu_i(d) = \mu_i(Y(\mathbf{Z}^{(N)});d)$ and $\E[\mu_i(z;d)] = \E_{\mathbf{Z}_{-i}^{(N)}}[\mu_i(Y(\mathbf{Z}^{(N)});d)]$ as in the main text. Now, the sample average treatment effect (SATE) at $d$ is defined as $\tau_{SATE,N}(d) = \frac{1}{N}\sum_{i=1}^{N}  \tau_{i}(d) = \frac{1}{N}\sum_{i=1}^{N}  (\E[\mu_i(1;d)] - \E[\mu_i(0;d)])$. Similarly, the population average treatment effect (PATE) at $d$ is defined as $\tau_{PATE}(d) = \frac{1}{n}\sum_{i=1}^{n}  \tau_{i}(d) = \mathbb{E}[\tau_{SATE, N}(d)]$, where $\mathbb{E}$ is the expectation over sampling. We already know that for an estimate $\hat \tau_{SATE,N}(d)$ from either the Horvitz-Thompson estimator or the Hajek estimator, the central limit theorem holds: 
%$$
%\sqrt{N}\left(\hat \tau_{SATE,N}(d) - \tau_{SATE,N}(d)\right) \rightarrow \mathcal{N}(0, N\sigma^2(d))
%$$ 
%as $N \rightarrow \infty$, where $\sigma^2(d)$ is the corresponding variance of the estimator.

%Clearly, $\{\mu_i(1;d)\}_{d \in [0, \bar d]}$ and $\{\mu_i(0;d)\}_{d \in [0, \bar d]}$ are two stochastic processes indexed by $d$ on the sample $\{1,2,\dots, N\}$. 

%We define the population average treatment effect (PATE) at $d$ as $\tau_{PATE}(d) = \lim_{N \rightarrow \infty} \tau_{SATE,N}(d)$ and $\theta_0(d) = \lim_{N \rightarrow \infty}\frac{1}{N}\sum_{i=1}^{N}\mu_i(0;d)$, then
%\begin{align*}
%\mu_i(d) = \theta_0(d) + \tau_{PATE}(d)Z_i + \nu_i(d),
%\end{align*}
%where 
%$$
%\begin{aligned}
%\nu_i(d) = & \mu_i(d) - \theta_0(d) -  \tau_{PATE}(d)Z_i \\
%= & \mu_i(d) - \frac{1}{N}\sum_{i=1}^{N}\mu_i(0;d)  - \tau_{SATE, N}(d)Z_i \\
%& + \frac{1}{N}\sum_{i=1}^{N}\mu_i(0;d) - \theta_0(d) + \left(\tau_{SATE, N}(d) - \tau_{PATE}(d)\right)Z_i \\
%= & \nu_i^{\dagger}(d) + \nu_i^{\ddagger}(d).
%\end{aligned}
%$$
%Without loss of generality, we assume that $\nu_i(d) \sim \mathcal{N}(0, \sigma^2(d))$. We later show that replacing the Normally distributed $\nu_i(d)$ with any stochastic distribution won't affect our results. 

%Since $\E \left[\frac{N_n}{n}\right] = \omega_n \rightarrow \omega$, $N_n$ grows to infinity as $n \rightarrow \infty$.  Hence, from previous sections, we know that 
%
%\begin{align*}
%\frac{\hat \tau_{HA}(d) - \tau_{SATE, N_n}(d)}{\sigma(d)} \rightarrow N(0, 1).
%\end{align*}
%Since $\tau_{SATE, N_n}(d) - \tau_{PATE, n}(d) \rightarrow 0$, we know that
%\begin{align*}
%\frac{\hat \tau_{HA}(d) - \tau_{PATE, N_n}(d)}{\sigma(d)} \rightarrow N(0, 1)
%\end{align*}
%from Slutsky's lemma.
%The experimental design ensures that $\kappa$ and $\mu$ are independent to each other. 
%\section*{Confidence intervals for the kernel regression estimator}
%We assume that the true DGP is 
%\begin{align*}
%\mu_i(d) = \theta_0(d) + \tau_{PATE}(d)Z_i + \nu_i(d),
%\end{align*}
Assuming that each $d \in \mathcal{D}$ and $|\mathcal{D}| = J$, there are in total $N * J$ circle average observations in our sample that we use to estimate an AME curve. For each  $\mu_i(d)$, we have
$$
\begin{aligned}
\mu_i(d) = \bar{\mu}^0(d) + Z_i \tau(d; \eta) +  + \varepsilon_i(d) = a(d) + Z_i \tau(d) +  \varepsilon_i(d),
\end{aligned}
$$
where
$$
\begin{aligned}
a(d) = & \bar{\mu}^0(d), \tau(d) = \tau(d; \eta), \\
\varepsilon_i(d) = & Z_i (\mu_i(Y(1, \mathbf{Z}_{-i});d) - \mu_i(Y(0, \mathbf{Z}_{-i});d) - \tau(d; \eta)) + \mu_i(Y(0, \mathbf{Z}_{-i});d)  - \bar{\mu}^0(d).
\end{aligned}
$$
Suppose that $d$ values are indexed as  $\{d_1, d_2, \dots, d_J\}$. We impose two structural restrictions on the data generating process to motivate a kernel regression estimator to estimate the AME curve:
\begin{itemize}
\item[1.] $a(d) = \tilde{a}\left(\frac{d}{d_J}\right)$ and $\tau(d) = \tilde{\tau}\left(\frac{d}{d_J}\right)$; both $\tilde{a}()$ and $\tilde{\tau}()$ are are smooth functions on $[0, 1]$ with the $S$ times continuously differentiable;
\item[2.] $\varepsilon_i(d)$ are weakly correlated across units and over distance values, which means that $\frac{1}{N^2J}\sum_{j=1}^J \sum_{i=1}^N \sum_{i'=1}^N \varepsilon_i(d_j) \varepsilon_{i'}(d_{j}) \leq C_2$ and $\frac{1}{NJ^2}\sum_{j=1}^J \sum_{j'=1}^J \sum_{i=1}^N  \varepsilon_i(d_j) \varepsilon_{i}(d_{j'}) \leq C_1$ for constants $C_1$ and $C_2$.
\end{itemize}
Both parts of the second restriction are guaranteed by our assumption C4a. The first restriction is satisfied in various scenarios. For example, when the effects are smooth and additive across intervention nodes, as in Section \ref{struc-int}, we know that $\tau(d; \eta)$ is the circle average of several effect functions, all of which have continuous directional derivatives along any direction. Therefore, $\tau(d; \eta)$ is a smooth function of distance $d$.

%For each outcome $\mu_i(d)$, we know that
%$$
%\begin{aligned}
%\mu_i(d) = & Z_i \mu_i(Y(1, \mathbf{Z}^{(N)}_{-i});d) + (1-Z_i) \mu_i(Y(0, \mathbf{Z}^{(N)}_{-i});d) \\
%= & Z_i (\mu_i(Y(1, \mathbf{Z}^{(N)}_{-i});d) - \mu_i(Y(0, \mathbf{Z}^{(N)}_{-i});d)) + \mu_i(Y(0, \mathbf{Z}^{(N)}_{-i});d) \\
%= & Z_i \tau_i(d) + \mu_i(Y(0, \mathbf{Z}^{(N)}_{-i});d) \\
%& + Z_i (\mu_i(Y(1, \mathbf{Z}^{(N)}_{-i});d) - \mu_i(Y(0, \mathbf{Z}^{(N)}_{-i});d) - \tau_i(d)) \\
%= & Z_i \tau_{PATE}(d) + \mathbb{E}[\E[\mu_i(0;d)]] + e_i(d), \\
%= & a(d) + Z_i \tau(d) +  \varepsilon_i(d),
%\end{aligned}
%$$
%where
%$$
%\begin{aligned}
%a(d) = & \mathbb{E}[\E[\mu_i(0;d)]]. \\
%\tau(d) = & \tau_{PATE}(d), \\
%\varepsilon_i(d) = & Z_i (\mu_i(Y(1, \mathbf{Z}^{(N)}_{-i});d) - \mu_i(Y(0, \mathbf{Z}^{(N)}_{-i});d) - \tau_{PATE}(d)) \\
%& + \mu_i(Y(0, \mathbf{Z}^{(N)}_{-i});d)  - \mathbb{E}[\E[\mu_i(0;d)]].
%\end{aligned}
%$$
%It is clear that $\mathbb{E}[\E[\mu_i(d)]] = a(d) + Z_i\tau(d)$ and $\varepsilon_i(d) = \mu_i(d) - \mathbb{E}[\E[\mu_i(d)]]$. We impose two structural restrictions on the data generating process so that we can rely on the kernel regression estimator to estimate the AMR:
%\begin{itemize}
%\item[1.] $a(d) = \tilde{a}\left(\frac{d}{d_J}\right)$ and $\tau(d) = \tilde{\tau}\left(\frac{d}{d_J}\right)$; both $\tilde{a}()$ and $\tilde{\tau}()$ are are smooth functions on $[0, 1]$ with the $S$ times continuously differentiable;
%\item[2.] $e_i(d)$ are weakly correlated across units and over distance values, which means that $\frac{1}{N^2J}\sum_{j=1}^J \sum_{i=1}^N \sum_{i'=1}^N e_i(d_j) e_{i'}(d_{j}) \leq C_2$ and $\frac{1}{NJ^2}\sum_{j=1}^J \sum_{j'=1}^J \sum_{i=1}^N  e_i(d_j) e_{i}(d_{j'}) \leq C_1$ for constants $C_1$ and $C_2$.
%\end{itemize}
%Both parts of the second restriction are guaranteed by our condition C5. The first restriction is satisfied in various scenarios. For example, when the effects are structural and additive across intervention nodes, we know that $\mu_i(Y(1, \mathbf{Z}^{(N)}_{-i});d) - \mu_i(Y(0, \mathbf{Z}^{(N)}_{-i});d) = \tau_{PATE}(d) = f(d)$, hence $e_i(d) = \mu_i(Y(0, \mathbf{Z}^{(N)}_{-i});d)  - \mathbb{E}[\E[\mu_i(0;d)]]$. It is obvious from condition C5 that $e_i(d)$ is correlated with a fixed number of $e_i(d')$. 


%All the estimators we propose take the form of a linear combination of the outcome values:
%$$
%\hat \tau(d)  = \sum_{i=1}^N \sum_{d' \in \tilde{D}} \kappa_i(d';d) \mu_{i}(d') = \kappa^{'}(d)\mu
%$$
%for any $d \in \tilde{D}$, where $\kappa(d) = (\kappa_1(d_1;d),\kappa_2(d_1;d),\dots, \kappa_N(d_{J};d))$ and $\mu = (\mu_1(d_1),\mu_2(d_1),\dots, \mu_N(d_{J}))$. For example,
%$$
%\kappa_i(d';d) = \begin{cases} 0, \text{ if } d' \neq d \\ \frac{Z_i - p}{Np(1-p)}, \text{ if } d' = d \end{cases}
%$$
%in the Horvitz-Thompson estimator. 

We consider the asymptotics where $N$ grows to infinity and $J$ remains fixed, as in \citet{robinson2012nonparametric}. In the kernel regression estimator, we have the $(N * J)\times 4$ matrix of regressors
$$
\mathbf{X}^{\dagger}(d) = \begin{pmatrix}
1 & Z_1 & (d_1 - d) &  Z_1 * (d_1 - d) \\
\vdots & \vdots & \vdots &  \vdots \\
1 & Z_N & (d_1 - d) &  Z_N * (d_1 - d) \\
1 & Z_1 & (d_2 - d) &  Z_1 * (d_2 - d) \\
\vdots & \vdots & \vdots &  \vdots \\
1 & Z_N & (d_{J} - d) &  Z_N * (d_{J} - d)
\end{pmatrix}  
$$
and the $(N * J)\times (N * J)$ matrix of kernel weights
$$
\mathbf{W}^{K}_h(d) = \begin{pmatrix}
K\left(\frac{d_1 - d}{h}\right) &  &  &  & \\
&  \ddots & & & \\
 &  & K\left(\frac{d_1 - d}{h}\right) & &  \\
 &  & & \ddots &  \\
&  & & & K\left(\frac{d_{J} - d}{h}\right)
\end{pmatrix}.
$$
%\begin{pmatrix}
%1 & 0 & 0 & 0 \\
%0 & 0 & 0 & 0 \\
%0 & 0 & 0 & 0 \\
%0 & 0 & 0 & 0 \\
%\end{pmatrix}
Then, $\hat \tau_K(d)$ equals to the second row of
$$
\begin{aligned}
\hat \beta(d) = & \left(\mathbf{X}^{\dagger '}(d)\mathbf{W}^{K}_h(d)\mathbf{X}^{\dagger}(d) \right)^{-1}\left(\mathbf{X}^{\dagger '}(d)\mathbf{W}^{K}_h(d)\mu \right) \\
= & \mathbf{P}(d)\E\mu + \mathbf{P}(d)\varepsilon
\end{aligned}
$$
where $\mathbf{P}(d) = \left(\mathbf{X}^{\dagger '}(d)\mathbf{W}^{K}_h(d)\mathbf{X}^{\dagger}(d) \right)^{-1}\left(\mathbf{X}^{\dagger '}(d)\mathbf{W}^{K}_h(d) \right)$, $\E\mu = \begin{pmatrix}
\E[\mu_1(d_1)] \\
\E[\mu_2(d_1)] \\
\vdots  \\
\E[\mu_N(d_J)]
\end{pmatrix}$, and $\varepsilon = \begin{pmatrix}
\varepsilon_1(d_1)\\
\varepsilon_2(d_1) \\
\vdots  \\
\varepsilon_N(d_J)
\end{pmatrix}$.

%Remember that
%$$
%\begin{pmatrix}
%\mu_{1}(d) \\
%\vdots \\
%\mu_{N}(d)
%\end{pmatrix}  = \begin{pmatrix}
%\frac{\mathbf{1}\{d_1(x_{1}) = d\}}{\sum_{x \in \mathcal{X}} \mathbf{1}\{d_1(x) = d\}} & \frac{\mathbf{1}\{d_1(x_{2}) = d\}}{\sum_{x \in \mathcal{X}} \mathbf{1}\{d_1(x) = d\}} & \dots & \frac{\mathbf{1}\{d_1(x_{|\mathcal{X}|}) = d\}}{\sum_{x \in \mathcal{X}} \mathbf{1}\{d_1(x) = d\}} \\
%\vdots & \vdots & \ddots & \vdots \\
%\frac{\mathbf{1}\{d_N(x_{1}) = d\}}{\sum_{x \in \mathcal{X}} \mathbf{1}\{d_N(x) = d\}} & \frac{\mathbf{1}\{d_N(x_{2}) = d\}}{\sum_{x \in \mathcal{X}} \mathbf{1}\{d_N(x) = d\}}& \dots & \frac{\mathbf{1}\{d_N(x_{|\mathcal{X}|}) = d\}}{\sum_{x \in \mathcal{X}} \mathbf{1}\{d_N(x) = d\}}
%\end{pmatrix} \begin{pmatrix}
%Y_{1} \\
%\vdots \\
%Y_{|\mathcal{X}|}
%\end{pmatrix}.
%$$
%Plugging the expression into the estimator, we have,
%$$
%\begin{pmatrix}
%\hat \theta(d) \\
%\hat \tau(d)
%\end{pmatrix}  = \sum_{x \in \mathcal{X}} \tilde{\omega}_x(d) \Y_{x}
%$$
Note that $\mathbf{X}^{\dagger} = (\iota, \mathbf{Z}^{(N)}) \otimes (\iota, \mathbf{d}_{J} - d)$, where $\iota$ is the unit vector whose $N$ elements equal to 1 and $\mathbf{d}_{J} - d = \begin{pmatrix}
d_1 - d \\
d_2 - d \\
\vdots  \\
d_{J} - d
\end{pmatrix}.$ $\otimes$ is the Kronecker product.
Applying Taylor expansion to $\E\mu$, we have
$$
\E\mu = (\iota, \mathbf{Z}^{(N)}) \otimes (\iota, (\mathbf{d}_{J} - d), \dots, (\mathbf{d}_{J} - d)^P) \begin{pmatrix}
\beta_1(d) \\
\beta_2(d) \\
\vdots  \\
\beta_{2(P+1)}(d)/(P!)
\end{pmatrix} + \mathbf{R}_{P+1}(d),
$$
where $\mathbf{R}_{P+1}(d)$ is the remainder whose order is higher than $P+1$. Hence, the estimation bias is
$$
\begin{aligned}
\hat \beta(d) - \beta(d)  = & \mathbf{P}(d) (\iota, \mathbf{Z}^{(N)}) \otimes ((\mathbf{d}_{J} - d)^2, \dots, (\mathbf{d}_{J} - d)^p) \begin{pmatrix}
\beta_5(d)/(2!) \\
\vdots  \\
\beta_{2(p+1)}(d)/(P!)
\end{pmatrix} \\
& + \mathbf{P}(d)\mathbf{R}_{p+1}(d) + \mathbf{P}(d)\varepsilon.
\end{aligned}
$$ The expectation of $\hat \beta(d) - \beta(d)$ is the asymptotic bias of $\hat \beta(d)$. As we are interested in $\hat \tau_K(d)$, the second row of $\hat \beta(d)$, we denote the second row of the expectation as $B$.  From standard theories on nonparametric regression (e.g. \citet{li2007nonparametric}), we know that $B = O(h^2)$.

%Because of the independence between $\kappa$ and $\mu$, we know that
%If we ignore the bias part, the variance of the estimates is decided by the last term, thus
%$$
%\hat \tau_{PATE}(d) - \tau_{PATE}(d)  = \sum_{i=1}^N \sum_{d' \in \tilde{D}} \kappa_i(d';d) \nu_{i}(d') + Bias,
%$$
%$$
%\begin{pmatrix}
%\hat \theta(d) \\
%\hat \tau(d)
%\end{pmatrix} - \begin{pmatrix}
%\theta_0(d) \\
%\tau_{PATE}(d)
%\end{pmatrix}  = \sum_{i=1}^N \sum_{d' \in \tilde{D}} \omega_i(d') \nu_{i}(d') + Bias,
%$$
%where 
%$$
%\begin{aligned}
%Bias  & = \sum_{i=1}^N \sum_{d' \in \tilde{D}}\kappa_i(d';d) (\theta_0(d) +\tau_{PATE}(d) Z_i ) - \tau_{PATE}(d) \\
%& \rightarrow \sum_{i=1}^N \sum_{d' \in \tilde{D}}\E\left[\kappa_i(d';d) (\theta_0(d) +\tau_{PATE}(d) Z_i ) \right]- \tau_{PATE}(d).
%\end{aligned}
%$$
%And
%$$
%\begin{aligned}
%\Var\left( \hat \tau_{PATE}(d)\right) = & \Var\left(\sum_{i=1}^N \sum_{d' \in \tilde{D}} \kappa_i(d';d) \mu(d')\right) \\
%= & \sum_{i=1}^N \sum_{d' \in \tilde{D}} \Var\left(\kappa_i(d';d)\right) \Var\left(\mu(d')\right) \\
%& + \sum_{d' \in \tilde{D}}\sum_{i=1}^N \sum_{d^{''} \in \tilde{D}}\sum_{j \in  \mathcal{B}(i;d')}  \Var\left(\kappa_i(d^{'};d)\right) \Var\left(\kappa_i(d^{''};d)\right)\Cov\left( \mu(d'), \mu(d^{''})\right).
%\end{aligned}
%$$
%In practice, we estimate $\Var\left( \hat \tau_{PATE}(d)\right)$ using the plug-in estimator. We have shown that the estimate is asymptotically unbiased and consistent for the Horvitz-Thompson estimator and the Hajek estimator. For the kernel regression estimator, let's denote $(\mathbf{e}, \mathbf{Z}^{(N)}) \otimes ((\mathbf{d}_{J} - d)^2, \dots, (\mathbf{d}_{J} - d)^p) \begin{pmatrix}
%\beta_5(d) \\
%\vdots  \\
%\beta_{2(p+1)}(d)
%\end{pmatrix} + \mathbf{R}_{p+1}(d) + \nu$ as $\tilde{\mathbf{R}}(d)$. Then, it is straightforward to derive the expression of the residuals from the kernel regression estimator:
%$$
%\hat{\mathbf{e}}(d) = \left(\mathbf{I} - \mathbf{X}^{\dagger '}(d)\mathbf{P}(d)\right)\tilde{\mathbf{R}}(d).
%$$
The variance-covariance matrix of the regression coefficients equals to 
$$
\begin{aligned}
& \Var\left(\hat \beta(d)\right) \\
& = \left(\mathbf{X}^{\dagger '}(d)\mathbf{W}^{K}_h(d)\mathbf{X}^{\dagger}(d) \right)^{-1}\left(\mathbf{X}^{\dagger '}(d)\mathbf{W}^{K}(d)\Omega \mathbf{W}^{K}_h(d)\mathbf{X}^{\dagger '}(d) \right)\left(\mathbf{X}^{\dagger '}(d)\mathbf{W}^{K}_h(d)\mathbf{X}^{\dagger}(d) \right)^{-1},
\end{aligned}
$$
where $\Omega$ is the variance-covariance matrix of the residuals. We are interested in the $(2, 2)$th entry of $\Var\left(\hat \beta(d)\right)$ which we denote as $V$. $V = O\left(\frac{1}{NJh}\right)$ under the assumption of local interference. We estimate the variance using a plug-in estimator: 
$$
\begin{aligned}
&\widehat{\Var}\left(\hat \beta(d)\right) \\
& = \left(\mathbf{X}^{\dagger '}(d)\mathbf{W}^{K}_h(d)\mathbf{X}^{\dagger}(d) \right)^{-1}\left(\mathbf{X}^{\dagger '}(d)\mathbf{W}^{K}(d)\hat{\Omega}(d) \mathbf{W}^{K}_h(d)\mathbf{X}^{\dagger '}(d) \right)\left(\mathbf{X}^{\dagger '}(d)\mathbf{W}^{K}_h(d)\mathbf{X}^{\dagger}(d) \right)^{-1},
\end{aligned}
$$
where $\hat{\Omega}(d) = \hat{\mathbf{e}}(d)\hat{\mathbf{e}}(d)^{'} \odot \mathcal{D}$ is a $(N * J)\times (N * J)$ matrix and $\hat{\mathbf{e}}(d)$ is the residuals from the kernel regression. The element at $(i*J+d^{'}, j*J+d^{''})$ in $\mathcal{D}$ equals to $1$ if $j \in \mathcal{B}(i; d')$ in  and $0$ otherwise. $\odot$ represents element-wise multiplication of matrices. As $N$ grows to infinity, the bandwidth $h \rightarrow 0$ and $\widehat{\Var}\left(\hat \beta(d)\right)$ converges to the variance estimate for the Hajek estimator. Hence, $\widehat{\Var}\left(\hat \beta(d)\right)$ is asymptotically unbiased and consistent for $\Var\left(\hat \beta(d)\right)$. We take the second element on the variance-covariance matrix's diagonal as the estimate of $\Var\left( \hat \tau_{K}(d)\right)$.

%\section*{Bias correction for the kernel regression estimator}
We apply bias correction developed in \citet{calonico2014robust} to the kernel regression estimator for more precise estimates. Denote 
$$
\mathbf{X}^{\ddagger}(d) = \begin{pmatrix}
1 & Z_1 & (d_1 - d) &  Z_1 * (d_1 - d)  & (d_1 - d)^2 &  Z_1 * (d_1 - d)^2 \\
\vdots & \vdots & \vdots &  \vdots & \vdots &  \vdots \\
1 & Z_N & (d_1 - d) &  Z_N * (d_1 - d) & (d_1 - d)^2  &  Z_N * (d_1 - d)^2 \\
1 & Z_1 & (d_2 - d) &  Z_1 * (d_2 - d)  & (d_2 - d)^2 &  Z_1 * (d_2 - d)^2 \\
\vdots & \vdots & \vdots &  \vdots \\
1 & Z_N & (d_{J} - d) &  Z_N * (d_{J} - d) & (d_{J} - d)^2 &  Z_N * (d_{J} - d)^2
\end{pmatrix}  
$$
and 
$$
\mathbf{X}^{\ddagger}_{,(5:6)}(d) = \begin{pmatrix}
 (d_1 - d)^2 &  Z_1 * (d_1 - d)^2 \\
 \vdots &  \vdots \\
 (d_1 - d)^2  &  Z_N * (d_1 - d)^2 \\
 (d_2 - d)^2 &  Z_1 * (d_2 - d)^2 \\
\vdots &  \vdots \\
 (d_{J} - d)^2 &  Z_N * (d_{J} - d)^2
\end{pmatrix}  
$$
Estimates from the kernel regression estimator with $\mathbf{X}^{\ddagger}(d)$ as the regressors are
$$
\hat \beta^{\ddagger}(d) = \left(\mathbf{X}^{\ddagger '}(d)\mathbf{W}^{K}_b(d)\mathbf{X}^{\ddagger}(d) \right)^{-1}\left(\mathbf{X}^{\ddagger '}(d)\mathbf{W}^{K}_b(d)\mu \right),
$$
where $h$ is the optimal bandwidth for this bias-correction regression.
Then, the bias-corrected estimator is
$$
\hat \beta^{bc}(d) = \hat \beta(d) - \frac{1}{2} \left(\mathbf{X}^{\dagger '}(d)\mathbf{W}^{K}_h(d)\mathbf{X}^{\dagger}(d) \right)^{-1}\left(\mathbf{X}^{\dagger '}(d)\mathbf{W}^{K}_h(d)\mathbf{X}^{\ddagger}_{,(5:6)}(d)\right)\hat \beta^{\ddagger}_{(5:6)}(d). 
$$
Note that 
\begin{align*}
\hat \beta^{bc}(d) = & \left(\mathbf{X}^{\dagger '}(d)\mathbf{W}^{K}_h(d)\mathbf{X}^{\dagger}(d) \right)^{-1}\left(\mathbf{X}^{\dagger '}(d)\mathbf{W}^{K}_h(d)\mu \right) \\
& - \frac{1}{2} \left(\mathbf{X}^{\dagger '}(d)\mathbf{W}^{K}_h(d)\mathbf{X}^{\dagger}(d) \right)^{-1}\left(\mathbf{X}^{\dagger '}(d)\mathbf{W}^{K}_h(d)\mathbf{X}^{\ddagger}_{,(5:6)}(d)\right)\\ 
& \begin{pmatrix}
\nu_{5}^{'} \\
\nu_{6}^{'}
\end{pmatrix} \left(\mathbf{X}^{\ddagger '}(d)\mathbf{W}^{K}_b(d)\mathbf{X}^{\ddagger}(d) \right)^{-1}\left(\mathbf{X}^{\ddagger '}(d)\mathbf{W}^{K}_b(d)\mu \right) \\
= & \left(\mathbf{X}^{\dagger '}(d)\mathbf{W}^{K}_h(d)\mathbf{X}^{\dagger}(d) \right)^{-1}\Lambda \mu,
\end{align*}
where $\Lambda = \mathbf{X}^{\dagger '}(d)\mathbf{W}^{K}_h(d) - \frac{1}{2}\left(\mathbf{X}^{\dagger '}(d)\mathbf{W}^{K}_h(d)\mathbf{X}^{\ddagger}_{,(5:6)}(d)\right)\begin{pmatrix}
\nu_{5}^{'} \\
\nu_{6}^{'}
\end{pmatrix} \left(\mathbf{X}^{\ddagger '}(d)\mathbf{W}^{K}_b(d)\mathbf{X}^{\ddagger}(d) \right)^{-1}\mathbf{X}^{\ddagger '}(d)\mathbf{W}^{K}_b(d)$, $\nu_{p}$ is a 6-dimensional vector whose $p$-th entry equals to 1 and other entries equal to 0. It is easy to see that 
$$
\widehat{\Var}\left(\hat \beta^{bc}(d)\right) = \left(\mathbf{X}^{\dagger '}(d)\mathbf{W}^{K}_h(d)\mathbf{X}^{\dagger}(d) \right)^{-1}\left(\Lambda\hat{\Omega}(d) \Lambda^{'} \right)\left(\mathbf{X}^{\dagger '}(d)\mathbf{W}^{K}_h(d)\mathbf{X}^{\dagger}(d) \right)^{-1},
$$
where $\hat{\Omega}(d)$ is similarly defined, with residuals from the bias-correction regression. We can show that with bias correction or not, the estimate $\hat \tau_K(d)$ is asymptotically normal, since the kernel regression estimator is linear and the residuals satisfy conditions required by lemma \ref{lemma:ogburn-2020-1}.

%\section*{Confidence band}
%We consider the confidence band for both the nonparametric estimators and the kernel regression estimator, following the approach discussed in \citet{wasserman2006-nonparametric}. For any estimator $\hat \tau_{PATE}(d)$ that is linear in the outcome $\mu(d)$, \citet{wasserman2006-nonparametric} shows that the confidence band takes the form of
%\begin{align*}
%I(d) = \left(\hat \tau_{PATE}(d) - c\hat \sigma_{PATE}(d), \hat \tau_{PATE}(d) + c\hat \sigma_{PATE}(d) \right),
%\end{align*}
%where $\hat \sigma_{PATE}(d)  = \sqrt{\widehat \Var\left( \hat \tau_{PATE}(d)\right) }$. Now, 
%$$
%P(\tau_{PATE}(d) \notin I(d) \text{ for some } d) = P\left(\max_{d} \Big|\frac{\hat \tau_{PATE}(d) - \tau_{PATE}(d)}{\hat \sigma_{PATE}(d)}\Big| > c\right).
%$$
%Suppose we know that $\tilde{\tau}(d) = \Big|\frac{\hat \tau_{PATE}(d) - \tau_{PATE}(d)}{\hat \sigma_{PATE}(d)}\Big|$ converges to the Gaussian distribution uniformly for a sequence of $d$, then $\max_{d}|\tilde{\tau}(d)|$ obeys the Gumbel distribution according to \citet{berman1964limit} and $c$ satisfies
%\begin{align*}
%2(1 - \Phi(c)) + \frac{\kappa_0}{\pi}e^{-\frac{c^2}{2}} = \alpha
%\end{align*}
%for size $\alpha$ and $\kappa_0 = \int_{\tilde{D}}\left\Vert \partial\left( \frac{\kappa(d)}{\Vert \kappa(d) \Vert} \right)/\partial d \right\Vert \mathtt{d}d$. In the case of kernel regression, \citet{wasserman2006-nonparametric} suggests that we can approximate  $\kappa_0$ with
%$$
%\frac{d_{\max}-d_{\min}}{h}\frac{\Vert K' \Vert}{\Vert K \Vert},
%$$ 
%where $K$ is the selected kernel; $\Vert K \Vert^2 = \int_{\tilde{D}}K^2(d) \mathtt{d}d$; $d_{\max}$ and $d_{\min}$ correspond to the largest and smallest value in $\tilde{D}$. As we are using the Gaussian kernel in regression, the critical value equals to $3.191$.
%
%%\begin{align*}
%%& P\left[\tau(d) \in I_c = [\hat \tau(d) - c\hat \sigma(d), \hat \tau(d) + c\hat \sigma(d)] \right] \\
%%= & P\left[\max_{d \in [0, \bar d]}\Big|\frac{\hat \tau(d) - \tau(d)}{\hat \sigma(d)}\Big| \leq c \right]  \geq 1-\alpha.
%%\end{align*}
%%Consider the Hajek estimator $\hat \tau_{HA}(d)$. We know that $\frac{\hat \tau_{HA}(d) - \tau_{HA}(d)}{\hat \sigma_{HA}(d)} \sim N(0, 1)$ in the limit. Therefore, we only need to bound the tail of a Gaussian process.
%%
%%Note that the Hajek estimator is an extreme case of nonparametric estimators where we impose no restriction on smoothness thus the estimate is unbiased but potentially has a large variance.
%\section*{Bias and variance of the kernel regression estimator}
%To see that $B = O(h^2)$, let's define $\xi_j = \frac{d_j - d}{h}$, 
%$$
%\tilde{\mathbf{X}}^{\dagger}(d) = \begin{pmatrix}
%1 & Z_1 & \frac{(d_1 - d)}{h} &  Z_1 * \frac{(d_1 - d)}{h}\\
%\vdots & \vdots & \vdots &  \vdots \\
%1 & Z_N & \frac{(d_1 - d)}{h} &  Z_N * \frac{(d_1 - d)}{h} \\
%1 & Z_1 & \frac{(d_2 - d)}{h} &  Z_1 * \frac{(d_2 - d)}{h} \\
%\vdots & \vdots & \vdots &  \vdots \\
%1 & Z_N & \frac{(d_J - d)}{h} &  Z_N * \frac{(d_J - d)}{h}
%\end{pmatrix}  
%$$
%and
%$$
%\tilde{\mathbf{W}}^{K}_h(d) = \begin{pmatrix}
%\frac{1}{h}K\left(\frac{(d_1 - d)}{h}\right) &  &  &  & \\
%&  \ddots & & & \\
% &  & \frac{1}{h}K\left(\frac{(d_1 - d)}{h}\right) & &  \\
% &  & & \ddots &  \\
%&  & & & \frac{1}{h}K\left(\frac{(d_J - d)}{h}\right)
%\end{pmatrix}.
%$$
%Then,
%$$
%\tiny
%\begin{aligned}
%& \frac{\tilde{\mathbf{X}}^{\dagger}(d)' \tilde{\mathbf{W}}^{K}_h(d) \tilde{\mathbf{X}}^{\dagger}(d)}{NJ} = \\
%& \begin{pmatrix}
%\frac{1}{Jh}\sum_{j=1}^J K\left(\xi_j\right) & \frac{1}{NJh}\sum_{j=1}^J K\left(\xi_j\right) \sum_{i=1}^N Z_i & \frac{1}{Jh}\sum_{j=1}^J K\left(\xi_j\right) \xi_j  & \frac{1}{NJh}\sum_{j=1}^J K\left(\xi_j\right) \xi_j \sum_{i=1}^N Z_i   \\
%\frac{1}{NJh}\sum_{j=1}^J K\left(\xi_j\right) \sum_{i=1}^N Z_i & \frac{1}{NJh}\sum_{j=1}^J K\left(\xi_j\right) \sum_{i=1}^N Z_i & \frac{1}{NJh}\sum_{j=1}^J K\left(\xi_j\right) \xi_j \sum_{i=1}^N Z_i  & \frac{1}{NJh}\sum_{j=1}^J K\left(\xi_j\right) \xi_j \sum_{i=1}^N Z_i   \\
% \frac{1}{Jh}\sum_{j=1}^J K\left(\xi_j\right) \xi_j  & \frac{1}{NJh}\sum_{j=1}^J K\left(\xi_j\right) \xi_j \sum_{i=1}^N Z_i  & \frac{1}{Jh}\sum_{j=1}^J K\left(\xi_j\right) \xi_j^2 &  \frac{1}{NJh}\sum_{j=1}^J K\left(\xi_j\right) \xi_j^2 \sum_{i=1}^N Z_i \\
% \frac{1}{NJh}\sum_{j=1}^J K\left(\xi_j\right) \xi_j \sum_{i=1}^N Z_i & \frac{1}{NJh}\sum_{j=1}^J K\left(\xi_j\right) \xi_j^2 \sum_{i=1}^N Z_i & \frac{1}{NJh}\sum_{j=1}^J K\left(\xi_j\right) \xi_j^2 \sum_{i=1}^N Z_i &  \frac{1}{NJh}\sum_{j=1}^J K\left(\xi_j\right) \xi_j^2 \sum_{i=1}^N Z_i
%\end{pmatrix}.
%\end{aligned}
%$$
%We can show that $\frac{\tilde{\mathbf{X}}^{\dagger}(d)' \tilde{\mathbf{W}}^{K}_h(d) \tilde{\mathbf{X}}^{\dagger}(d)}{NJ}$ converges to 
%$$
%\tiny
%\begin{aligned} 
%\begin{pmatrix}
%\int_{0}^{\infty}K(\xi)f(\xi h + d)d\xi & p\int_{0}^{\infty}K(\xi)f(\xi h + d)d\xi & \int_{0}^{\infty}K(\xi)\xi f(\xi h + d)d\xi  & p\int_{0}^{\infty}K(\xi)\xi f(\xi h + d)d\xi    \\
%p\int_{0}^{\infty}K(\xi)f(\xi h + d)d\xi & p\int_{0}^{\infty}K(\xi)f(\xi h + d)d\xi & p\int_{0}^{\infty}K(\xi)\xi f(\xi h + d)d\xi  & p\int_{0}^{\infty}K(\xi)\xi f(\xi h + d)d\xi   \\
% \int_{0}^{\infty}K(\xi)\xi f(\xi h + d)d\xi & p\int_{0}^{\infty}K(\xi)\xi f(\xi h + d)d\xi  & \int_{0}^{\infty}K(\xi)\xi^2 f(\xi h + d)d\xi  &  p\int_{0}^{\infty}K(\xi)\xi^2 f(\xi h + d)d\xi \\
% p\int_{0}^{\infty}K(\xi)\xi f(\xi h + d)d\xi  & \frac{1}{NJh}p\int_{0}^{\infty}K(\xi)\xi^2 f(\xi h + d)d\xi &  \frac{1}{NJh}p\int_{0}^{\infty}K(\xi)\xi^2 f(\xi h + d)d\xi & p\int_{0}^{\infty}K(\xi)\xi^2 f(\xi h + d)d\xi
%\end{pmatrix},
%\end{aligned}
%$$
%which is a matrix with the order of $O(1)$. Hence, $\frac{\tilde{\mathbf{X}}^{\dagger}(d)' \tilde{\mathbf{W}}^{K}_h(d) \tilde{\mathbf{X}}^{\dagger}(d)}{NJ} = O_P(1)$.
%Similarly, if we define 
%$$
%\tilde{\mathbf{X}}^{\ddagger}_{,(5:6)}(d) = \begin{pmatrix}
% \left(\frac{d_1 - d}{h}\right)^2 &  Z_1 * \left(\frac{d_1 - d}{h}\right)^2 \\
% \vdots &  \vdots \\
% \left(\frac{d_1 - d}{h}\right)^2  &  Z_N * \left(\frac{d_1 - d}{h}\right)^2 \\
% \left(\frac{d_2 - d}{h}\right)^2 &  Z_1 * \left(\frac{d_2 - d}{h}\right)^2 \\
%\vdots &  \vdots \\
% \left(\frac{d_J - d}{h}\right)^2 &  Z_N * \left(\frac{d_J - d}{h}\right)^2
%\end{pmatrix}  
%$$
%we can show that $\frac{\tilde{\mathbf{X}}^{\dagger}(d)' \tilde{\mathbf{W}}^{K}_h(d) \tilde{\mathbf{X}}^{\ddagger}_{,(5:6)}(d)}{NJ}$ converges to another matrix with the order of $O(1)$:
%$$
%\begin{pmatrix}
% \int_{0}^{\infty}K(\xi)\xi^2 f(\xi h + d)d\xi &  p\int_{0}^{\infty}K(\xi)\xi^2 f(\xi h + d)d\xi \\
% p\int_{0}^{\infty}K(\xi)\xi^2 f(\xi h + d)d\xi  &  p\int_{0}^{\infty}K(\xi)\xi^2 f(\xi h + d)d\xi \\
% \int_{0}^{\infty}K(\xi)\xi^3 f(\xi h + d)d\xi &  p\int_{0}^{\infty}K(\xi)\xi^3 f(\xi h + d)d\xi\\
% p\int_{0}^{\infty}K(\xi)\xi^3 f(\xi h + d)d\xi &  p\int_{0}^{\infty}K(\xi)\xi^3 f(\xi h + d)d\xi
%\end{pmatrix}.
%$$
%Hence, $\frac{\tilde{\mathbf{X}}^{\dagger}(d)' \tilde{\mathbf{W}}^{K}_h(d) \tilde{\mathbf{X}}^{\ddagger}_{,(5:6)}(d)}{NJ} = O_P(1)$.
% In addition, we can see that
%$$
%\begin{aligned} 
%& \hat \beta(d) = \begin{pmatrix}
% 1 &  &  & \\
%  & 1 &  & \\
%  &  & \frac{1}{h}  & \\
%  &  &  & \frac{1}{h} \\
%\end{pmatrix}   \left(\frac{\tilde{\mathbf{X}}^{\dagger}(d)' \tilde{\mathbf{W}}^{K}_h(d) \tilde{\mathbf{X}}^{\dagger}(d) }{NJ}\right)^{-1}\frac{\tilde{\mathbf{X}}^{\dagger}(d)' \tilde{\mathbf{W}}^{K}_h(d) \mu}{NJ}
%\end{aligned} 
%$$
%$$
%\begin{aligned} 
%\hat \beta(d) - \beta(d) = & h^2\begin{pmatrix}
% 1 &  &  & \\
%  & 1 &  & \\
%  &  & \frac{1}{h}  & \\
%  &  &  & \frac{1}{h} \\
%\end{pmatrix}\left(\frac{\tilde{\mathbf{X}}^{\dagger}(d)' \tilde{\mathbf{W}}^{K}_h(d) \tilde{\mathbf{X}}^{\dagger}(d) }{NJ}\right)^{-1}\frac{\tilde{\mathbf{X}}^{\dagger}(d)' \tilde{\mathbf{W}}^{K}_h(d) \tilde{\mathbf{X}}^{\ddagger}_{,(5:6)}(d)}{NJ} + \mathbf{R}_2(d) \\
%= & O_P(h^2)
%\end{aligned} 
%$$
%Hence, $B$ as the second row of $\E[\hat \beta(d) - \beta(d)]$ has the order of $O(h^2)$.
%
%Next, for variance, let's denote $(N(j-1)+i, N(j'-1)+i')$th entry of $\Omega$ as $\sigma^2_{(N(j-1)+i, N(j'-1)+i')}$. We know that $\sigma^2_{(N(j-1)+i, N(j'-1)+i')} = 0$ if $|d_j - d_{j'}| > \bar d$ or node $i' \notin \mathcal{B}(i)$. Then, $\frac{h\tilde{\mathbf{X}}^{\dagger}(d)' \tilde{\mathbf{W}}^{K}_h(d) \Omega \tilde{\mathbf{W}}^{K}_h(d) \tilde{\mathbf{X}}^{\dagger}(d)}{NJ}$ converges to a matrix with the order $O(1)$. For example, the $(1, 1)$th entry of $\frac{h\tilde{\mathbf{X}}^{\dagger}(d)' \tilde{\mathbf{W}}^{K}_h(d) \Omega \tilde{\mathbf{W}}^{K}_h(d) \tilde{\mathbf{X}}^{\dagger}(d)}{NJ}$ equals to
%$$
%\frac{1}{NJh}\sum_{i=1}^N \sum_{j=1}^J \sigma^2_{(N(j-1)+i, N(j-1)+i)}K\left(\xi_j\right) + \frac{1}{NJh}\sum_{i=1}^N \sum_{j=1}^J \sum_{i' \in \mathcal{B}(i)}\sum_{j': |d_j - d_{j'}| \leq \bar d} \sigma^2_{(N(j-1)+i, N(j'-1)+i')}K\left(\xi_j\right),
%$$
%which converges to
%$$
%\begin{aligned}
%& \frac{1}{NJ}\sum_{i=1}^N \sum_{j=1}^J \sigma^2_{(N(j-1)+i, N(j-1)+i)}\int_{0}^{\infty}K^2(\xi) f(\xi h + d)d\xi \\
%+ & \frac{1}{NJ}\sum_{i=1}^N \sum_{j=1}^J \sum_{i' \in \mathcal{B}(i)}\sum_{j': |d_j - d_{j'}| \leq \bar d} \sigma^2_{(N(j-1)+i, N(j'-1)+i')}\int_{0}^{\infty}K^2(\xi) f(\xi h + d)d\xi.
%\end{aligned}
%$$
%Since every term in the summation is bounded, the total expression has an order of $O(1)$.
%
%%$$
%%\tiny
%%\begin{aligned}
%%& \frac{\tilde{\mathbf{X}}^{\dagger}(d)' \tilde{\mathbf{W}}^{K}_h(d) \Omega \tilde{\mathbf{W}}^{K}_h(d) \tilde{\mathbf{X}}^{\dagger}(d)}{NJ} = \\
%%& \begin{pmatrix}
%%\frac{1}{NJh^2}\sum_{i=1}^N \sum_{j=1}^J \sigma^2_{(N(j-1)+i, N(j-1)+i)}K\left(\xi_j\right) & \frac{1}{NJh}\sum_{j=1}^J K\left(\xi_j\right) \sum_{i=1}^N Z_i & \frac{1}{Jh}\sum_{j=1}^J K\left(\xi_j\right) \xi_j  & \frac{1}{NJh}\sum_{j=1}^J K\left(\xi_j\right) \xi_j \sum_{i=1}^N Z_i   \\
%%\frac{1}{NJh}\sum_{j=1}^J K\left(\xi_j\right) \sum_{i=1}^N Z_i & \frac{1}{NJh}\sum_{j=1}^J K\left(\xi_j\right) \sum_{i=1}^N Z_i & \frac{1}{NJh}\sum_{j=1}^J K\left(\xi_j\right) \xi_j \sum_{i=1}^N Z_i  & \frac{1}{NJh}\sum_{j=1}^J K\left(\xi_j\right) \xi_j \sum_{i=1}^N Z_i   \\
%% \frac{1}{Jh}\sum_{j=1}^J K\left(\xi_j\right) \xi_j  & \frac{1}{NJh}\sum_{j=1}^J K\left(\xi_j\right) \xi_j \sum_{i=1}^N Z_i  & \frac{1}{Jh}\sum_{j=1}^J K\left(\xi_j\right) \xi_j^2 &  \frac{1}{NJh}\sum_{j=1}^J K\left(\xi_j\right) \xi_j^2 \sum_{i=1}^N Z_i \\
%% \frac{1}{NJh}\sum_{j=1}^J K\left(\xi_j\right) \xi_j \sum_{i=1}^N Z_i & \frac{1}{NJh}\sum_{j=1}^J K\left(\xi_j\right) \xi_j^2 \sum_{i=1}^N Z_i & \frac{1}{NJh}\sum_{j=1}^J K\left(\xi_j\right) \xi_j^2 \sum_{i=1}^N Z_i &  \frac{1}{NJh}\sum_{j=1}^J K\left(\xi_j\right) \xi_j^2 \sum_{i=1}^N Z_i
%%\end{pmatrix}.
%%\end{aligned}
%%$$
%Note that 
%$$
%\begin{aligned}
%& \Var\left(\hat \beta(d)\right) \\
%& = \frac{1}{NJh} \left(\frac{\tilde{\mathbf{X}}^{\dagger}(d)' \tilde{\mathbf{W}}^{K}_h(d) \tilde{\mathbf{X}}^{\dagger}(d)}{NJ} \right)^{-1}\left(\frac{h\tilde{\mathbf{X}}^{\dagger}(d)' \tilde{\mathbf{W}}^{K}_h(d) \Omega \tilde{\mathbf{W}}^{K}_h(d) \tilde{\mathbf{X}}^{\dagger}(d)}{NJ} \right)\left(\frac{\tilde{\mathbf{X}}^{\dagger}(d)' \tilde{\mathbf{W}}^{K}_h(d) \tilde{\mathbf{X}}^{\dagger}(d)}{NJ}\right)^{-1}.
%\end{aligned}
%$$
%Therefore, $V = O_P\left(\frac{1}{NJh}\right)$.

%\bibliography{../all}
%\end{document}




==> proofs/uniform_convergence.tex <==
%\input{tex-header}
%\begin{document}
%\section*{Joint convergence to a multivariate Gaussian distribution}
Next, we rely on a result developed in \citet{raivc2004multivariate} to prove the joint convergence of our estimates from the Horvitz-Thompson estimator, $\{\hat \tau(d)\}_{d=d_1,d_2,\dots,d_J}$, to a multivariate Gaussian distribution. We first restate the result in \citet{raivc2004multivariate} using terms under our framework. We use $\mathbf{I}_J$ to denote the $J$-dimensional diagonal matrix and $\mathbf{Z}$ a $J$-dimensional random vector drawn from $\mathcal{N}(0, \mathbf{I}_J)$. We then define $M_2(f) = \sup_{\mathbf{x} \neq \mathbf{y}} \frac{|f'(\mathbf{x}) - f'(\mathbf{y})|}{|\mathbf{x} - \mathbf{y}|}$, where $|\cdot|$ represents the Euclidean norm of a vector. The result is as follows:
\begin{lemma}(Rai\v{c} (2004), Theorem 3) Consider a set of $N$ units. Let $\mathbf{X}_1, \dots, \mathbf{X}_N$ be $\mathbb{R}^J$-valued random vectors. Suppose $\E [\mathbf{X}_i] = 0$ and $\mathbf{W} \equiv \sum_{i=1}^N \mathbf{X}_i$ is $L^2$-convergent with $\Var[\mathbf{W}] = \mathbf{I}_J$. If $c_i(d) \leq \tilde{c}$ for all $i$, then for every differentiable function $f : \mathbb{R}^m \rightarrow \mathbb{R}$, we have
$$
|\E[f(\mathbf{W}) - f(\mathbf{Z})] | \leq \frac{53}{23} M_2(f)(1 + \tilde{c})\sum_{i=1}^N \E\left[|\mathbf{X}_i|^2 \min\Bigg\{1, \frac{\sqrt{2\pi}}{2}(1 + \tilde{c}) |\mathbf{X}_i|\Bigg\}\right ]
$$
\end{lemma}

Let's define $X_i(d) = \hat{\tau}_i(d) - \tau_i(d)$, where $\hat{\tau}_i(d) = \frac{Z_i\mu(\mathbf{Y}(\mathbf{Z}); d)}{p} - \frac{(1-Z_i)\mu(\mathbf{Y}(\mathbf{Z}); d)}{1-p}$.
We further define $\mathbf{X}_i = (\mathbf{X}_i(d_1), \mathbf{X}_i(d_2), \dots, \mathbf{X}_i(d_J))'$, $\mathbf{W} = \frac{1}{\sqrt N} \sum_{i=1}^N \mathbf{X}_i$, $\tilde{\mathbf{X}}_i = \frac{1}{\sqrt N}\left(\Var[\mathbf{W}]\right)^{-\frac{1}{2}} \mathbf{X}_i$, and $\tilde{\mathbf{W}} = \sum_{i=1}^N \tilde{\mathbf{X}}_i$, where $\left(\Var[\mathbf{W}]\right)^{-\frac{1}{2}} \left(\Var[\mathbf{W}]\right)^{-\frac{1}{2}} = \left(\Var[\mathbf{W}]\right)^{-1}$. Note that $\E [\tilde{\mathbf{X}}_i] = 0$,  $\Var[\mathbf{W}] = O(1)$, and $\Var[\tilde{\mathbf{W}}] = \mathbf{I}_J$. Hence, $\tilde{\mathbf{X}}_i$ and $\tilde{\mathbf{W}}$ satisfy the requirements in Lemma.  Hence, the distance between $\tilde{\mathbf{W}}$ and $\mathbf{Z}$ is bounded by $C (1 + \tilde{c})^2 N^{-\frac{1}{2}} \frac{1}{N} \sum_{i=1}^N \E\left[|\mathbf{X}_i|^3 \right ]$. As long as $\frac{1 + \tilde{c}}{N^{\frac{1}{4}}} = o_P(1)$, $\tilde{\mathbf{W}}$ will be converging to $\mathbf{Z}$ as $N \rightarrow \infty$. This condition is clearly satisfied under our framework.


%\section*{Using bootstrap to approximate the maximum of estimates}
%We rely on the method of Gaussian bootstrap developed by \citet{chernozhukov2013gaussian} to calculate the quantiles of the maximum of our estimates and construct confidence bands. We have seen that $\mathbf{W} = \frac{1}{\sqrt N} \sum_{i=1}^N \mathbf{X}_i \rightarrow \mathcal{N}(0, \Var[\mathbf{W}])$. To approximate the distribution of $T = \max_{d \in \{d_1,d_2,\dots,d_J\}}\frac{1}{\sqrt N} \sum_{i=1}^N \mathbf{X}_i$, we construct bootstrapped statistics
%$$
%\tilde T = \max_{d \in \{d_1,d_2,\dots,d_J\}}\frac{1}{\sqrt N} \sum_{i=1}^N \mathbf{X}_i e_i,
%$$
%where $e_i \sim \mathcal{N}(0, 1)$.
% 
%\citet{chernozhukov2013gaussian} prove that quantiles of $\tilde T$ converge to the quantiles of $T$. Suppose we want to test the null hypothesis that 

%\section*{Construct the confidence bands}
%We follow an approach adapted from the one in \citet{lee2017doubly} to construct confidence bands. 
%\section*{Gaussian approximation of the estimates' suprema}
%For any given $d$, each of our estimators (Horvitz-Thompson, Hajek, and smoothed) could be seen as a random function from the sampling space to $\mathcal{R}$. Hence, as the values of $d$ vary, it forms an empirical process indexed by $d$:
%$$
%\begin{aligned}
%\mathbb{G}_d & = \sqrt{N} \left( \hat{\tau}_d - \tau_d \right)  \\
%& = \frac{1}{\sqrt N} \sum_{i=1}^{N} \left[f_d(\mathbf{W}_i) - \tau_d \right],
%\end{aligned}
%$$
%where $\mathbf{W}_i = (Z_i, \mu_i(\mathbf{Y};d))$ the form of $f_d$ is decided by each estimator. For the Horvitz-Thompson estimator, for instance, $f_d(\mathbf{W}_i) = \frac{Z_i\mu_i(\mathbf{Y};d)}{P(Z_i = 1)}$
%
%We want to show that under assumptions in the paper, such an empirical process can be approximated by a Gaussian process. We first prove that for any discrete set $\tilde D = \{d_1, d_2, \dots, d_J\}$, 

%\bibliography{../all}
%\end{document}




==> proofs/variance_expression-for-paper.tex <==
%\input{tex-header}
%\begin{document}
\noindent We now characterize the variance of the Horvitz-Thompson estimator. 
\begin{lemma}\label{lemma:ht-var}
Under conditions C\ref{assn:bern-des}-C\ref{assn:local-inf} as defined in the main text, the variance of estimator $\widehat{\tau}(d)$ is bounded as follows:
\begin{align*}
& \Var\left(\widehat{\tau}(d) \right) \\
\leq & \frac{1}{N^2p} \sum_{i=1}^N \E\left[\muit^2\right] + \frac{1}{N^2(1-p)} \sum_{i=1}^N \E\left[ \muic^2 \right] \\
& + \frac{1}{N^2}\sumij\sum_{a=0}^1\sum_{b=0}^1 (-1)^{a+b}\Big\{ \E\left[\muiab\mujab  \right] - \E\left[\muia\right] \E\left[\mujb\right]\Big\},
\end{align*}
and, in addition under C\ref{assn:spacing}, we have that
\begin{align*}
 \Var\left(\widehat{\tau}(d) \right) = O\left(\frac{1}{N}\right).
\end{align*}
\end{lemma}


\begin{proof}
Using the expression of the Horvitz-Thompson estimator, we have:
\begin{align*}
& \Var\left(\widehat{\tau}(d)  \right) \\
= &\frac{1}{N^2} \Var\left[\sum_{i=1}^N \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y; d) \right] \\
= & \frac{1}{N^2} \sum_{i=1}^N \Var\left[ \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y; d) \right] \\
& + \frac{1}{N^2} \sum_{i=1}^N \sum_{j \neq i} \Cov\left[ \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y; d), \left(\frac{Z_j}{p} - \frac{1-Z_j}{1-p}\right)\mu_j(\Y; d) \right] \\
= & \frac{1}{N^2} \sum_{i=1}^N \E\left[\left( \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y; d) \right)^2\right] - \frac{1}{N^2} \sum_{i=1}^N \left(\E\left[ \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y; d) \right] \right)^2\\
& + \frac{1}{N^2} \sum_{i=1}^N \sum_{j \neq i} \Cov\left[ \frac{Z_i}{p}\mu_i(\Y; d), \frac{Z_j}{p} \mu_j(\Y; d) \right] \\
& - \frac{1}{N^2} \sum_{i=1}^N \sum_{j \neq i} \Cov\left[ \frac{Z_i}{p}\mu_i(\Y; d), \frac{1-Z_j}{1-p} \mu_j(\Y; d) \right] \\
& - \frac{1}{N^2} \sum_{i=1}^N \sum_{j \neq i} \Cov\left[ \frac{1-Z_i}{1-p}\mu_i(\Y; d), \frac{Z_j}{p} \mu_j(\Y; d) \right] \\
& + \frac{1}{N^2} \sum_{i=1}^N \sum_{j \neq i} \Cov\left[ \frac{1-Z_i}{1-p}\mu_i(\Y; d), \frac{1-Z_j}{1-p} \mu_j(\Y; d) \right].
\end{align*}

We further expand the first two terms in the above expression:
\begin{align*}
 & \frac{1}{N^2} \sum_{i=1}^N \E\left[\left( \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y; d) \right)^2\right] - \frac{1}{N^2} \sum_{i=1}^N \E\left[ \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y; d) \right]^2\\
= & \frac{1}{N^2} \sum_{i=1}^N \E\left[ \frac{Z_i^2}{p^2} \mu_i^2(\Y; d) \right] + \frac{1}{N^2} \sum_{i=1}^N \E\left[ \frac{(1-Z_i)^2}{(1-p)^2} \mu_i^2(\Y); d) \right] \\
& - \frac{1}{N^2} \sum_{i=1}^N \E^2\left[ \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y; d) \right] \\
= & \frac{1}{N^2p} \sum_{i=1}^N \E\left[\muit^2\right] + \frac{1}{N^2(1-p)} \sum_{i=1}^N \E\left[ \muic^2\right] - \frac{1}{N^2} \sum_{i=1}^N \left(\E\left[\muit - \muic \right]\right)^2 \\
\leq &  \frac{1}{N^2p} \sum_{i=1}^N \E\left[\muit^2 \right] + \frac{1}{N^2(1-p)} \sum_{i=1}^N \E\left[ \muic^2\right].
\end{align*}
We also have:
\begin{align*}
 \frac{1}{Np} \sum_{i=1}^N \E\left[\muit^2\right] + \frac{1}{N^2(1-p)} \sum_{i=1}^N \E\left[ \muic^2\right] - \frac{1}{N^2} \sum_{i=1}^N \left(\E\left[\muit - \muic \right]\right)^2= O\left(1\right),
\end{align*}
since C\ref{assn:bounded-y} implies that all the moments are bounded. Next, we examine the first covariance term, which equals
\begin{align*}
& \frac{1}{N^2} \sum_{i=1}^N \sum_{j \neq i} \Cov\left[ \frac{Z_i}{p}\mu_i(\Y(\Z); d), \frac{Z_j}{p} \mu_j(\Y(\Z); d) \right] = \frac{1}{N^2}\sumij\Cov\left[ \frac{Z_i}{p}\mu_i(\Y(\Z); d), \frac{Z_j}{p} \mu_j(\Y(\Z); d) \right] \\
= & \frac{1}{N^2} \sumij\E\left[\muitt\mujtt\right]- \frac{1}{N^2}\sumij\E\left[\muit \right]\E\left[\mujt \right].
\end{align*}
The first equality holds because of assumption C3 on local interference. For $j \notin \mathcal{B}(i;d)$, $\muitt =\muit$ and $\E\left[\muitt\mujtt \right] =\E[\muitt]\E[\mujt]$, following the definition of interference in Section 4. Moreover,
\begin{align*}
\frac{1}{N^2} \sumij\E\left[\muitt\mujtt\right]- \frac{1}{N^2}\sumij\E\left[\muit \right]\E\left[\mujt \right]= O\left(1\right),
\end{align*}
since $|\mathcal{B}(i;d)|$ is bounded by (C4a). Other covariance terms have similar forms. We obtain the bound of the variance and its convergence rate by combining these terms together. 
\end{proof}

%\begin{proof}
%Using the expression of the Horvitz-Thompson estimator, we have:
%\begin{align*}
%& \Var\left(\widehat{\tau}(d)  \right) \\
%= &\frac{1}{N^2} \Var\left[\sum_{i=1}^N \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y(\Z); d) \right] \\
%= & \frac{1}{N^2} \sum_{i=1}^N \Var\left[ \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y(\Z); d) \right] \\
%& + \frac{1}{N^2} \sum_{i=1}^N \sum_{j \neq i} \Cov\left[ \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y(\Z); d), \left(\frac{Z_j}{p} - \frac{1-Z_j}{1-p}\right)\mu_j(\Y(\Z); d) \right] \\
%= & \frac{1}{N^2} \sum_{i=1}^N \Var\left[ \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y(\Z); d) \right] \\
%& + \frac{1}{N^2} \sum_{i=1}^N \sum_{j \in \mathcal{B}(i;d)} \Cov\left[ \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y(\Z); d), \left(\frac{Z_j}{p} - \frac{1-Z_j}{1-p}\right)\mu_j(\Y(\Z); d) \right] \\
%= & \frac{1}{N}\times \frac{1}{N}\Var\left[ \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y(\Z); d) \right] \\
%+ & \frac{1}{N}\times \frac{1}{N}\sum_{i=1}^N \sum_{j\in\mathcal{B}(i;d)}\Cov\left[ \left(\frac{Z_i}{p} - \frac{1-Z_i}{1-p}\right)\mu_i(\Y(\Z); d), \left(\frac{Z_j}{p} - \frac{1-Z_j}{1-p}\right)\mu_j(\Y(\Z); d) \right]\\
%= & \frac{1}{N}\times O(1) + \frac{1}{N}\times O(1),
%\end{align*}
%where for the last line we used C\ref{assn:bounded-y}-C\ref{assn:local-inf}. In particular the cardinally of $\mathcal{B}(i;d)$ is bounded for all $i=1,...,N$.
%\end{proof}

Next, we derive the limiting variance of the Hajek estimator using linearization.

\begin{lemma}\label{lemma:ha-var}
Consider the estimator $\widehat{\tau}_{HA}(d)$ defined in (\ref{eq:hajek}). It has the following asymptotic linear expansion:
\begin{align*}\label{eq:ha-taylor}
	& \widehat{\tau}^{Taylor}_{HA}(d) = \bar{\mu}^1(d)-\bar{\mu}^0(d) + \frac{1}{Np}\sum_{i=1}^N Z_i( \mu_i(\Y(\Z); d) - \bar{\mu}^1(d)) \\
	&  -  \frac{1}{Np}\sum_{i=1}^N (1-Z_i)(\mu_i(\Y(\Z);d) -\bar{\mu}^0(d)),
\end{align*}
where $\bar{\mu}^1(d) = \frac{1}{N}\sum_{i=1}^N \E \left[\mu_i(\Y(1,\Z_{-i}); d)\right]$ and $\bar{\mu}^0(d) = \frac{1}{N}\sum_{i=1}^N \E \left[\mu_i(\Y(0,\Z_{-i}); d)\right]$.
Such an expansion satisfies
\begin{align*}
\sqrt{N}( \widehat{\tau}^{Taylor}_{HA}(d)-\widehat{\tau}_{HA}(d))=o_p(1).
\end{align*}
\end{lemma}

\begin{proof}
Denote $\hat{\mu}^1(d)=\frac{1}{Np}\sum_{i=1}^N Z_i \mu_i(\Y(\Z); d)$, $\hat{\mu}^0(d)=\frac{1}{N(1-p)}\sum_{i=1}^N (1-Z_i) \mu_i(\Y(\Z); d)$, $\hat{N}_1=\frac{\sum_{i=1}^N Z_i}{Np}$, $\hat{N}_0=\frac{\sum_{i=1}^N (1-Z_i)}{N(1-p)}$, and $\W = (\hat{\mu}^1(d), \hat{\mu}^0(d), \hat{N}_1, \hat{N}_0)$.  

We know that $\E \left[\hat{\mu}^1(d) \right] = \bar{\mu}^1(d)$, $\E \left[\hat{\mu}^0(d) \right] = \bar{\mu}^0(d)$, $\E[\hat{N}_1] = \E[\hat{N}_0] =1$. Thus, $\E[ \W] = (\bar{\mu}^1(d), \bar{\mu}^0(d)), 1, 1)$. Define $f(a, b, c, d) = \frac{a}{c} - \frac{b}{d}$. Then the Hajek estimator can be written as $ f(\W)=f(\hat{\mu}^1(d), \hat{\mu}^0(d), \hat{N}_1, \hat{N}_0)$.

With probability approaching $1$, we have the following Taylor expansion of the Hajek estimator:
\begin{align*}
& \widehat{\tau}_{HA}(d) = \sqrt{N}f(\hat{\mu}^1(d), \hat{\mu}^0(d), \hat{N}_1, \hat{N}_0) = f(\W) \\
= & f(\E[ \W]) + \left.\frac{\partial f}{\partial \W}\right|'_{\W=\E[ \W]}(\W - \E[ \W]) + O_P(||\W - \E[ \W]||_2^2).\footnote{ $||\cdot||$ denotes the vector $l_2$ norm.}
\end{align*}
Following the same argument as in Lemma \ref{lemma:ht-var}, we have that $N||\W - \E[ \W]||_2^2=O_p(1)$ and $O_P(\sqrt{N}||\W - \E[ \W]||_2^2)=o_P(1)$. It is easy to see that $ \frac{\partial f}{\partial \W}|_{\E[ \W]} = (1, -1, -\bar{\mu}^1(d), \bar{\mu}^0(d))^{'}$. Some algebraic manipulations prove that the first two terms simplify to the expressions in $\hat{\tau}_{HA}^{Taylor}(d)$. 
\end{proof}

\begin{lemma}\label{lemma:ha-var-homo}
The variance of the linearized Hajek estimator can be expressed as

\begin{align}
	& \Var \left(\widehat{\tau}_{HA}^{Taylor}(d)\right)\\
	=&\frac{1}{N^2p}\sum_{i=1}^N \E\left[\left(\mu_i(\Y(1, \Z_{-i}); d) - \bar {\mu}^1\right)^2\right] + \frac{1}{N^2(1-p)}\sum_{i=1}^N \E\left[\left(\mu_i(\Y(0, \Z_{-i}); d)- \bar {\mu}^0\right)^2\right]  \label{LemmaA4:hajekvar1}\\
	-&  \frac{1}{N^2}\sum_{i=1}^N\E^2\left[ \mu_i(\Y(1, \Z_{-i}); d) - \mu_i(\Y(0, \Z_{-i}); d) - (\bar{\mu}^1(d) - \bar{\mu}^0(d) )\right]\\
	+ & \frac{1}{N^2} \sum_{i=1} \sum_{j \in \mathcal{B}(i;d)}\sum_{a,b=0}^1 (-1)^{a+b} \E[\left(\mu_i(\Y(a, b, \Z_{-(i, j)}); d) - \bar{\mu}^a(d)\right) \left(\mu_j(\Y(a, b, \Z_{-(i,j)}); d) - \bar{\mu}^b(d)\right)] \\
	- & \frac{1}{N^2} \sum_{i=1} \sum_{j \in \mathcal{B}(i;d)}\sum_{a,b=0}^1 (-1)^{a+b} \E[\mu_i(\Y(a, \Z_{-i}); d) - \bar{\mu}^a(d)] E[\mu_j(\Y(b, \Z_{-j}); d) - \bar{\mu}^b(d)], \label{LemmaA4:hajekvar2}
\end{align}

Under conditions C\ref{assn:bern-des}-C\ref{assn:homo}, we have the following variance bound for $\Var \left(\widehat{\tau}_{HA}^{Taylor}(d)\right)$:
\begin{align}
\tilde{V} = & \frac{1}{N^2p}\sum_{i=1}^N \E\left[\left(\mu_i(\Y(1, \Z_{-i}); d) - \bar {\mu}^1(d)\right)^2\right] + \frac{1}{N^2(1-p)}\sum_{i=1}^N \E\left[\left(\mu_i(\Y(0, \Z_{-i}); d)- \bar {\mu}^0(d)\right)^2\right] \label{LemmaA4:hajekvarb1}\\
+ & \frac{1}{N^2} \sum_{i=1} \sum_{j \in \mathcal{B}(i;d)}\sum_{a,b=0}^1 (-1)^{a+b} \E[\left(\mu_i(\Y(a, b, \Z_{-(i, j)}); d) - \bar{\mu}^a(d)\right) \left(\mu_j(\Y(a, b, \Z_{-(i,j)}); d) - \bar{\mu}^b(d)\right)].\label{LemmaA4:hajekvarb2}
\end{align}
\end{lemma}
\begin{proof}
	Recalling the definitions of $\W$ and $f(\cdot)$ from the proof of Lemma \ref{lemma:ha-var}, we first characterize the variance of the linearized Hajek estimator is:
	\begin{align*}
		& \Var \left(\widehat{\tau}_{HA}^{Taylor}(d)\right) = \E\left[ \left.\frac{\partial f}{\partial \W}\right|'_{\W=\E[ \W]}*(\W - \E[ \W]) \right]^2  \\
		= & \left(\frac{\partial f}{\partial \W}|_{\E[ \W]}\right)^{'}\Var\left[\W\right]\frac{\partial f}{\partial \W}|_{\E[ \W]}
	\end{align*}
	Further,
	\begin{align*}
		& \Var\left[\W\right] = \\
		& \begin{pmatrix}
			\Var\left[\hat{\mu}^1(d)\right] & \Cov\left[\hat{\mu}^1(d), \hat{\mu}^0(d)\right] & \Cov\left[\hat{\mu}^1(d), \hat{N}_1\right] & \Cov\left[\hat{\mu}^1(d), \hat{N}_0\right] \\
			\Cov\left[\hat{\mu}^1(d), \hat{\mu}^0(d)\right] & \Var\left[\hat{\mu}^0(d)\right] & \Cov\left[\hat{\mu}^0(d), \hat{N}_1\right] & \Cov\left[\hat{\mu}^0(d), \hat{N}_0\right] \\
			\Cov\left[\hat{\mu}^1(d), \hat{N}_1\right]  & \Cov\left[\hat{\mu}^0(d), \hat{N}_1\right] & \Var\left[\hat{N}_1\right] & \Cov\left[\hat{N}_1, \hat{N}_0\right] \\
			\Cov\left[\hat{\mu}^1(d), \hat{N}_0\right] & \Cov\left[\hat{\mu}^0(d), \hat{N}_0\right] & \Cov\left[\hat{N}_1, \hat{N}_0\right] & \Var\left[\hat{N}_0\right]
		\end{pmatrix} 
	\end{align*}
	Therefore,
	\begin{align*}
		& \left(\frac{\partial f}{\partial \W}|_{\E[ \W]}\right)^{'}\Var\left[\W\right]\frac{\partial f}{\partial \W}|_{\E[ \W]} \\
		= & \Var\left[\hat{\mu}^1(d)\right] + \Var\left[\hat{\mu}^0(d)\right] +\left(\bar{\mu}^1(d) \right)^2\Var\left[\hat{N}_1\right]  + \left(\bar{\mu}^0(d) \right)^2\Var\left[\hat{N}_0\right]  \\
		& -2\Cov\left[\hat{\mu}^1(d), \hat{\mu}^0(d)\right] - 2\bar{\mu}^1(d) \Cov\left[\hat{\mu}^1(d), \hat{N}_1\right] + 2\bar{\mu}^0(d) \Cov\left[\hat{\mu}^1(d), \hat{N}_0\right] \\
		& + 2\bar{\mu}^1(d) \Cov\left[\hat{\mu}^0(d), \hat{N}_1\right] - 2\bar{\mu}^0(d) \Cov\left[\hat{\mu}^0(d), \hat{N}_0\right] - 2\left(\bar{\mu}^1(d) \bar{\mu}^0(d)\right)\Cov\left[ \hat{N}_1, \hat{N}_0\right] \\
		= &\Var\left[\hat{\mu}^1(d) - \bar{\mu}^1(d) \hat{N}_1\right] + \Var\left[\hat{\mu}^0(d) - \bar{\mu}^0(d) \hat{N}_0\right] - 2\Cov\left[\hat{\mu}^1(d) - \bar{\mu}^1(d) \hat{N}_1, \hat{\mu}^0(d) - \bar{\mu}^0(d) \hat{N}_0\right] \\
%		= & \Var\left[\hat{\mu}^1(d) - \bar{\mu}^1(d) \hat{N}_1 - \left(\hat{\mu}^0(d) - \bar{\mu}^0(d) \hat{N}_0\right)\right] \\
	%	= & \Var\left[\hat{\mu}^1(d) - \hat{\mu}^0(d)\right] +  \Var\left[\bar{\mu}^1(d) \hat{N}_1 - \bar{\mu}^0(d) \hat{N}_0\right] - 2\Cov\left[\hat{\mu}^1(d) - \hat{\mu}^0(d), \bar{\mu}^1(d) \hat{N}_1 - \bar{\mu}^0(d) \hat{N}_0\right] \\
%		= & \Var\left(\hat \tau(d)\right) -  \Var\left[\bar{\mu}^1(d) \hat{N}_1 - \bar{\mu}^0(d) \hat{N}_0\right] \\
%		& - 2\Cov\left[\hat{\mu}^1(d) - \hat{\mu}^0(d) - \left(\bar{\mu}^1(d) \hat{N}_1 - \bar{\mu}^0(d) \hat{N}_0\right), \bar{\mu}^1(d) \hat{N}_1 - \bar{\mu}^0(d) \hat{N}_0\right].
	\end{align*}
%	It is thus obvious that $\Var \left(\widehat{\tau}_{HA}^{Taylor}(d)\right)$ is no larger than $\Var\left(\hat \tau(d)\right)$ as long as the covariance term in the last line is positive or sufficiently small. From our derivation below, we can see that the magnitude of this term is decided by the average difference between $\tau(d;\eta) = \bar{\mu}^1(d) - \bar{\mu}^0(d)$ and $\E\left[\mu_i(\Y(1, 1, \Z_{-(i,j)}); d)\right] - \E\left[\mu_i(\Y(0, 1, \Z_{-(i,j)}); d)\right]$ or $\E\left[\mu_i(\Y(1, 0, \Z_{-(i,j)}); d)\right] - \E\left[\mu_i(\Y(0, 0, \Z_{-(i,j)}); d)\right]$. The last two terms capture the ``indirect effect'' generated by the treatment effect of another node $j$ on the circle average of node $i$. Therefore, the covariance term will offset the variance term only when the average indirect effect dominates the AME at $d$. Even though we can construct scenarios where this is true, such scenarios should not be common in practice.
	
	For the term $  \Var\left[\hat{\mu}^1(d) - \bar{\mu}^1(d) \hat{N}_1\right]  $, we have:
	\begin{align*}
		& \Var\left[\hat{\mu}^1(d) - \bar{\mu}^1(d) \hat{N}_1\right] = \frac{1}{N^2p^2}\Var\left[\sum_{i=1}^N Z_i\left(\mu_i(\Y(\Z); d) - \bar{\mu}^1(d) \right)\right] \\
		= & \frac{1}{N^2p^2}\sum_{i=1}^N\Var\left[ Z_i\left(\mu_i(\Y(\Z); d) - \bar{\mu}^1(d) \right)\right] \\
		& + \frac{1}{N^2p^2}\sum_{i=1}^N\sum_{j\neq i}\Cov\left[ Z_i\left(\mu_i(\Y(\Z); d) - \bar{\mu}^1(d) \right), Z_j\left(\mu_j(\Y(\Z); d) - \bar{\mu}^1(d) \right)\right] \\
		= & \frac{1}{N^2p^2}\sum_{i=1}^N\E\left[ Z_i\left(\mu_i(\Y(\Z); d) - \bar{\mu}^1(d) \right)\right]^2 - \frac{1}{N^2p^2}\sum_{i=1}^N\E^2\left[ Z_i\left(\mu_i(\Y(\Z); d) - \bar{\mu}^1(d) \right)\right] \\
		& + \frac{1}{N^2p^2}\sum_{i=1}^N\sum_{j \neq i}\Cov\left[ Z_i\left(\mu_i(\Y(\Z); d) - \bar{\mu}^1(d) \right), Z_j\left(\mu_j(\Y(\Z); d) - \bar{\mu}^1(d) \right)\right]\\
		= & \frac{1}{N^2p}\sum_{i=1}^N\E\left[\mu_i(\Y(1, \Z_{-i}); d) - \bar{\mu}^1(d) \right]^2  - \frac{1}{N^2}\sum_{i=1}^N\E^2\left[ \mu_i(\Y(1, \Z_{-i}); d) - \bar{\mu}^1(d) \right] \\
		& + \frac{1}{N^2}\sum_{i=1}^N\sum_{j \neq i}\E\left[ \left(\mu_i(\Y(1, 1, \Z_{-(i,j)}); d) - \bar{\mu}^1(d) \right)\left(\mu_j(\Y(1, 1, \Z_{-(i, j)}); d) - \bar{\mu}^1(d) \right)\right] \\
		& - \frac{1}{N^2}\sum_{i=1}^N\sum_{j \neq i}\E\left[\mu_i(\Y(1, \Z_{-i}); d) - \bar{\mu}^1(d) \right] \E\left[\mu_j(\Y(1, \Z_{-j}); d) - \bar{\mu}^1(d) \right] \\
		= & \frac{1}{N^2p}\sum_{i=1}^N\E\left[\mu_i(\Y(1, \Z_{-i}); d) - \bar{\mu}^1(d) \right]^2  - \frac{1}{N^2}\sum_{i=1}^N\E^2\left[ \mu_i(\Y(1, \Z_{-i}); d) - \bar{\mu}^1(d) \right] \\
		& + \frac{1}{N^2}\sum_{i=1}^N\sum_{j\in\mathcal{B}(i;d)}\E\left[ \left(\mu_i(\Y(1, 1, \Z_{-(i,j)}); d) - \bar{\mu}^1(d) \right)\left(\mu_j(\Y(1, 1, \Z_{-(i, j)}); d) - \bar{\mu}^1(d) \right)\right] \\
		& - \frac{1}{N^2}\sum_{i=1}^N\sum_{j\in\mathcal{B}(i;d)}\E\left[\mu_i(\Y(1, \Z_{-i}); d) - \bar{\mu}^1(d) \right] \E\left[\mu_j(\Y(1, \Z_{-j}); d) - \bar{\mu}^1(d) \right] ].
	\end{align*}
	Similarly, 	for the term $ \Var\left[\hat{\mu}^0(d) - \bar{\mu}^0(d) \hat{N}_1\right] $, we have:
	\begin{align*}
		& \Var\left[\hat{\mu}^0(d) - \bar{\mu}^0(d) \hat{N}_0\right] \\
		= & \frac{1}{N^2(1-p)}\sum_{i=1}^N\E\left[\mu_i(\Y(0, \Z_{-i}); d) - \bar{\mu}^0(d) \right]^2  - \frac{1}{N^2}\sum_{i=1}^N\E^2\left[ \mu_i(\Y(0, \Z_{-i}); d) - \bar{\mu}^0(d) \right] \\
		& + \frac{1}{N^2}\sum_{i=1}^N\sum_{j\in\mathcal{B}(i;d)}\E\left[ \left(\mu_i(\Y(0, 0, \Z_{-(i,j)}); d) - \bar{\mu}^0(d) \right)\left(\mu_j(\Y(0, 0, \Z_{-(i, j)}); d) - \bar{\mu}^0(d) \right)\right] \\
		& - \frac{1}{N^2}\sum_{i=1}^N\sum_{j\in\mathcal{B}(i;d)}\E\left[\mu_i(\Y(0, \Z_{-i}); d) - \bar{\mu}^0(d) \right] \E\left[\mu_j(\Y(0, \Z_{-j}); d) - \bar{\mu}^0(d) \right] ].
	\end{align*}
For the term  $\Cov\left[\hat{\mu}^1(d) - \bar{\mu}^1(d) \hat{N}_1, \hat{\mu}^0(d) - \bar{\mu}^0(d) \hat{N}_0\right]$, we have
	\begin{align*}
		& \Cov\left[\hat{\mu}^1(d) - \bar{\mu}^1(d) \hat{N}_1, \hat{\mu}^0(d) - \bar{\mu}^0(d) \hat{N}_0\right] \\
		= & \frac{1}{N^2p(1-p)}\Cov\left[\sum_{i=1}^N Z_i\left(\mu_i(\Y(\Z); d) - \bar{\mu}^1(d) \right), \sum_{j=1}^N (1-Z_j)\left(\mu_j(\Y(\Z); d) - \bar{\mu}^0(d) \right)\right]  \\
		= & - \frac{1}{N^2}\sum_{i=1}^N\E\left[\mu_i(\Y(1, \Z_{-i}); d) - \bar{\mu}^1(d) \right] \E\left[\mu_i(\Y(0, \Z_{-i}); d) - \bar{\mu}^0(d)\right] \\
		& +  \frac{1}{N^2}\sum_{i=1}^N\sum_{j \neq i}^N\E\left[ \left(\mu_i(\Y(1, 0, \Z_{-(i, j)}); d) - \bar{\mu}^1(d) \right) \left(\mu_j(\Y(1, 0, \Z_{-(i, j)}); d) - \bar{\mu}^0(d) \right)\right]\\
		& - \frac{1}{N^2}\sum_{i=1}^N\sum_{j \neq i}^N\E\left[\mu_i(\Y(1, \Z_{-i}); d) - \bar{\mu}^1(d) \right] \E\left[\mu_j(\Y(0, \Z_{-j}); d) - \bar{\mu}^0(d)\right]\\
		= & - \frac{1}{N^2}\sum_{i=1}^N\E\left[\mu_i(\Y(1, \Z_{-i}); d) - \bar{\mu}^1(d) \right] \E\left[\mu_i(\Y(0, \Z_{-i}); d) - \bar{\mu}^0(d)\right] \\
		& +  \frac{1}{N^2}\sum_{i=1}^N\sum_{j\in \mathcal{B}(i;d)}^N\E\left[ \left(\mu_i(\Y(1, 0, \Z_{-(i, j)}); d) - \bar{\mu}^1(d) \right) \left(\mu_j(\Y(1, 0, \Z_{-(i, j)}); d) - \bar{\mu}^0(d) \right)\right]\\
		& - \frac{1}{N^2}\sum_{i=1}^N\sum_{j\in \mathcal{B}(i;d)}^N\E\left[\mu_i(\Y(1, \Z_{-i}); d) - \bar{\mu}^1(d) \right] \E\left[\mu_j(\Y(0, \Z_{-j}); d) - \bar{\mu}^0(d)\right]
	\end{align*}
Combining these terms leads to the variance expression stated in the lemma. Note that for the terms in  lines (\ref{LemmaA4:hajekvar1}) and (\ref{LemmaA4:hajekvar2})  we have, up to a minus sign, that
%Alternatively, we also have:
%	\begin{align*}
%	& \Cov\left[\hat{\mu}^1(d) - \bar{\mu}^1(d) \hat{N}_1, \hat{\mu}^0(d) - \bar{\mu}^0(d) \hat{N}_0\right] \\
%	= & \frac{1}{N^2p(1-p)}\Cov\left[\sum_{i=1}^N Z_i\left(\mu_i(\Y(\Z); d) - \bar{\mu}^1(d) \right), \sum_{j=1}^N (1-Z_j)\left(\mu_j(\Y(\Z); d) - \bar{\mu}^0(d) \right)\right]  \\
%	= &  \frac{1}{N^2p(1-p)}\sum_{i=1}^N\sum_{j=1}^N\Cov\left[ Z_i\left(\mu_i(\Y(\Z); d) - \bar{\mu}^1(d) \right),  (1-Z_j)\left(\mu_j(\Y(\Z); d) - \bar{\mu}^0(d) \right)\right]\\
%	= &  \frac{1}{N^2p(1-p)}\sum_{i=1}^N\sum_{j=1}^N\Cov\left[ (1-Z_i)\left(\mu_i(\Y(\Z); d) - \bar{\mu}^1(d) \right),  Z_j\left(\mu_j(\Y(\Z); d) - \bar{\mu}^0(d) \right)\right]\\
%	= &   \frac{1}{N^2p(1-p)}\sum_{i=1}^N \sum_{j\in \mathcal{B}(i;d)}\Cov\left[ (1-Z_i)\left(\mu_i(\Y(\Z); d) - \bar{\mu}^1(d) \right),  Z_j\left(\mu_j(\Y(\Z); d) - \bar{\mu}^0(d) \right)\right]
%\end{align*}
%Thus we have:
%\begin{align*}
%2&\Cov\left[\hat{\mu}^1(d) - \bar{\mu}^1(d) \hat{N}_1, \hat{\mu}^0(d) - \bar{\mu}^0(d) \hat{N}_0\right]\\
%=&\frac{1}{N^2p(1-p)}\sum_{i=1}^N \sum_{j\in \mathcal{B}(i;d)}\Cov\left[ Z_i\left(\mu_i(\Y(\Z); d) - \bar{\mu}^1(d) \right),  (1-Z_j)\left(\mu_j(\Y(\Z); d) - \bar{\mu}^0(d) \right)\right]  \\
%+ &  \frac{1}{N^2p(1-p)}\sum_{i=1}^N \sum_{j\in \mathcal{B}(i;d)}\Cov\left[ (1-Z_i)\left(\mu_i(\Y(\Z); d) - \bar{\mu}^1(d) \right),  Z_j\left(\mu_j(\Y(\Z); d) - \bar{\mu}^0(d) \right)\right]
%\end{align*}
%We now prove the variance bounding result.  This follows by noting that second to fifth lines of the expression in (\ref{lemma:ha-var-formula}) can be expanded as:
%\begin{align*}
%= & \frac{1}{N^2p^2} \sum_{i=1} \sum_{j \in \mathcal{B}(i;d)}\E[Z_iZ_j\left(\mu_i(\Y(\Z); d) - \bar{\mu}^1(d)\right)\left( \mu_j(\Y(\Z); d) - \bar{\mu}^0(d)\right)]\\
%& + \frac{1}{N^2(1-p)^2} \sum_{i=1} \sum_{j \in \mathcal{B}(i;d)}\E[(1-Z_i)(1-Z_j)\left(\mu_i(\Y(\Z); d) - \bar{\mu}^1(d)\right)\left( \mu_j(\Y(\Z); d) - \bar{\mu}^0(d)\right)] \\
%& -\frac{1}{N^2p(1-p)} \sum_{i=1} \sum_{j \in \mathcal{B}(i;d)}\E[(1-Z_i)Z_j\left(\mu_i(\Y(\Z); d) - \bar{\mu}^1(d)\right)\left( \mu_j(\Y(\Z); d) - \bar{\mu}^0(d)\right)] \\
%& - \frac{1}{N^2p(1-p)} \sum_{i=1} \sum_{j \in \mathcal{B}(i;d)}\E[
%Z_i(1-Z_j)\left(\mu_i(\Y(\Z); d) - \bar{\mu}^1(d)\right)\left( \mu_j(\Y(\Z); d) - \bar{\mu}^0(d)\right)] \\ 
%& - \frac{1}{N^2} \sum_{i=1} \sum_{j \in \mathcal{B}(i;d)}\sum_{a,b=0}^1 (-1)^{a+b}\E\left[\mu_i(\Y(a, \Z_{-i}); d) - \bar{\mu}^1(d)\right] \E\left[\mu_j(\Y(b, \Z_{-j}); d) - \bar{\mu}^0(d)\right].
%\end{align*}
%All we need to show is that the last line  is less than or equal to zero in the limit under C\ref{assn:homo}. We know that,
%\begin{align*}
%& \frac{1}{N}\sum_{i=1}^N \sum_{j\in \mathcal{B}(i;d)}(-1)^{a+b}\E\left[\mu_i(\Y(a,\Z_{-i}); d) - \bar{\mu}^a(d)\right] \E\left[\mu_j(\Y(b,\Z_{-j}); d) - \bar{\mu}^b(d) \right]  \\
%= & \frac{1}{N}\sum_{i=1}^N \sum_{j\in \mathcal{B}(i;d)}\E\left[\mu_i(\Y(a,\Z_{-i}); d)\right] \E\left[\mu_j(\Y(b,\Z_{-j}); d) \right] \\
%& - \frac{1}{N^2} \left(\sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i;d)} \E \left[\mu_i (\Y(a, \mathbf{Z}_{-i});d)\right]\right)\sum_{k=1}^N \E \left[\mu_k (\Y(b, \mathbf{Z}_{-k});d)\right] \\
%& - \frac{1}{N^2} \left(\sum_{i=1}^{N} \sum_{j \in \mathcal{B}(i;d)} \E \left[\mu_j (\Y(b, \mathbf{Z}_{-j});d)\right]\right)\sum_{k=1}^N \E \left[\mu_k (\Y(a, \mathbf{Z}_{-k});d)\right] \\
%& + \frac{1}{N}\sum_{i=1}^N \sum_{j\in \mathcal{B}(i;d)}\frac{1}{N^2} \left(\sum_{k=1}^N \E \left[\mu_k (\Y(a, \mathbf{Z}_{-k});d)\right]\right) \left(\sum_{l=1}^N \E \left[\mu_l (\Y(b, \mathbf{Z}_{-k});d)\right]\right)  + o_P(1) \\
%= & \frac{1}{N}\sum_{i=1}^N \E \left[\mu_i (\Y(a, \mathbf{Z}_{-k});d)\right]  \left(\sum_{j \in \mathcal{B}(i;d)} \E \left[\mu_j (\Y(b, \mathbf{Z}_{-i});d)\right] - \frac{1}{N}\sum_{k=1}^{N} \sum_{j \in \mathcal{B}(k;d)} \E \left[\mu_k (\Y(b, \mathbf{Z}_{-k});d)\right]\right)\\
%& + \frac{1}{N^2} \sum_{i=1}^{N}\sum_{k=1}^N \left(c_i(d) - \frac{1}{N}\sum_{i=1}^N c_i(d)\right) \E \left[\mu_i (\Y(a, \mathbf{Z}_{-i});d)\right] \E \left[\mu_k (\Y(b, \mathbf{Z}_{-k});d)\right].
%\end{align*}
\begin{align*}
& \frac{1}{N^2}\sum_{i=1}^N\E^2\left[ \mu_i(\Y(1, \Z_{-i}); d) - \mu_i(\Y(0, \Z_{-i}); d) - (\bar{\mu}^1(d) - \bar{\mu}^0(d) )\right] \\
& + \frac{1}{N}\sum_{i=1}^N \sum_{j\in \mathcal{B}(i;d)} \sum_{a,b=0}^1 (-1)^{a+b}\E\left[\mu_i(\Y(a,\Z_{-i}); d) - \bar{\mu}^a(d)\right] \E\left[\mu_j(\Y(b,\Z_{-j}); d) - \bar{\mu}^b(d) \right]  \\
= & \frac{1}{N}\sum_{i=1}^N  (\tau_i(d;\eta) - \tau(d;\eta))^2 \\
 & + \frac{1}{N}\sum_{i=1}^N \sum_{j\in \mathcal{B}(i;d)} \bigg\{ \E\left[\mu_i(\Y(1,\Z_{-i}); d) - \bar{\mu}^1(d)\right] \\
& \times \E\left[\mu_j(\Y(1,\Z_{-j}); d) - \mu_j(\Y(0,\Z_{-j}); d) - (\bar{\mu}^1(d) - \bar{\mu}^0(d))\right]\bigg\} \\
& - \frac{1}{N}\sum_{i=1}^N \sum_{j\in \mathcal{B}(i;d)} \bigg\{ \E\left[\mu_j(\Y(0,\Z_{-j}); d) - \bar{\mu}^0(d)\right] \\ 
& \times \E\left[\mu_i(\Y(1,\Z_{-i}); d) - \mu_i(\Y(0,\Z_{-i}); d) - (\bar{\mu}^1(d) - \bar{\mu}^0(d))\right] \bigg\} \\
= & \frac{1}{N}\sum_{i=1}^N  (\tau_i(d;\eta) - \tau(d;\eta)) \sum_{j\in \{i\} \cup \mathcal{B}(i;d)} (\tau_j(d;\eta) - \tau(d;\eta)). 
\end{align*}
where $\tau_i(d;\eta)$, $\tau_j(d;\eta)$ and $\tau(d;\eta)$ are defined as in C\ref{assn:homo}. Hence the terms combining expressions in (\ref{LemmaA4:hajekvar1}) and (\ref{LemmaA4:hajekvar2})  is smaller than or equal to zero in the limit under C\ref{assn:homo}, which proves the lemma.
%Under C5, $\sum_{j \in \mathcal{B}(i;d)} \E \left[\mu_j (\Y(b, \mathbf{Z}_{-i});d)\right] = \frac{1}{N}\sum_{k=1}^{N} \sum_{j \in \mathcal{B}(k;d)} \E \left[\mu_k (\Y(b, \mathbf{Z}_{-k});d)\right] + o_P(1)$ and $c_i(d) = c(d) + o_P(1)$. Hence the expression above equals to $o_P(1)$. The lemma is proved. 
\end{proof}

%and show that we can consistently estimate the variance via the spatial HAC estimator under assumptions C1-C5. The following lemmas summarize some facts that will be used in the proof below.
%
%\begin{lemma}\label{lemma:local-inter1}
%Under assumption C3, the following equation holds:
%\begin{description}
%\item[C\ref{assn:local-inf}.1]\begin{align*}
%& \sum_{i=1}^N\sum_{j\notin \mathcal{B}(i;d)}\E\left[ \mu_i(\Y(a, b,\Z_{-(i,j)}); d) \mu_j(\Y(a, b, \Z_{-(i,j)}); d) \right] \\
%= & \sum_{i=1}^N\sum_{j\notin \mathcal{B}(i;d)}\E\left[ \mu_i(\Y(a, \Z_{-i}); d) \right]\E\left[\mu_j(\Y(b, \Z_{-j}); d) \right]
%\end{align*}    
%\end{description}
%for any $a, b\in \{0, 1\}$.
%\end{lemma}
%





